Nonparametric Involutive Markov Chain Monte Carlo

A challenging problem in probabilistic programming is to develop inference algorithms that work for arbitrary programs in a universal probabilistic programming language (PPL). We present the nonparametric involutive Markov chain Monte Carlo (NP-iMCMC) algorithm as a method for constructing MCMC inference algorithms for nonparametric models expressible in universal PPLs. Building on the unifying involutive MCMC framework, and by providing a general procedure for driving state movement between dimensions, we show that NP-iMCMC can generalise numerous existing iMCMC algorithms to work on nonparametric models. We prove the correctness of the NP-iMCMC sampler. Our empirical study shows that the existing strengths of several iMCMC algorithms carry over to their nonparametric extensions. Applying our method to the recently proposed Nonparametric HMC, an instance of (Multiple Step) NP-iMCMC, we have constructed several nonparametric extensions (all of which new) that exhibit significant performance improvements.

==> section/almost-sure-termination.tex <==
% !TEX root = ./../icml2022.tex

We start the correctness proof by checking whether \cref{alg: np-imcmc (hybrid)}
almost surely terminates (and generates a new sample).
Let $\enta$ denote the entropy trace computed in Line 12
and $\enta^{(n)} $ denote the entropy trace after $n$ iterations of
the while loop (Line 13 to 17).
Hence $\enta = \enta^{(0)}$.
Then, \cref{vass: partial block diagonal inv}
ensures that $\enta^{(n+1)} = \enta^{(n)} \concat [\entelem]$ for some $\entelem \in \entspace$.
Consider the termination condition of the while loop.
To terminate, we need to make sure that
for almost every infinite entropy trace $\entb$
there is a $k$ such that $\enta \concat \range{\entb}{1}{k}$ is in the support of $\extree$.

\begin{proposition}
  \label{prop: AST weight function iff AST truncations}
  Let $\tree$ be an almost surely terminating tree representable function
  on the trace space $\traces$.
  Then its extension $\extree$ satisfies the following.
  \begin{enumerate}
    \item $\measure{\entspace^n}{(\nsupport{n}{\extree})}\to 1$ as $n\to\infty$.

    \item $\measure{\entspace^n}{(\entspace^n\setminus \support{\trunc{n}})}\to 0$ as $n\to\infty$.
  \end{enumerate}
\end{proposition}

\begin{proof}
  \begin{enumerate}
    \item
    By \cref{prop: tree and extree}, we have
    $ \measure{\entspace^n}(\nsupport{n}{\extree})
    = \measure{\traces}(\bigcup_{i=1}^n \nsupport{i}{\tree})
    = \sum_{i=1}^n \measure{\traces}(\nsupport{i}{\tree})$.
    Letting $n \to \infty$, we get
    \begin{align*}
      \lim_{n\to\infty} \measure{\entspace^n}(\nsupport{n}{\extree})
      = \sum_{i=1}^{\infty} \measure{\traces}(\nsupport{i}{\tree})
      = \measure{\traces}(\bigcup_{i=1}^{\infty}\nsupport{i}{\tree})
      = \measure{\traces}(\support{\tree}) = 1
    \end{align*}

    \item Since $\measure{\entspace^n}$ is probabilistic, we have
    $
    \lim_{n\to\infty} \measure{\entspace^n}(\entspace^n \setminus \nsupport{n}{\extree})
    = \lim_{n\to\infty} \big( \measure{\entspace^n}(\entspace^n) - \measure{\entspace^n}(\nsupport{n}{\extree})\big)
    = \lim_{n\to\infty} \big( 1 - \measure{\entspace^n}(\nsupport{n}{\extree})\big)
    = 1 - \lim_{n\to\infty}\measure{\entspace^n}(\nsupport{n}{\extree})
    = 0
    $.

  \end{enumerate}
\end{proof}

\cref{prop: AST weight function iff AST truncations}.2 shows that the measure of
the set of entropy traces that is not in the support of $\extree$ tends to zero.
This means for almost every infinite entropy trace $\enta$,
there is a $k$ such that $\extree$ is positive on $\range{\enta}{1}{k}$.
Hence, the while loop (Line 13 to 17) almost surely terminates
and we have our first theorem.

\ast


==> section/case-studies.tex <==
% !TEX root = ./../icml2022.tex

Here we use the NP-iMCMC framework described in \cref{sec: np-imcmc}
with the special ingredients presented in \cref{sec: combination}
to design two novel MCMC algorithms for universal PPLs.
We first show how one can extend the Look Ahead Hamiltonian Monte Carlo sampler
(\cite{DBLP:conf/icml/Sohl-DicksteinMD14}) using the NP-iMCMC method.
Then, we design a novel


\begin{example}[NP-Gibbs with fixed scan]
\label{eg: np-gibbs with fixed scan}
Recall in \cref{eg: np-gibbs} we show how the Gibbs sampler can be extended to update the $i$-th component of a sample from nonparametric models.
In order to update all components of the sample, it is common for a Gibbs sampler to iterate through every component of the current sample.\footnote{Here, we consider the so-called ``fixed scan'' Gibbs sampler. There are other common Gibbs samplers, such as the ``random scan'', which is a state-independent mixture of the Gibbs updates.}
We can apply the same idea to NP-Gibbs by iterating through every component of the current sample.
As noted in \cref{eg: np-gibbs}, it is important that the position of updated component to be smaller than or equal to the size of the sample.
Hence, a fixed scan NP-Gibbs updates the current sample $\enta_0$ as follows:
\begin{compactenum}[1.]
  \item Initialise the position $i$ of the updated component to be $1$ and $\enta = \enta_0$.

  \item Test whether $i > \len{\enta}$. If so, return $\enta$ as the next sample; otherwise
  \begin{compactitem}
    \item Update the $i$-th component of $\enta$ via the NP-Gibbs (\cref{eg: np-gibbs}) method to obtain a new sample $\enta$
    \item Increment $i$ to $i+1$
    \item goto 2.
  \end{compactitem}
\end{compactenum}
\end{example}


==> section/convergence.tex <==
% !TEX root = ./../icml2022.tex

Last but not least, we check for
the convergence of the marginalised chain to the target distribution $\tdist$.

\begin{description}
  \item[\cass\label{cass: very strong irreducible}]
  $\ninvo{n}$ is \defn{very strong irreducible}.
  %i.e.~for all $n\in\Nat$, $\enta \in \entspace^n$ and $\entseta \in \algebra{\entspace^n}$ where $\enta \in \support{\trunc{n}} $ and $\tdist_n(\entseta) > 0$, there exists a non-null measurable set $\auxseta \in \algebra{\auxspace^n} $ where for all $\auxa \in \auxseta$, $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $,
  %where $\tdist_n$ is the distribution with pdf $1/Z_n\cdot\trunc{n}$ where $Z_n$ is the normalising constant.
  \changed[cm]{i.e.~for all $n\in\Nat$, $\enta \in \entspace^n$ and $\entseta \in \algebra{\entspace^n}$,
  if $\enta \in \support{\trunc{n}} $ and $\tdist_n(\entseta) > 0$ then there exists a non-null $\auxseta \in \algebra{\auxspace^n} $ such that for all $\auxa \in \auxseta$, $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $},
  where $\tdist_n$ is the distribution with pdf $1/Z_n\cdot\trunc{n}$ where $Z_n$ is the normalising constant.

\lo{This is a rather strong assumption.}

  \item[\cass\label{cass: everywhere positive aux density}] $\auxkernel{n}$ is \defn{everywhere positive}, i.e.~for all $\enta \in \entspace$ and $\auxa \in \auxspace$, $\auxpdf{n}(\enta,\auxa) > 0$.
\end{description}


Recall the conditions on the transition kernel to ensure convergence.

\begin{lemma}[\cite{Tierney94}, Theorem 1 and Corollary 2]
  \label{lemma: Tieryney}
  If the transition kernel $\transkernel{}$ with invariant distribution $\tdist$
  is $\tdist$-irreducible and $\tdist$-aperiodic, then
  for all $\state$, $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$ with $\norm{\cdot}$ denoting total variation distance.
\end{lemma}

\lo{Forget what I said about convergence in distribution -- I must have misremembered.
You are right: standard convergence results for Markov chains over continuous sample space are given in terms of total variational distance. See e.g.~\cite[Thm.~4]{Roberts2004} and \cite[Thm 11.3.1]{DoucMPS18}.}

% In our setting, we show that the irreducibility and aperiodicity of the \emph{fixed} dimension transition kernels w.r.t.~the \emph{fixed} dimension target distributions implies the same for the \emph{unbounded} transition kernel $\transkernel{\cref{alg: np-imcmc (hybrid)}}$.
We assume that \allvass{} and \allcass{} are satisfied.

\cm{\cref{cass: very strong irreducible} is slightly stronger than saying that the fixed dimension transition kernels are strongly irreducible. If the conclusion is $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $ or ($\accept(\enta,\auxa) \not=1$ and $\enta \in \entseta$), then it will be exactly strongly irreducibility.}

\cm{I would like to relax this assumption to assuming the fixed dimension transition kernels are just irreducible. But more work would need to be done.}

\begin{proposition}
  \label{prop: acceptance > 0}
  $\accept \not= 0$ on $\validstates$.
\end{proposition}

\begin{proof}
  Assume for contradiction that $(\enta,\auxa) \in \validstates$ is such that
  $\accept(\enta,\auxa) = 0$.
  Then for $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$,
  we must have either
  $\trunc{\len{\enta}}(\enta') = 0$ or
  $\nauxpdf{\len{\enta}}(\enta',\auxa') = 0$ or
  $\det(\grad{\ninvo{\len{\enta}}}(\enta,\auxa)) = 0$.
  By the definition of $\validstates$ and \cref{cass: everywhere positive aux density},
  $\trunc{\len{\enta}}(\enta') \not= 0$ and
  $\nauxpdf{\len{\enta}}(\enta',\auxa') \not= 0$.
  Moreover, since $\ninvo{\len{\enta}}$ is a continuously differentiable involution, by chain rule we have
  $\grad{(\ninvo{\len{\enta}} \circ \ninvo{\len{\enta}})}(\state) = \grad{\ninvo{\len{\enta}}}(\ninvo{\len{\enta}}(\state)) \cdot \grad{\ninvo{\len{\enta}}}(\state) = \id(\state)$.
  Hence $\det(\grad{\ninvo{\len{\enta}}}(\ninvo{\len{\enta}}(\state))) \cdot \det(\grad{\ninvo{\len{\enta}}}(\state)) = 1$ which tells us that
  $\det(\grad{\ninvo{\len{\enta}}}(\state)) \not= 0$.
\end{proof}

\begin{lemma}
  \label{lemma: strong irreducible}
  Let $\trace \in \traces$ and $\traceset \in \algebra{\traces}$ where $\tree(\trace) > 0$ and $\tdist(\traceset) > 0$.
  Then $\transkernel{\cref{alg: np-imcmc (hybrid)}}(\trace,\traceset) > 0$.
\end{lemma}

\begin{proof}
  Let $\trace \in \traces$ and $\traceset \in \algebra{\traces}$ where $\tree(\trace) > 0$ and $\tdist(\traceset) > 0$. We want to show that $\transkernel{\cref{alg: np-imcmc (hybrid)}}(\trace,\traceset) > 0$. Note that we have
  \begin{align*}
    \transkernel{\cref{alg: np-imcmc (hybrid)}}(\trace,\traceset) & := \transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(\traceset)) \tag{for $\state \in \inv{\marg}(\{\trace\})$} \\
    & = \int_{\states}\ \transkernel{2}(\state',\inv{\marg}(\traceset))\ \transkernel{1}(\state,\dif\state')\\
    & = \int_{\validstates}\ \transkernel{2}(\state',\inv{\marg}(\traceset))\ \transkernel{1}(\state,\dif\state').
    \tag{$\transkernel{1}(\state,\validstates) = 1 $}
  \end{align*}
  Hence we need to prove that there exists a measurable subset $\stateset \subseteq \validstates$ where (1) $\transkernel{1}(\state,\stateset) >0$ and (2) for all $\state' \in \stateset$, $\transkernel{2}(\state',\inv{\marg}(\traceset)) > 0 $.

  For sufficiently large $n \in \Nat$, we must have
  $\tdist_n(\proj{1}{\inv{\marg}(\traceset)\cap \validstates_n}) > 0$.
  By \cref{cass: very strong irreducible}, for any $\enta \in \entspace^n$ where $\NPempty(\enta,\tree) = \trace$, there exists a non-null measurable set $\auxseta_{\enta} \in \algebra{\auxspace^n} $ where for all $\auxa \in \auxseta_{\enta}$, $(\enta',\auxa') := \ninvo{n}(\enta,\auxa) \in \proj{1}{\inv{\marg}(\traceset)\cap \validstates_n} \times \auxspace^n $.
  Since $\enta, \enta' \in \support{\trunc{n}}$, there exists $k$ such that $(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \validstates$.

  We claim that $\stateset := \set{(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \validstates \mid \NPempty(\enta,\tree) = \trace \text{ and } \auxa \in \auxseta_{\enta}}$ satisfies (1) and (2).
  \begin{enumerate}[(1)]
    \item Consider $\transkernel{1}(\state,\stateset)$. Since $\auxseta_{\enta}$ is non-null for all $\enta \in \entspace^n$ where $\NPempty(\enta,\tree) = \trace$, by \cref{cass: everywhere positive aux density}
    \begin{align*}
      &\transkernel{1}(\state,\stateset) \\
      & =
      \sum_{n=1}^\infty
      \int_{\auxspace^n}
      \int_{\traces}
      [(\valuefn{\NPfill(\trace)}(\traceb') \concat\traceb'' ,\auxa) \in \stateset \cap \validstates_n]
      \nonumber \\
      & \qquad\qquad\qquad \nauxpdf{n}(\valuefn{\NPfill(\trace)}(\traceb') \concat\traceb'' ,\auxa)\
      {\measure{\traces}}{(\dif(\traceb' \concat\traceb''))}\
      {\measure{\auxspace^n}}{(\dif\auxa)} \\
      & =
      \sum_{k=1}^n
      \int_{\auxseta_{\enta}}
      \int_{\traces}
      [\enta = \valuefn{\NPfill(\trace)}(\traceb') \concat\traceb''] \cdot
      \nauxpdf{k}(\range{\enta}{1}{k},\range{\auxa}{1}{k})\
      {\measure{\traces}}{(\dif(\traceb' \concat\traceb''))}\
      {\measure{\auxspace^n}}{(\dif\auxa)} \\
      & > 0
    \end{align*}

    \item
    Let $(\entb,\auxb) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \stateset$ where $\NPempty(\enta,\tree) = \trace$ and $\auxa \in \auxseta_{\enta}$.
    \begin{align*}
      \transkernel{2}((\entb,\auxb), \inv{\marg}(\traceset))
      & :=
      \accept(\entb,\auxb)\cdot [\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)] \\
      & +
      (1-\accept(\entb,\auxb))\cdot [(\entb,\auxb) \in \inv{\marg}(\traceset)]
    \end{align*}
    By \cref{prop: acceptance > 0}, $\accept(\entb,\auxb) \not= 0$. So, it is enough to show $\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)$.

    Let $(\enta',\auxa') := \ninvo{n}(\enta,\auxa) \in \proj{1}{\inv{\marg}(\traceset)\cap \validstates_n} \times \auxspace^n $.
    Then, we have $\NPempty(\enta',\tree) \in A$.
    Since $\entb \in \support{\trunc{k}}$, applying \cref{vass: partial block diagonal inv} gives $\ninvo{k}(\entb,\auxb) = (\range{\enta'}{1}{k},\range{\auxa'}{1}{k})$.
    Since $(\entb,\auxb) \in \stateset \subseteq \validstates$, by \cref{prop: valid states are preserved by involutions} $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k}) \in \validstates$ and hence $\NPempty(\range{\enta'}{1}{k},\tree) = \NPempty(\enta',\tree) \in \traceset $.
    So $\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)$ and
    $\transkernel{2}((\entb,\auxb), \inv{\marg}(\traceset)) > 0$.
  \end{enumerate}
\end{proof}

\begin{lemma}[\cite{DBLP:conf/icfp/BorgstromLGS16}, Corollary~2 and Lemma~33]
  \label{lemma: strong irred implies irred and aperiodic}
  A strong $\tdist$-irreducible transition kernel is also $\tdist$-irreducible and $\tdist$-aperiodic.
\end{lemma}

Finally by Tierney's Theorem (\cref{lemma: Tieryney}), the
$\tdist$-irreducible and $\tdist$-aperiodic (\cref{lemma: strong irreducible,lemma: strong irred implies irred and aperiodic}) transition kernel $\transkernel{\cref{alg: np-imcmc (hybrid)}}$ with invariant distribution $\tdist$ (\cref{lemma: marginalised distribution is the target distribution}) generates a Markov chain that converges to the target distribution $\tdist$.

\convergence

==> section/correctness.tex <==
% !TEX root = ./../icml2022.tex

Here we show the correctness of the NP-iMCMC sampler with the hybrid parameter space.

\subsection{Hybrid Entropy Space}
\label{app: hybrid entropy space}

Before we formalise the algorithm, we change the definition of the entropy space in \cref{sec:trace space} and define new helper functions that translate traces to entropy traces.

The entropy space $\entspace$ is now defined to be the \emph{product} space of the SPCF continuous and discrete samplers.
Formally, $\entspace := \Real \times \Bool$,
\changed[lo]{$\algebra{\entspace} := \sigma\big(\set{\realset \times \boolset \mid \realset \in \Borel, \boolset \in \algebra{\Bool}}\big)$}
and $\measure{\entspace}(\entseta) := \expandint{\Bool}{\Gau(\set{\reala \in \Real \mid (\reala,\boola) \in \entseta})}{\measure{\Bool}}{\boola}$.\footnote{Since $\Gau$ and $\measure{\Bool}$ are $\sigma$-finite, the product measure is uniquely defined.}
%\lo{The preceding is confusing, and not a definition. A measure $\mu$ on a product measurable space is called a \emph{product measure} if it satisfies $\mu(V \times W) = \mu_1(V) \, \mu_2(W)$. Note that not all measurable subsets are of the form $V \times W$. If the measures are $\sigma$-finite, then the product measure is uniquely defined (but not if they are s-finite!).}
Again, we denote the product of $n$ copies of entropy space as $(\entspace^n, \algebra{\entspace^n}, \measure{\entspace^n})$ and call it the \defn{$n$-dimensional entropy space}.
Note that $\measure{\entspace}$ (and hence $\measure{\entspace^n}$) is a probability measure.
\changed[cm]{An \defn{entropy trace} is an element in some $n$-dimensional entropy space and is denoted as $\enta, \entb$.}
% \lo{@Carol: We should discuss this. What we call ``entropy trace'' or ``entropy trace'' (why variable?) is actually not an element of the entropy space $\entspace$, but rather a sequence of entropys i.e.~elements of $\bigcup_{n \geq 0} \entspace^n$. This is confusing. Though not ideal, it would be better to call them \emph{entropy traces}.}

Given an entropy trace $\enta$, we can construct traces $\traceb$ by selecting either a real or boolean value %for each coordinate
from each ordered pair of a prefix of $\enta$.
%($\dagger$)
\changed[cm]{For instance, from the entropy trace $[(-0.2,\true), (2.9, \true), (1.3, \false)]$, traces like $[-0.2,\true, \false]$ and $[\true]$ can be formed}, which we call \defn{instances} of the entropy.
\lo{The reader can easily confuse ``instances of $\enta$'' with ``instances of $\enta$ w.r.t.~$w$''.}
Formally, $\traceb \in \traces$ is an instance of an entropy trace $\enta \in \bigcup_{n \geq 0} \entspace^n$
%\lo{Should be $\enta \in \bigcup_{n \geq 0} \entspace^n$} if
$\len{\traceb} \leq \len{\enta}$ and
$\seqindex{\traceb}{i} \in \set{\reala,\boola \mid (\reala,\boola) = \seqindex{\enta}{i}}$ for all $i = 1,\dots, \len{\traceb}$.
We denote the set of all instances of $\enta$ as $\instances{\enta}$.

Furthermore, given a tree representable function $\tree$,
each entropy trace $\enta$ in the support of the extension $\extree$ of $\tree$ can be uniquely partitioned into three traces $\traceb_1, \traceb_2, \traceb_3$ where
\begin{itemize}
  \item $\traceb_1$ is the instance of $\enta$ that is in the support of $\tree$;

  \item $\traceb_2$ is the part of $\enta$ where $\zip(\traceb_1, \traceb_2) = \range{\enta}{1}{\len{\traceb_1}}$,
  where $\zip$ is a function that takes two sequences of equal length and return a sequence with pairs of elements from each input sequence;

  \item $\traceb_3$ is the suffix of $\enta$ where $\zip(\traceb_1, \traceb_2) \concat \traceb_3 = \enta$.
\end{itemize}
For instance, say $[\true, 2.9]$ is in the support of the tree representable function $\tree$.
Then, the entropy trace $[(-0.2,\true), (2.9, \true), (1.3, \false)]$ can be partitioned into
$[\true, 2.9]$,
$[-0.2, \true]$ and
$[1.3, \false]$.

% talking about empty and fill functions
\iffalse
there is at most one instance of $\enta$ that lies in the support of $\tree$.
The function $\NPempty:\bigcup_{n\in\Nat}\entspace^n\to\traces$ returns this instance if it exists. Formally
\[
  \NPempty(\enta)
  :=
  \begin{cases}
    \traceb\in\instances{\enta} & \text{if } \tree(\traceb) > 0 \\
    \emptytrace & \text{otherwise.}
  \end{cases}
\]

On the other hand,
given a trace $\traceb \in \traces$, we can construct an entropy trace $\enta$ by ``filling'' the missing components of the real-boolean pair.
For example, we can ``fill'' the trace $[-0.2,\true,\false]$ with a boolean $\false$ and real numbers $2.1$ and $1.1$ to make an entropy trace of the same dimension $[(-0.2,\false),(2.1,\true),(1.1,\false)]$.
The (stochastic) function $\NPfill(\traceb_0)$ in \cref{line: fill start} to \cref{line: fill end} fills the trace $\traceb_0$ by sampling from the respective distribution.
\fi

\subsection{Assumptions}
\label{sec: ass on vanilla np-imcmc}

We generalise the assumptions given in \cref{sec: assumptions} for the hybrid parameter space as follows:

\begin{description}

  \item[\cref{vass: integrable tree}] $\tree$ is \defn{integrable}, i.e.~$\shortint{\traces}{\tree}{\measure{\traces}} =: Z < \infty$.

  \item[\cref{vass: almost surely terminating tree}] $\tree$ is \defn{almost surely terminating (AST)}, i.e.~$\measure{\traces}(\set{\traceb\in \traces \mid \tree(\traceb) > 0}) = 1$.

  \item[\cref{vass: partial block diagonal inv}] $\ninvo{n}$ are \defn{partial block diagonal (PBD)},
  i.e.~For all $(\enta, \auxa) \in \states$ where $\traceb \in \support{\tree}\cap\instances{\enta}$, $\proj{\len{\enta}}{k}(\ninvo{\len{\enta}}(\enta, \auxa)) = \ninvo{\len{\traceb}}(\proj{\len{\enta}}{k}(\enta, \auxa)) $ for all $k = \len{\traceb}, \dots, \len{\enta}$.
\end{description}

Here we generalise the idea of extension of tree representable function in \cref{sec: assumptions} for the hybrid entropy space as
$\extree: \bigcup_{n\in\Nat}\entspace^n \to \pReal $ where
\[
  \extree:\enta \mapsto \max\{ \tree(\traceb) \mid \traceb \in \instances{\enta} \}
\]

The prefix property and \emph{type property} implies that for any $\enta \in \bigcup_{n\in\Nat}\entspace^n$,
\[
  \exists \traceb \in \instances{\enta} .\ \traceb \in \support{\tree}
  \iff
  \enta \in \support{\extree}.
\]

\iffalse
\subsubsection{Truncations}
\label{sec: truncations}

Given a tree representable function $\tree:\traces \to \pReal$,
we define its $n$-th \defn{truncation} $\trunc{n}$ as a measurable function \changed[lo]{on the $n$-dimensional entropy space} that captures the weight of $\tree$ up to the $n$-th dimension.
Formally, we have
\begin{align*}
  \trunc{n}:\ \entspace^n & \rightarrow \pReal \\
  \enta & \mapsto \sum \set{ \tree(\traceb) \mid \traceb\in \prefix{\enta}}
  \qquad\text{where }
  \prefix{\enta} := \set{\range{\enta}{1}{k}}_{k=1,\dots,\len{\enta}}
\end{align*}
%\lo{NOTE: This ``denegerate'' definition of $\prefix{\enta}$ is for the vanila version.}
%Thanks to the prefix property of the tree representable function $\tree$, at most one of $\tree([\trace_1,\dots,\trace_k])$ is non-zero.
Thanks to the prefix property of the tree representable function $\tree$, $\tree(\range{\enta}{1}{k})$ is non-zero for at most one $k \in \set{1, \cdots, \len{\enta}}$.
We call them truncations as they can be represented as finite trees of $\tree$ of depth $n$.
\cm{Draw tree}
\fi

We define the \defn{extended auxiliary kernel} $\exauxkernel:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} \auxspace^n$ which given an entropy trace $\enta \in \entspace^n$ with
$\traceb \in \instances{\enta} \cap \support{\tree}$, returns an auxiliary variable $\auxa$ where the first $\len{\traceb}$-th components of $\auxa$ has distribution $\nauxkernel{\len{\traceb}}(\range{\enta}{1}{\len{\traceb}}, \placeholder)$ and the rest of the components has the stock distribution $\measure{\auxspace}$.
Formally,
\[
  \exauxkernel: (\enta, \auxseta) \mapsto
  \begin{cases}
    \expandint{\auxseta}{\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}{\measure{\auxspace^{n}}}{\auxa} & \text{if } \traceb \in \instances{\enta} \cap \support{\tree} \text{ and } k = \len{\traceb} \\
    \measure{\auxspace^n}(\auxseta) & \text{otherwise.}
  \end{cases}
\]

\subsection{Algorithm}

Here we show how NP-iMCMC with hybrid parameter space generates a Markov chain by iterating \cref{alg: NP-iMCMC with hybrid parameter space}.

% \cref{alg line: fill start,alg line: fill end}
Line 3 to 10 in \cref{alg: NP-iMCMC with hybrid parameter space} pairs each value in the input trace $\traceb_0$ with a randomly drawn ``partner'' of the other type to an entropy-pair, resulting in an entropy trace $\enta_0$.
After that, Line 11 to 23 is the standard NP-iMCMC method as shown in \cref{sec: np-imcmc}.

\iffalse
\lo{NOTE: $\enta, \enta_0, \entb : \entspace^n$, $\entspace := \Real \times \Bool$ | $\traceb_0, \traceb : \traces := \bigcup_{n\in\Nat} (\Real \cup \Bool)^n$ | $\auxa, \auxa_0 : \auxspace^n$ \\
$\tree:\traces \to \pReal$ | $\trunc{n}:\ \entspace^n \rightarrow \pReal$ |
%$\auxkernel{n}: \entspace^n \times \algebra{\auxspace^n} \to \pReal$ | \\
$\ninvo{n}: \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n$ | $\NPempty(\cdot,\tree) : \entspace^n \to \traces$}
\cm{Now we have\\
  $\auxkernel{n}: \entspace \times \algebra{\auxspace} \to \pReal$ | %\\
  $\auxpdf{n}: \entspace \times \auxspace \to \pReal$ | %\\
  $\nauxkernel{n}: \entspace^n \times \algebra{\auxspace^n} \to \pReal$ | %\\
  $\nauxpdf{n}: \entspace^n \times \auxspace^n \to \pReal$ |
}
\fi
%\lo{The flow diagram (\cref{fig: flow diagram of np-imcmc}) is helpful!}

\begin{algorithm}
\caption{NP-iMCMC with hybrid parameter space}
\label{alg: NP-iMCMC with hybrid parameter space}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0 : \traces$,
    tree representable function $\tree :\traces \to \pReal$,
    family of involutions $\set{\ninvo{n} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$
    family of auxiliary kernels $\set{\nauxkernel{n} : \entspace^n \kernelto \auxspace^n}_n$ }
  \STATE \Output{Next sample $\traceb : \traces$}
  % \BlankLine
  \STATE $\enta_0 = \emptytrace$ \label{alg line: fill start}
  \FOR{$i = 1$ to $\len{\traceb_0}$}
    \IF{$\seqindex{\traceb_0}{i} \in \Real$}
      \STATE $\boola \sim \measure{\Bool}$; $\enta_0 = \enta_0 \concat [(\seqindex{\traceb_0}{i}, \boola)] $
    \ELSE[$\seqindex{\traceb_0}{i} \in \Bool$]
      \STATE $\reala \sim \measure{\Real}$; $\enta_0 = \enta_0 \concat [(\reala, \seqindex{\traceb_0}{i})] $
    \ENDIF
  \ENDFOR \label{alg line: fill end}
  % \COMMENT{$\enta_0$ is the entropy trace formed from $\traceb_0$ by pairing each value with randomly drawn ``partner''}
  \STATE $\auxa_0 \sim \cauxkernel{\len{\enta_0}}(\enta_0, \placeholder)$
  % \COMMENT{sample a value $\auxa_0 \in \auxspace^n$ from the cumulative auxiliary kernel $\cauxkernel{n}$ applied to $\enta_0$ (\cref{np-imcmc step: aux sample})}
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  % \COMMENT{compute the new state $(\enta,\auxa)$ by applying the involution $\ninvo{n}$ to the \emph{initial state} $(\enta_0,\auxa_0)$ where $n = \len{\enta_0}$. (\cref{np-imcmc step: involution})}
  \WHILE{$\enta \not\in\support{\extree} $}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % $\auxelem \sim \nauxkernel{\len{\enta_0}+1}(\entelem, \placeholder)$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    \label{line: Vanilla NP-iMCMC extend initial state}
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {\extree{(\enta)}\cdot\exauxpdf(\enta, \auxa)}
      {\extree{(\enta_0)}\cdot\exauxpdf(\enta_0, \auxa_0) }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta_0}}(\enta_0, \auxa_0)})}\bigg\}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\traceb \in \instances{\enta} \cap \support{\tree}$
  \ELSE
    \STATE \Return $\traceb \in \instances{\enta_0} \cap \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\cm{Put some comments into \cref{alg: NP-iMCMC with hybrid parameter space}}

% Flow diagram for np-imcmc
\iffalse
\begin{tikzpicture}[node distance = 3cm, scale=0.8, every node/.style={scale=0.8}]
  % Place nodes
  \node [] (input) {};
  % \node [block, below of=input, node distance = 1.5cm] (fill) {fill $\traceb_0$};
  \node [block, below of=input, node distance = 2cm] (aux)
    {Sample auxiliary variable $\auxa_0$ (\cref{line: Vanilla NP-iMCMC initialise aux var})};
  \node [block, below of=aux, node distance = 3.5cm] (inv)
    {Run involution $\ninvo{\len{\enta_0}}$ (\cref{line: Vanilla NP-iMCMC run involution,line: Vanilla NP-iMCMC loop run involution})};
  \node [decision, below of=inv] (good)
    {$\trunc{\len{\enta}}(\enta) > 0$? (\cref{line: Vanilla NP-iMCMC loop start})};
  \node [block, right of=good, yshift=1.5cm] (extend)
    {Extend initial state $(\enta_0,\auxa_0)$ with randomly drawn values (\cref{line: Vanilla NP-iMCMC extend initial state})};
  \node [draw=blue, algblock, fit= (inv) (good) (extend),
    label=north:{\hspace{2cm} \color{blue} Proposal (\cref{line: Vanilla NP-iMCMC run involution} to \cref{line: Vanilla NP-iMCMC loop end})}] (np-inv) {};
  \node [block, below of=good, node distance = 4cm] (mh)
    {Compute acceptance ratio (\cref{line: Vanilla NP-iMCMC acceptance})};
  \node [block, below of=mh] (empty)
    {Accept $\range{\enta}{1}{k}$ where $\tree(\range{\enta}{1}{k}) > 0$ with probability $P$};
  \node [right of=empty,node distance = 2.5cm] (output) {};

  % Draw edges
  \path [line] (input) edge node [label={0:$\enta_0 := \traceb_0$}] {} (aux);
  \path [line] (aux) edge node [label={10:$(\enta_0,\auxa_0)$}] {} (inv);
  \path [line] (inv) edge node [label=0:{$(\enta,\auxa)$}] {} (good);
  \path [line] (good) -| node [label={0:$(\enta_0,\auxa_0)$}] {} (extend);
  \path [line] (extend) |- node [label={0:$(\enta_0,\auxa_0)$}] {} (inv);
  \path [line] (good) -- node [label={0:$(\enta,\auxa)$ and $(\enta_0,\auxa_0)$}] {} (mh);
  \path [line] (mh) -- node [label={0:$P$}] {} (empty);
  \path [line] (empty) -- node [label=above:{$\traceb$}] {} (output);
\end{tikzpicture}
\fi

\subsection{Correctness}
\label{app: correctness}

In this section,
we show that the NP-iMCMC algorithm with hybrid parameter space is correct, in the sense that the Markov chain generated by iterating \cref{alg: NP-iMCMC with hybrid parameter space} converges to the target distribution, specified by
\begin{align*}
  {\tdist:}\
  {\Sigma_{\traces}}& \longrightarrow {\pReal} \\
  {U} & \longmapsto {\frac{1}{Z}\shortint{U}{\tree}{\measure{\traces}}}
  \qquad\text{where }
  Z := \shortint{\traces}{\tree}{\measure{\traces}}.
\end{align*}
% \lo{I.e.~we prove two results: (1) $\nu$ is an (the?) invariant distribution of the Markov chain induced by \cref{alg: NP-iMCMC with hybrid parameter space}; (2) The induced Markov chain converges to $\nu$ i.e.~for all $\state$, $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$ with $\norm{\cdot}$ denoting total variation distance.}
We do this by proving two statements:

\begin{restatable}[Invariant]{lemma}{invariant}
  \label{lemma: marginalised distribution is the target distribution}
  Given \allvass{}, $\tdist$ is the invariant distribution of the Markov chain generated by iterating \cref{alg: NP-iMCMC with hybrid parameter space}.
\end{restatable}

\begin{restatable}[Convergence]{theorem}{convergence}
% \begin{theorem}
  \label{thm: np-imcmc correct}
  Given \allvass{} and \allcass{}, the Markov chain generated by iterating \cref{alg: NP-iMCMC with hybrid parameter space} converges to the target distribution $\tdist$,
  i.e.~for all $\state$, $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$ with $\norm{\placeholder}$ denoting total variation distance.
% \end{theorem}
\end{restatable}

We start with some propositions about the tree representable function and its extension.

\begin{proposition}
  \label{prop: AST weight function iff AST truncations}
  Let $\tree$ be an almost surely terminating (\cref{vass: almost surely terminating tree}) tree representable function.
  Then its extension $\extree$ satisfies the following.
  \begin{enumerate}
    \item $\measure{\entspace^n}{(\nsupport{n}{\trunc{n}})}\to 1$ as $n\to\infty$.

    % \item $\measure{\entspace^\Nat}(\set{\enta \in \entspace^\Nat \mid
    % \exists k \in \Nat\ .\ \extree(\range{\enta}{1}{k}) > 0}) = 1$.
    % \item For almost all infinite sequences $\enta \in \entspace^{\Nat}$,
    % there exists $k \in \Nat$ where $\range{\enta}{1}{k} \in \support{\trunc{k}}$, and

    \item $\measure{\entspace^n}{(\entspace^n\setminus \support{\trunc{n}})}\to 0$ as $n\to\infty$.
  \end{enumerate}
\end{proposition}

\begin{proof}
  \begin{enumerate}
    \item
    \cm{Extend proof for hybrid entropy space.}

    For each $n\in\Nat$, we can write the set $\nsupport{n}{\trunc{n}}$ on $\entspace^n$ as
    $\bigcup_{i=1}^n \nsupport{i}{\tree} \times \entspace^{n-i} $.
    Since $\measure{\entspace^n}$ is probabilistic, we have
    $
    \measure{\entspace^n}(\nsupport{n}{\trunc{n}})
    = \sum_{i=1}^n \measure{\entspace^n}(\nsupport{i}{\tree} \times \entspace^{n-i})
    = \sum_{i=1}^n \measure{\entspace^i}(\nsupport{i}{\tree})
    = \measure{\traces}(\bigcup_{i=1}^n \nsupport{i}{\tree}).
    $
    Moreover, $\tree$ is almost surely terminating, so
    \begin{align*}
      \lim_{n\to\infty} \measure{\entspace^n}(\nsupport{n}{\trunc{n}})
      & = \lim_{n\to\infty} \measure{\traces}(\bigcup_{i=1}^n \nsupport{i}{\tree})
       = \lim_{n\to\infty} \sum_{i=1}^n  \measure{\traces}(\nsupport{i}{\tree})
       = \sum_{i=1}^{\infty} \measure{\traces}(\nsupport{i}{\tree}) \\
      & = \measure{\traces}(\bigcup_{i=1}^{\infty} \nsupport{i}{\tree}) \tag{$\measure{\traces}$ is countably additive} \\
      & = \measure{\traces}(\support{\tree}) \\
      & = 1 \tag{$\tree$ is almost surely terminating}
    \end{align*}

    % old proofs
    \iffalse
    Assume not, i.e.~there is a non-null set $\entseta \subseteq \entspace^\Nat$ where
    for all $\enta \in \entseta$ and all $k \in\Nat$, $\range{\enta}{1}{k} \not\in \support{\extree}$. Hence, $\range{\enta}{1}{k} \not\in\support{\tree} = \tertraces $.

    Note that since $\tree$ is AST, for almost all $\enta \in \entspace^{\Nat}$ there exists $k_{\enta} \in \Nat$ where
    $\range{\enta}{1}{k_{\enta}}\in\maxtraces $, i.e.~$\range{\enta}{1}{k_{\enta}}$ is the trace that the program takes to fill all the drawn values of sample and no more samples are called after that.

    Let $\entsetb_n := \set{\enta\in\entseta \mid k_{\enta} = n}$ be disjoint subsets of $\entseta$.
    Then, $\entseta = \bigcup_{n\in\Nat}\entsetb_n$ and
    $
    \measure{\entspace^\Nat}(\entseta)
    = \measure{\entspace^\Nat}(\bigcup_{n\in\Nat}\entsetb_n)
    = \sum_{n\in\Nat} \measure{\entspace^\Nat}(\entsetb_n) > 0.
    $
    So, there exists $n\in\Nat$ such that
    $\measure{\entspace^\Nat}(\entsetb_n) > 0.$
    Now say there exists $\entsetc_i \in \algebra{\entspace} $ where $\prod_{i\in\Nat}\entsetc_i = \entsetb_n$.
    Then,
    $\measure{\entspace^\Nat}(\entsetb_n) =
    \measure{\entspace^\Nat}(\prod_{i\in\Nat}\entsetc_i) =
    \prod_{i\in\Nat}\measure{\entspace}(\entsetc_i) >
    0.$
    So, for each $i \in\Nat$ we have $\measure{\entspace}(\entsetc_i) > 0.$

    Let $\traceset := \set{\range{\enta}{1}{n}\in\traces \mid \enta\in\entsetb_n} $.

    Let $\traceset := \bigcup \set{\instances{\range{\enta}{1}{k}} \mid \enta\in\entseta, k \in\Nat} \subseteq \traces$.
    Then, for any $\traceb\in\traceset$, there exists $\enta \in \entseta$ and $k \in\Nat$ where $\traceb \in \instances{\range{\enta}{1}{k}}$ and $\trunc{k}(\range{\enta}{1}{k}) = 0$, which implies $\tree(\traceb) = 0$.

    To show that $\traceset$ is non-null, we can assume WLOG that $\entseta$ is of the form $\entsetb_1 \times \dots \times \entsetb_\ell \times \entspace^\Nat$ for some $\ell \in \Nat$ and non-null sets $\entsetb_i \in \algebra{\entspace}$ for $i =1,\dots,\ell$.
    Then, $A \supseteq \instances{\entsetb_1 \times \dots \times \entsetb_\ell} \supseteq \entsetb_1 \times \dots \times \entsetb_\ell$ is non-null in $\entspace^\ell$; and hence $A$ is non-null in $\traces$.

    \item Assume not, i.e.~there is a non-null set $\entseta \subseteq \entspace^\Nat$ such that for all $\enta \in \entseta$ and all $k \in\Nat$, $\range{\enta}{1}{k} \not\in \support{\trunc{k}}$.
    We will construct a non-null set $\traceset$ in $\traces$ where $\tree$ is zero everywhere on it.
    Let $\traceset := \bigcup \set{\instances{\range{\enta}{1}{k}} \mid \enta\in\entseta, k \in\Nat} \subseteq \traces$.
    Then, for any $\traceb\in\traceset$, there exists $\enta \in \entseta$ and $k \in\Nat$ where $\traceb \in \instances{\range{\enta}{1}{k}}$ and $\trunc{k}(\range{\enta}{1}{k}) = 0$, which implies $\tree(\traceb) = 0$.

    To show that $\traceset$ is non-null, we can assume WLOG that $\entseta$ is of the form $\entsetb_1 \times \dots \times \entsetb_\ell \times \entspace^\Nat$ for some $\ell \in \Nat$ and non-null sets $\entsetb_i \in \algebra{\entspace}$ for $i =1,\dots,\ell$.
    Then, $A \supseteq \instances{\entsetb_1 \times \dots \times \entsetb_\ell} \supseteq \entsetb_1 \times \dots \times \entsetb_\ell$ is non-null in $\entspace^\ell$; and hence $A$ is non-null in $\traces$.
    \fi

    \item Since $\measure{\entspace^n}$ is probabilistic, we have
    $
    \lim_{n\to\infty} \measure{\entspace^n}(\entspace^n \setminus \nsupport{n}{\trunc{n}})
    = \lim_{n\to\infty} \big( \measure{\entspace^n}(\entspace^n) - \measure{\entspace^n}(\nsupport{n}{\trunc{n}})\big)
    = \lim_{n\to\infty} \big( 1 - \measure{\entspace^n}(\nsupport{n}{\trunc{n}})\big)
    = 1 - \lim_{n\to\infty}\measure{\entspace^n}(\nsupport{n}{\trunc{n}})
    = 1
    $.

    % old proof
    \iffalse
    \item Assume not, i.e.~$\measure{\entspace^n}{(\entspace^n\setminus \support{\trunc{n}})}\not\to 0$ as $n\to\infty$.
    Let $\entseta := \bigcap\set{ \entspace^k\setminus \support{\trunc{k}} \times \entspace^\Nat \mid k\in\Nat} \subseteq \entspace^\Nat$.
    Then, $\entseta$ is non-null as
    $\measure{\entspace^\Nat}(\entseta)
    = \lim_{k\in\infty} \measure{\entspace^\Nat}(\entspace^k\setminus \support{\trunc{k}} \times \entspace^\Nat)
    = \lim_{k\in\infty} \measure{\entspace^k}(\entspace^k\setminus \support{\trunc{k}})
    \not= 0$.
    Hence $\entseta$ is non-null, contradicting part (1).
    \fi
  \end{enumerate}
\end{proof}

With the result in \cref{prop: AST weight function iff AST truncations}, the algorithm (\cref{alg: NP-iMCMC with hybrid parameter space}) almost surely terminates.

\begin{restatable}{lemma}{vAST}
  \label{lemma: np-imcmc step almost surely terminates}
  A step of NP-iMCMC realised by \cref{alg: NP-iMCMC with hybrid parameter space} almost surely terminates.
\end{restatable}

\subsection{Invariant State Distribution}

Henceforth, we assume that the tree representable function $\tree$ is integrable (\cref{vass: integrable tree}) and almost surely terminating (\cref{vass: almost surely terminating tree}), the family of involutions $\set{\ninvo{n}}_n$ is partially block diagonal (\cref{vass: partial block diagonal inv}).
 % and the %family of
% auxiliary kernels $\set{\auxkernel{n}}_n$ are positive everywhere (\cref{cass: everywhere positive aux density}).

In \cref{alg: NP-iMCMC with hybrid parameter space}, we traverse the state (a entropy-auxiliary pair) instead of the sample to better explore the target distribution using involutions.
We now define the \defn{state distribution} $\sdist$ and prove that it is invariant against the Markov chain.

\changed[lo]{Recall that $\states := \bigcup_{n\in\Nat} (\entspace^n \times \auxspace^n)$.}
Let $\sdist$ be a distribution on $\states$ with density $\spdf$ (with respect to $\smeasure$) given by
\begin{align} \label{eq: defn of state distribution}
  \spdf(\enta,\auxa) :=
  \begin{cases}
    \frac{1}{Z} \trunc{\len{\enta}}(\enta) \cdot
    \exauxkernel(\enta, \auxa)
    % \prod_{i=1}^{\len{\enta}} \nauxpdf{i}(\seqindex{\enta}{i},\seqindex{\auxa}{i})
    & \text{if }(\enta,\auxa)\in \validstates \\
    {0} & \text{otherwise}
  \end{cases}
\end{align}
where
$Z := \shortint{\states}{\tree}{\measure{\states}}$ is the normalising constant and
$\validstates$ is %a subset of $\states$ which contains all valid states.
\changed[lo]{the subset of $\states$ consisting of all \emph{valid states}.}
We say a state $(\enta,\auxa)$ is \defn{valid} if
\begin{enumerate}[1.]
  \item $\enta \in \support{\trunc{\len{\enta}}}$, and
  \item $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$ implies $\enta' \in\support{\trunc{\len{\enta}}}$, and
  \item $(\range{\enta}{1}{k},\range{\auxa}{1}{k})\not\in \validstates$ for all $k <\len{\enta}$.
\end{enumerate}
%Valid states are the states when applied to involution $\ninvo{\len{\enta}}$ does not ``fall beyond'' the support of $\trunc{\len{\enta}}$.
\changed[lo]{Intuitively, valid states are the states which, when transformed by the involution $\ninvo{\len{\enta}}$, (the first component of which) does not ``fall beyond'' the support of $\trunc{\len{\enta}}$.}

We write $\validstates_n := \validstates \cap (\entspace^n \times \auxspace^n)$ to denote the the set of all $n$-dimensional valid states.
The following proposition shows that involutions preserve the validity of states.

\begin{proposition}
  \label{prop: valid states are preserved by involutions}
  $\ninvo{n}$ sends $\validstates_n$ to $\validstates_n$.
  i.e.~If $(\enta,\auxa) \in \validstates$ and $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$
  then $(\enta',\auxa') \in \validstates$.
\end{proposition}

\begin{proof}
  (1) $\enta' \in \support{\trunc{\len{\enta'}}}$ and (2) $(\enta'',\auxa'') = \ninvo{\len{\enta'}}(\enta',\auxa')$ implies $\enta'' \in\support{\trunc{\len{\enta}}}$ are immediate as $\ninvo{\len{\enta}}$ is involutive and $(\enta,\auxa)$ is a valid state.
  We prove (3) by induction on $\len{\enta}$, i.e.~$(\enta,\auxa) \in \validstates$ and $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$ implies
  $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k})\not\in \validstates$ for all $k <\len{\enta}$.

  The base case where $\len{\enta} = 1$ trivially holds.
  Assuming the statement holds for all $(\entb,\auxb) \in \validstates$ where $\len{\entb} < \len{\enta}$ and
  for contradiction that there exists some $k < \len{\enta}$ where
  $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k})\in \validstates$.
  Then since $\ninvo{\len{\enta}}$ is an involution, $\ninvo{\len{\enta}}(\enta',\auxa') = (\enta,\auxa)$.
  Moreover $\range{\enta'}{1}{k} \in \support{\trunc{k}}$ and applying \cref{vass: partial block diagonal inv} gives $\ninvo{k}(\range{\enta'}{1}{k},\range{\auxa'}{1}{k}) = (\range{\enta}{1}{k},\range{\auxa}{1}{k})$.
  By inductive hypothesis, $(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \validstates$
  which contradicts with the fact that $(\enta,\auxa)$ is a valid state.
\end{proof}

Since the the entropy component of all valid states must be supported by the corresponding truncation, the set of valid states can be written as
\[
  \validstates =
  \bigcup_{m=1}^{\infty}
  \{
    (\enta,\auxa) \in \validstates_m \mid
    \enta \in \support{\trunc{\len{\enta}}},
    \auxa \in \auxspace^m
  \}.
\]
Moreover by definition, the entropy component $\enta$ of a valid state must be in the support of the extension $\extree$ and, as shown in \cref{app: hybrid entropy space}, can be partitioned into three traces.
Hence the state distribution $\sdist$ can be written as
\begin{align} \label{eq: state distribution}
  \sdist: U \mapsto
  &
  \expandint{U}{
  [(\enta,\auxa) \in \validstates] \cdot
  \frac{1}{Z} \trunc{\len{\enta}}(\enta) \cdot \exauxpdf(\enta,\auxa)
  }{\smeasure}{(\enta,\auxa)} \nonumber \\
  & =
  \sum_{n=1}^{\infty}
  \expandint{\auxspace^n}{
  \expandint{\entspace^n}{
  [(\enta,\auxa) \in U \cap \validstates] \cdot
  \frac{1}{Z} \trunc{n}(\enta) \cdot \exauxpdf(\enta,\auxa)
  }{\measure{\entspace^n}}{\enta}
  }{\measure{\auxspace^n}}{\auxa}
  \nonumber \\
  & =
  \displaystyle
  \sum_{n=1}^{\infty}
  \int_{\auxspace^n}
  \int_{\traces}
  \int_{\traces}
  \int_{\traces}
  [(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa) \in U \cap \validstates]
  \frac{1}{Z} \tree(\traceb_1) \cdot
  \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa)\
  \nonumber\\
  & \displaystyle
  \quad
  {\measure{\traces}}{(\dif(\traceb_3))}\
  {\measure{\traces}}{(\dif(\traceb_2))}\
  {\measure{\traces}}{(\dif\traceb_1)}\
  {\measure{\auxspace^n}}{(\dif\auxa)}
\end{align}

\subsubsection{Invariant distribution}
\label{par: invariant}
% definition of transition kernel

Say there is an encoding $\church{\placeholder}$ for the auxiliary space $\auxspace$ in SPCF. i.e.~there is a type $\church{\auxspace}$ in SPCF such that for each $\auxa \in \auxspace$, there is a unique SPCF program $\church{\auxa}$ with type $\church{\auxspace}$.

Following the Church encodings of pairs and lists in SPCF as discussed in \cref{sec: church encodings},
we can extending $\church{\placeholder}$ to represent a state $(\enta,\auxa) \in \states$ in SPCF as
\[
\church{(\enta,\auxa)}
:=
\anbr
{[\anbr{\pcf{\seqindex{(\seqindex{\enta}{1})}{1}},\pcf{\seqindex{(\seqindex{\enta}{1})}{2}}}, \dots
\anbr{\pcf{\seqindex{(\seqindex{\enta}{\len{\enta}})}{1}},\pcf{\seqindex{(\seqindex{\enta}{\len{\enta}})}{2}}}],
[\church{\seqindex{\auxa}{1}}, \dots,
\church{\seqindex{\auxa}{\len{\enta}}}]}
\]
of type $\tystate := \typair{\tylist{\typair{\tyreal}{\tybool}}}{\tylist{\church{\auxspace}}}$.
Take a SPCF term $\set{x:\tystate} \vdash \terma:\tystate $,
its \defn{transition kernel}
$\transkernel{\terma}: \states \kernelto \states$ is given by
\begin{align*}
  \transkernel{\terma} ({\state},\stateset) := \shortint{\inv{v_{\terma}({\state},-)}(\stateset)}{\weightfn{\terma[\church{\state}/x]}}{\tmeasure}
\end{align*}
where the function $v_{\terma} :\states \times \traces \to \states$ is such that
$\church{v_{\terma}(\state,\traceb)} = \valuefn{\terma[\church{\state}/x]}(\traceb) $.
Intuitively,
$\transkernel{\terma} ({\state},\stateset)$ gives the probability of $\terma$ returning a state in $\stateset$ with the current state $\state$.

We say a distribution $\mu$ on states $\states$ is \defn{invariant} w.r.t.~a SPCF term $\set{x:\tystate} \vdash \terma:\tystate $ if
$\mu$ is not altered after applying $\terma$, formally:
$\expandint{\states}{\transkernel{\terma}(\state,\stateset)}{\mu}{\state} = \mu(\stateset)$.

\subsubsection{Equivalent Program}

Though the NP-iMCMC step with hybrid parameter space (\cref{alg: NP-iMCMC with hybrid parameter space}) traverses state, it takes and returns \emph{samples} $\traceb \in \traces$. This makes it awkward to ask the question whether the state distribution $\sdist$ is invariant against it.
Instead, we consider a program (\codeinline{eNPiMCMCstep} in \cref{code: e np-imcmc}) which takes and returns \emph{states} and prove $\sdist$ is invariant against it (\cref{lemma: e-np-imcmc invariant}). After that, we show how this would implies that the target distribution $\tdist$ on $\traces$ is invariant against \cref{alg: NP-iMCMC with hybrid parameter space}.

Program \codeinline{eNPiMCMCstep} in \cref{code: e np-imcmc} is similar to the NP-iMCMC step with hybrid parameter space (\cref{alg: NP-iMCMC with hybrid parameter space}).
It takes an initial state \codeinline{(x0,v0)},
a target density function \codeinline{w},
a family of involutions \codeinline{inv} where \codeinline{inv(x,v)} gives the result of $\ninvo{n}$ applied to the state \codeinline{(x,v)} for the $n$-length trace \codeinline{x},
% with extensions $\codeinline{ext}$ where $\codeinline{ext(y,u)}$ gives the value of $\extfn$ applied to the pair $\codeinline{(y,u)}$,
a family of auxiliary kernels \codeinline{aux} where \codeinline{aux(x)} samples from the distribution $\nauxkernel{n}(x)$ for the $n$-length trace \codeinline{x},
% a family of auxiliary kernels \codeinline{aux} where \codeinline{aux[i](e)} samples from the distribution $\nauxkernel{i}(e)$ for the element \codeinline{e}.
their densities \codeinline{pdfaux} where \codeinline{pdfaux(x,v)} gives the result of $\nauxpdf{n}$ applied to the state \codeinline{(x,v)}, and
a stock auxiliary measure \codeinline{auxstock} which samples from the auxiliary stock measure $\measure{\auxspace}$.

\codeinline{eNPiMCMCstep} then generates the next state \codeinline{(x,v)} in three steps --- Initialisation, Involution and Acceptance. We will have a closer look at each of them later.

Helper functions \codeinline{extree(w)}, \codeinline{expdfaux}, \codeinline{instance} and \codeinline{accept} are given in \cref{code:helper}.
We assume the following primitive functions are implemented:
\codeinline{normal} is the sampler that draws from the standard normal distribution $\Gau$.
\codeinline{uniform} is the sampler that draws from the standard uniform distribution $\Uni(0,1)$.
\codeinline{coin} is the fair coin.
\codeinline{grad(f,x)} gives the gradient of the function \codeinline{f} at \codeinline{x}.
Standard primitives such as \codeinline{sum(list)}, \codeinline{abs(x)}, \codeinline{type(t)}, and \codeinline{product(list,n)}\footnote{\codeinline{product(list,n)} gives the list of all (ordered) permutation of \codeinline{n} elements of over the set \codeinline{list}.} are assumed to be implemented.

\input{section/proof-code}

\begin{remark}
  Programs in \cref{code: e np-imcmc,code:helper} are given in Python syntax, but they can be translated into SPCF via Church encodings as discussed in \cref{sec: church encodings,par: invariant}.
\end{remark}

\subsubsection{Initialisation (Step 1)}

Assuming the initial state \codeinline{(x0,v0)} is valid, the initiation step in \codeinline{eNPiMCMCstep}
% first defines the extension of \codeinline{w} and
first finds the instance \codeinline{t0} of \codeinline{x0} which is in the support of \codeinline{w}.
Note that this step is deterministic and does not affect the transition kernel.

After that, it constructs a state \codeinline{(x0,v0)} by
first sampling partners for each value in the trace \codeinline{t0} to form a entropy trace \codeinline{x0} of the same length. Say \codeinline{t} are the samples drawn, then we can write the trace \codeinline{x0} as \codeinline{zip(t0,t)}.
Next, it samples the auxiliary variable \codeinline{v0} from \codeinline{aux(x0)}.

Finally, it finds a \emph{valid} state by keep appending \codeinline{x0} with samples from \codeinline{normal} and \codeinline{coin} and auxiliary element \codeinline{v0} with samples from the auxiliary stock measure \codeinline{auxstock} until the state \codeinline{(x0,v0)} is valid.
If \codeinline{t'} are the samples drawn for the entropy trace, then we can write \codeinline{x0} as \codeinline{zip(t0,t)+t'}.

The transition kernel of this step is then
\begin{align*}
  \transkernel{1}((\enta_0,\auxa_0),U)
  =
  \sum_{n=1}^{\infty}
  \int_{\auxspace^n}
  \int_{\traces}
  \int_{\traces}
  &
  [(\zip(\traceb_0, \traceb) \concat\traceb' ,\auxa) \in U \cap \validstates]
  \nonumber \\
  & \exauxpdf(\zip(\traceb_0, \traceb) \concat\traceb' ,\auxa)\
  {\measure{\traces}}{(\dif(\traceb'))}\
  {\measure{\traces}}{(\dif(\traceb))}\
  {\measure{\auxspace^n}}{(\dif\auxa)}
\end{align*}
if $(\enta_0,\auxa_0) \in \validstates$ and $\traceb_0 \in \instances{\enta_0} \cap \support{\tree}$; and $0$ otherwise.

\begin{proposition}
  \label{prop: step 1 is probabilistic}
  For any $(\enta_0,\auxa_0) \in \validstates$, we have
  $\transkernel{1}((\enta_0,\auxa_0),\states) = 1$.
\end{proposition}

\begin{proof}
  Given all inputs to \codeinline{eNPiMCMC} with the initial state $\codeinline{(x0,v0)}:= \church{(\enta_0,\auxa_0)}$,
  step 1 of \codeinline{eNPiMCMC} can be described by a closed SPCF term that does not contain $\score{\placeholder}$ as a subterm (following \cref{app: primitive functions,sec: church encodings}) and thus by \cref{lemma: np-imcmc step almost surely terminates} terminates almost surely.
  By \cref{prop: AST SPCF term gives probability measure}, the value measure of this term must be probabilistic. Hence
  $\transkernel{1}((\enta_0,\auxa_0),\states) = 1$.
\end{proof}

\begin{proposition}
  \label{prop: step 1 is invariant}
  The state distribution $\sdist$ is invariant against step 1 of \codeinline{eNPiMCMC}.
\end{proposition}

\begin{proof}
  We aim to show: \(\expandint{\states}{\transkernel{1}((\enta_0,\auxa_0),U)}{\sdist}{(\enta_0,\auxa_0)} = \sdist(U)\) for any measurable set $U \in \Sigma_{\states}$.
  (Changes are underlined for readability.)
  \begin{calculation}
    \displaystyle
    \expandint{\underline{\states}}{\transkernel{1}((\enta_0,\auxa_0),U)}{\sdist}{(\enta_0,\auxa_0)}
    %
    \step[=]{
      $\transkernel{1}((\enta_0,\auxa_0),U) = 0$ for all $(\enta_0,\auxa_0) \not\in \validstates$
    }
    \displaystyle
    \underline{\int_{\validstates}}\ {\transkernel{1}((\underline{\enta_0},\auxa_0),U)}\
    \underline{{\sdist}{(\dif(\enta_0,\auxa_0))}}
    %
    \step[=]{Formulation of $\sdist$ in \cref{eq: state distribution} writing $\enta_0$ as $\zip(\traceb_1, \traceb_2) \concat\traceb_3$ where $\tree(\traceb_1) > 0$}
    \displaystyle
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}\
    \int_{\traces}\
    \int_{\traces}\
    \int_{\traces}\
    \underline{\transkernel{1}((\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0),U)}\cdot
    \\
    \displaystyle
    \quad
    \Big(
    [(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0) \in \validstates] \cdot
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0)\Big)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}
    %
    \step[=]{Definition of $\transkernel{1}$}
    \displaystyle
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \Big(\displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa) \in U \cap \validstates]
    \\
    \qquad\qquad\qquad\qquad\qquad\qquad
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa)\
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    \Big)\cdot
    \\
    \displaystyle
    \quad
    [(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0) \in \validstates] \cdot
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0)\Big)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}
    %
    \step[=]{Rearranging}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \Big(\displaystyle
    \underline{
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0) \in \validstates] \cdot}
    \\
    \qquad\qquad\qquad\qquad\qquad\qquad
    \underline{
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\traceb_3 ,\auxa_0)\Big)\
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}}
    \Big)\cdot
    \\
    \displaystyle
    \quad
    [(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa) \in U \cap \validstates]
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    %
    \step[=]{$(\hat{\enta_0}, \hat{\auxa_0})$ is an arbitrary valid state where $\traceb_0 \in \instances{\hat{\enta_0}}$}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \underline{\transkernel{1}((\hat{\enta_0}, \hat{\auxa_0}), \validstates)}\cdot
    \\
    \displaystyle
    \quad
    \Big(
    [(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa) \in U \cap \validstates]
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    %
    \step[=]{By \cref{prop: step 1 is probabilistic}, $\transkernel{1}((\hat{\enta_0},\hat{\auxa_0}),\validstates) = \transkernel{1}((\hat{\enta_0},\hat{\auxa_0}),\states) = 1$}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa) \in U \cap \validstates]
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\traceb_3' ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    \step[=]{Formulation of $\sdist$ in \cref{eq: state distribution} writing $\enta_0$ as $\zip(\traceb_1, \traceb_2') \concat\traceb_3'$ where $\tree(\traceb_0) > 0$}
    \sdist(U)
  \end{calculation}
\end{proof}

\subsubsection{Involution (Step 2) and Acceptance (Step 3)}

After constructing a valid state \codeinline{(x0,v0)}, \codeinline{eNPiMCMCstep} traverses the state distribution via the involution \codeinline{inv} to obtain a proposal state \codeinline{(x,v)}.
Like iMCMC samplers, the proposed state \codeinline{(x,v)} is accepted with probability specified by \codeinline{accept}.

The transition kernel for steps 2 is given by
\[
  \transkernel{2}(\state_0,U) =
  \begin{cases}
    {\accept(\state_0)\cdot[\ninvo{n}(\state_0) \in U] + (1-\accept(\state_0))\cdot [\state_0 \in U]}& \text{if }{\state_0 \in \validstates_n} \\
    {0}
    & \text{otherwise.}
  \end{cases}
\]
Note that the acceptance ratio $\accept$
for $(\enta_0,\auxa_0) \in \entspace^n \times \auxspace^n $ is
$$
% \accept(\enta_0,\auxa_0)
% :=
\min \set{1,
  \displaystyle
  \frac
    {\trunc{n}(\enta)\cdot \exauxpdf(\enta,\auxa) }
    {\trunc{n}(\enta_0)\cdot \exauxpdf(\enta_0,\auxa_0) } \cdot
  \abs{\det{\big(\grad{\ninvo{n}}(\enta_0,\auxa_0)\big)}}
}
= \min \set{1,
  \displaystyle
  \frac
    {\spdf(\enta,\auxa) }
    {\spdf(\enta_0,\auxa_0) } \cdot
  \abs{\det{\big(\grad{\ninvo{n}}(\enta_0,\auxa_0)\big)}}
}
$$
where $(\enta,\auxa) = \ninvo{n}(\enta_0,\auxa_0)$.

\begin{proposition}
  \label{prop: step 2 is invariant}
  The state distribution $\sdist$ is invariant against step 2 of \codeinline{eNPiMCMC}.
\end{proposition}

\begin{proof}
  We aim to show:
  $\expandint{\states}{\transkernel{2}(\state,U)}{\sdist}{\state} = \sdist(U)$
  for all $U \in \Sigma_{\states}$.

  First we notice that for any valid state $(\enta,\auxa) \in \validstates$ where $(\enta',\auxa') := \ninvo{n}(\enta,\auxa)$ and $n := \len{\enta}$, we have
  \begin{align*}
    & \accept(\ninvo{n}(\enta,\auxa))\cdot \spdf(\ninvo{n}(\enta,\auxa))\cdot \abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}} \\
    & = \accept(\enta',\auxa')\cdot \spdf(\enta',\auxa')\cdot \abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}
    \tag{$(\enta, \auxa) = \ninvo{n}(\enta', \auxa')$}
    \\
    & = \begin{cases}
      \multicolumn{2}{@{}l@{\quad}}{\frac
        {\spdf(\enta,\auxa)}
        {\spdf(\enta',\auxa')} \cdot
      \abs{\det{\big(\grad{\ninvo{n}}(\enta',\auxa')\big)}} \cdot
      \spdf(\enta',\auxa')\cdot \abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}} \\
      & \text{if }
      \frac
        {\spdf(\enta,\auxa) \cdot \abs{\det{(\grad{\ninvo{n}}(\enta',\auxa'))}}}
        {\spdf(\enta',\auxa')} < 1 \\
      \spdf(\enta',\auxa')\cdot \abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}} & \text{otherwise}
    \end{cases}
    % \tag{$\ninvo{n}$ is involutive and $\spdf(\enta,\auxa) = \trunc{n}(\enta)\cdot \nauxpdf{n}(\enta,\auxa)$}
    \tag{Differentiating $\ninvo{n} \circ \ninvo{n} = \id$ gives $\abs{\det{\big(\grad{\ninvo{n}}(\enta',\auxa')\big)}} = 1/\abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}$} \\
    & = \begin{cases}
      {\spdf(\enta,\auxa)}
      & \text{if }
      \frac
        {\spdf(\enta,\auxa)}
        {\spdf(\enta',\auxa') \cdot \abs{\det{(\grad{\ninvo{n}}(\enta,\auxa))}}} < 1 \\
      \spdf(\enta',\auxa')\cdot \abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}} & \text{otherwise}
    \end{cases}
    \\
    & = \accept(\enta,\auxa) \cdot \spdf(\enta,\auxa).
  \end{align*}

  Recall in \cref{prop: valid states are preserved by involutions} we have shown that $\ninvo{n}$ is an involution that maps $\validstates_n$ to itself for all $n\in\Nat$. Thus, $\ninvo{n}(\state) = \inv{\ninvo{n}}(\state)$ for all $\state \in \validstates_n$ and $\ninvo{n}(\validstates_n) = \validstates_n$.
  Hence, we have
  \begin{align*}
    &\expandint{\states}{\transkernel{2}(\state,U)}{\sdist}{\state} \\
    & =
    \expandint{\validstates}{\transkernel{2}(\state,U)}{\sdist}{\state}
    \tag{$\transkernel{2}(\state, U) = 0$ for all $\state \in \states\setminus\validstates$}
    \\
    & =
    \sum_{n=1}^{\infty} \expandint{\validstates_n}{\transkernel{2}(\state,U)\cdot \spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & =
    \shortint{U}{\spdf}{\smeasure}
    +
    \sum_{n=1}^{\infty}
    \bigg(
      \expandint{\validstates_n}{[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & \qquad\qquad\qquad\qquad
      -
      \expandint{\validstates_n}{[\state \in U \cap \validstates_n]\cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state}
    \bigg)\\
    & =
    \shortint{U}{\spdf}{\smeasure}
    +
    \sum_{n=1}^{\infty}
    \bigg(
      \expandint{\validstates_n}{[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & \qquad\qquad\qquad\qquad
      -
      \expandint{\validstates_n}{
      [\ninvo{n}(\state) \in U \cap \validstates_n]\cdot \accept(\ninvo{n}(\state)) \cdot\spdf(\ninvo{n}(\state)) \cdot
      \abs{\det{\big(\grad{\ninvo{n}}(\state)\big)}}
      }{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state}
    \bigg)
    \tag{$\accept(\ninvo{n}(\state))\cdot \spdf(\ninvo{n}(\state))\cdot \abs{\det{\big(\grad{\ninvo{n}}(\state)\big)}} = \accept(\state) \cdot \spdf(\state)$ for all $\state \in \validstates$}
    \\
    & =
    \shortint{U}{\spdf}{\smeasure}.
  \end{align*}
\end{proof}

Since the transition kernel $\transkernel{\cref{code: e np-imcmc}}$ of \codeinline{eNPiMCMCstep} is the composition of $\transkernel{1}$ and $\transkernel{2}$,
i.e.~$\transkernel{\cref{code: e np-imcmc}}(\state,U) := \int_{\states} \transkernel{2}(\state',U)\ \transkernel{1}(\state,\dif \state') $ for $\state \in \states$ and $U \in \algebra{\states}$,
and both $\transkernel{1}$ and $\transkernel{2}$ are invariant against $\sdist$ (\cref{prop: step 1 is invariant,prop: step 2 is invariant}), with \cref{prop: invariant is closed under composition} we conclude with the following lemma.

\begin{lemma}
  \label{lemma: e-np-imcmc invariant}
  $\sdist$ is the invariant distribution of the Markov chain generated by iterating \codeinline{eNPiMCMCstep}.
\end{lemma}

\subsection{Marginalised Markov Chains}

As discussed above, the Markov chain $\set{(\enta^{(i)},\auxa^{(i)})}_{i\in\Nat}$ on $\states$ generated by iterating \codeinline{eNPiMCMCstep} (which has invariant distribution $\sdist$) is \emph{not} the samples generated by \cref{alg: NP-iMCMC with hybrid parameter space}.
The chain we are in fact interested in is the \emph{marginalised} chain $\set{\marg(\enta^{(i)},\auxa^{(i)})}_{i\in\Nat}$ where the measurable function $\marg:\validstates \to \traces$ takes a valid state $(\enta,\auxa)$ and returns the instance of the entropy trace $\enta$ that is in the support of the tree representable function $\tree$.

In this section we show that this marginalised chain has the target distribution $\tdist$ as its invariant distribution.
Let $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}: \support{w} \kernelto {\traces}$ be the transition kernel of this marginalised chain, defined as $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\traceb, A) := \transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))$ where $\state \in \inv{\marg}(\set{\traceb})$
for $\traceb \in \traces$ and $A \in \algebra{\traces}$.

\begin{proposition}
  \label{prop: properties about marg}
  Writing $\validstates_{\leq n} := \bigcup_{k=1}^n \validstates_k$,
  we let $\sdist_n$ be a probability distribution on measurable space $\entspace^n \times \auxspace^n$
  \[
    \sdist_n(U) := \shortint{U}{\spdf_n}{\measure{\entspace^n \times \auxspace^n}}
    \quad
    \text{where }
    \spdf_n(\enta,\auxa) := \frac{1}{Z_n} \trunc{n}(\enta) \cdot \exauxpdf(\enta,\auxa)
  \]
  and $Z_n := \shortint{\entspace^n \times \auxspace^n}{\trunc{n}}{\measure{\entspace^n \times \auxspace^n}}$.
  \begin{enumerate}[1.]
    \item $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}$ is well-defined.

    \item $\transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(A)) = \transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\marg(\state),A)$ for all $\state \in \validstates$ and $A \in \algebra{\traces}$.

    \item $\sdist(\states \setminus {\validstates_{\leq n}}) \to 0$ as $n\to \infty$.

    \item $\exauxpdf(\enta, \auxa) = \expandint{\entspace \times \auxspace}{\exauxpdf(\enta \concat \enta', \auxa \concat \auxa')}{\measure{\entspace \times \auxspace}}{(\enta', \auxa')} $ for all $(\enta, \auxa) \in \validstates$.

    \item For $n \geq k$, $Z_k\cdot\sdist_k = Z_n\cdot {\proj{n}{k}}_*\sdist_n$ on $\validstates_k$.
    Recall $\proj{n}{k}(\enta,\auxa) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) $.

    \item $Z\cdot\sdist = Z_n\cdot g^{(n)}_*\sdist_n$ on ${\validstates_{\leq n}}$ where
    $g^{(n)} : \entspace^n \times \auxspace^{n}\partialto {\validstates_{\leq n}}$ such that
    $g^{(n)}(\enta,\auxa) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in {\validstates_{\leq n}}$.
  \end{enumerate}
\end{proposition}

\begin{proof}
  \begin{enumerate}[1.]

    \item Let $\traceb \in \traces$ and $A \in \algebra{\traces}$.
    For any $\state,\state' \in \inv{\marg}(\set{\traceb})$,
    $\transkernel{\cref{code: e np-imcmc}}(\state, U) = \transkernel{\cref{code: e np-imcmc}}(\state', U)$ since $\transkernel{1}$ applies $\marg$ to the input.

    \item Let $\state \in \validstates$ and $A \in \algebra{\traces}$. Then,
    $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\marg(\state),A) = \transkernel{\cref{code: e np-imcmc}}(\state',\inv{\marg}(A))$ for some $\state' \in \inv{\marg}(\set{\marg(\state)})$.
    Since $\state \in \inv{\marg}(\set{\marg(\state)})$ and by above, we have $\transkernel{\cref{code: e np-imcmc}}(\state',\inv{\marg}(A)) = \transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(A))$.

    \item First note that $\sdist$ is an invariant distribution and hence is probabilistic.
    The sum $\sum_{n=1}^{\infty} \sdist(\validstates_n)$ which equals $\sdist(\bigcup_{n=1}^{\infty} \validstates_n) = \sdist(\validstates)$ must converge.
    Moreover, $\sdist(\states \setminus \validstates) = \expandint{}{[\state \in (\states\setminus\validstates) \cap \validstates] \cdot \spdf(\state)}{\measure{\states}}{\state} = 0$.
    Hence
    $
    \sdist(\states \setminus {\validstates_{\leq n}})
    = \sdist(\validstates \setminus {\validstates_{\leq n}})
    = \sum_{i=n+1}^{\infty} \sdist(\validstates_i)
    \to 0
    $ as $n\to \infty$.

    \item Simple application.

    \item Let $U \in \algebra{\states}$ where $ U \subseteq {\validstates_k}$. Then,
    \begin{align*}
      & Z_n \cdot ({\proj{n}{k}}_*\sdist_n)(U) \\
      & = Z_n \cdot \sdist_n(\inv{{\proj{n}{k}}}{(U)}) \\
      & = \expandint{\entspace^n \times \auxspace^n}
      {[(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in U] \cdot Z_n \spdf_n(\enta,\auxa)}
      {\measure{\entspace^n \times \auxspace^n}}{(\enta,\auxa)} \\
      & = \expandint{\entspace^n \times \auxspace^n}{
        [(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in U] \cdot Z_k \spdf_k(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \cdot
        \frac{\exauxpdf(\enta,\auxa)}{\exauxpdf(\range{\enta}{1}{k},\range{\auxa}{1}{k})}
      }{\measure{\entspace^n \times \auxspace^n}}{(\enta,\auxa)} \\
      & =
      \int_{\entspace^k \times \auxspace^k}\
      [(\enta',\auxa') \in U] \cdot Z_k \spdf_k(\enta',\auxa') \cdot \\
      &\qquad
      \Big(\expandint{\entspace^{n-k} \times \auxspace^{n-k}}{
        \frac
          {\exauxpdf(\enta'\concat\enta'',\auxa'\concat\auxa'')}
          {\exauxpdf(\enta',\auxa')}
        % \prod_{j=1}^{n-k}\auxpdf{k+j}(\seqindex{\enta''}{j},\seqindex{\auxa''}{j})
      }{\measure{\entspace^{n-k} \times \auxspace^{n-k}}}{(\enta'',\auxa'')}\Big)
      \ {\measure{\entspace^k \times \auxspace^k}}{(\dif(\enta',\auxa'))} \\
      % & =
      % \int_{\entspace^k \times \auxspace^k}\
      % [(\enta',\auxa') \in U] \cdot Z_k \spdf_k(\enta',\auxa') \cdot \\
      % &\qquad
      % \Big(\expandint{\entspace^{n-k} \times \auxspace^{n-k}}{
      %   \auxpdf{n-k}(\enta'',\auxa'')
      % }{\measure{\entspace^{n-k} \times \auxspace^{n-k}}}{(\enta'',\auxa'')}\Big)
      % \ {\measure{\entspace^k \times \auxspace^k}}{(\dif(\enta',\auxa'))} \\
      & =
      \expandint{\entspace^k \times \auxspace^k}{
      [(\enta',\auxa') \in U] \cdot Z_k \spdf_k(\enta',\auxa')
      }{\measure{\entspace^k \times \auxspace^k}}{(\enta',\auxa')} \tag{$\auxpdf{j}$ are probabilistic} \\
      & =
      Z_k\sdist_k(U)
    \end{align*}
    \label{item: partial pointwise auxiliary kernel is used}

    \item Let $U \in \algebra{\states}$ where $ U \subseteq {\validstates_{\leq n}}$. Then,
    \begin{align*}
      Z\cdot \sdist(U)
      & = \expandint{U}{\extree(\enta)\cdot\exauxpdf(\enta, \auxa)}{\measure{\states}}{(\enta, \auxa)} \\
      & = \sum_{k=1}^n \expandint{U\cap\validstates_k}{\extree(\enta)\cdot\exauxpdf(\enta, \auxa)}{\measure{\entspace^k\times\auxspace^k}}{(\enta, \auxa)} \\
      & = \sum_{k=1}^n Z_k \cdot \sdist_k(U\cap \validstates_k) \\
      & = Z_n \sum_{k=1}^n {\proj{n}{k}}_* \sdist_n (U\cap \validstates_k) \tag{Part 5} \\
      & = Z_n \cdot \sdist_n (\bigcup_{k=1}^n
          \set{ (\enta,\auxa) \in \entspace^n \times \auxspace^n \mid (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in U\cap \validstates_k}) \\
      & = Z_n \cdot g^{(n)}_*\sdist_n (U).
    \end{align*}
  \end{enumerate}
\end{proof}


% \begin{lemma}
%   \label{lemma: marginalised distribution is the target distribution}
%   Given \allvass{}, $\tdist$ is the invariant distribution of the Markov chain generated by iterating \cref{alg: NP-iMCMC with hybrid parameter space}.
% \end{lemma}
\invariant*

\lo{Check: $\nu$ is the unique(?) invariant distribution of the induced Markov chain.}

%\lo{Note the standard result about existence and uniqueness of invariant distribution:}
\begin{proof}
  Assuming (1) $\tdist = \marg_*\sdist$ on $\traces$ and (2) $\tmeasure = \marg_*\smeasure$ on $\support{w}$, then for any $A \in \algebra{\traces}$,
  \begin{align*}
    \tdist(A) & = \marg_*\sdist(A) \tag{1} \\
    & = \expandint{\states}{\transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))}{\smeasure}{\state} \tag{\cref{lemma: e-np-imcmc invariant}} \\
    & = \expandint{\validstates}{\transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))}{\smeasure}{\state} \\
    & = \expandint{\validstates}{\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\marg(\state), A)}{\smeasure}{\state} \tag{\cref{prop: properties about marg}.2} \\
    & = \expandint{\support{\tree}}{\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}} (\traceb, A)}{\marg_*\smeasure}{\traceb} \\
    & = \expandint{\support{\tree}}{\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}} (\traceb, A)}{\tmeasure}{\traceb} \tag{2} \\
    & = \expandint{\traces}{\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}} (\traceb, A)}{\tmeasure}{\traceb}.
  \end{align*}
  It is enough to show (1) and (2).

  \begin{enumerate}[1.]
    \item
    Let $A \in \algebra{\traces}$ where $A \subseteq \nsupport{n}{\tree} $ and $\delta > 0$.
    Then partitioning $\inv{\marg}(A)$ using $\validstates_k$, we have {for sufficiently large $m$},
    \begin{align*}
      \marg_*\sdist(A)
      & = \sdist\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right)
        + \sdist\left(\bigcup_{k=m+1}^\infty \inv{\marg}(A)\cap \validstates_k\right) \\
      & < \frac{Z_m}{Z} \cdot
        g^{(m)}_*\sdist_m\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right) + \delta
      \tag{by \cref{prop: properties about marg}.3, \cref{prop: properties about marg}.5} \\
      & \leq \frac{Z_m}{Z} \cdot \sdist_m(
      \set{(\zip(\traceb, \traceb')\concat \entb, \auxa) \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}, \auxa \in \auxspace^m}
      ) + \delta \\
      & = \frac{1}{Z} \expandint{\set{\zip(\traceb, \traceb')\concat \entb \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}}}{
        \trunc{m}(\enta)\cdot
        \big(\expandint{\auxspace^m}{\exauxpdf(\enta,\auxa)}{\measure{\auxspace^m}}{\auxa}\big)
      }{\measure{\entspace^m}}{\enta}
      + \delta \\
      & = \frac{1}{Z} \expandint{A}{\tree(\traceb)}{\measure{\traces}}{\traceb}
      + \delta
      \tag{$A \subseteq \nsupport{n}{\tree}$}
      \\
      & = \tdist(A) + \delta.
    \end{align*}
    For any measurable set $A \in \Sigma_{\traces}$,
    we have
    $
    \marg_*\sdist(A)
    = \marg_*\sdist(A \cap \support{\tree})
    = \sum_{n=1}^\infty \marg_*\sdist(A \cap \nsupport{n}{\tree})
    \leq \sum_{n=1}^\infty \tdist(A \cap \nsupport{n}{\tree})
    = \tdist(A \cap \support{\tree})
    = \tdist(A)$.
    Since both $\tdist$ and $\sdist$ are {probability} distributions, we also have
    $\tdist(A) = 1 - \tdist(\traces \setminus A)
    \leq 1 - \marg_*\sdist(\traces \setminus A)
    = 1 - (1- \marg_*\sdist(A))
    = \marg_*\sdist(A)$.
    Hence
    $\marg_*\sdist = \tdist$ on $\traces$.

    \item
    Similarly, let $A \in \algebra{\traces}$ where $A \subseteq \nsupport{n}{\tree} $ and $\delta > 0$.
    Then by \cref{prop: properties about marg}.3, {for sufficiently large $m$}, we must have
    $\smeasure(\bigcup_{k=m+1}^\infty \validstates_k) = \smeasure(\validstates \setminus \validstates_{\leq m}) < \delta$.
    Hence,
    \begin{align*}
      & \marg_*\smeasure(A) \\
      & = \smeasure\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right)
        + \smeasure\left(\bigcup_{k=m+1}^\infty \inv{\marg}(A)\cap \validstates_k\right) \\
      & < \sum_{k=1}^m \measure{\entspace^{k}\times\auxspace^{k}} (\inv{\marg}(A)\cap \validstates_k) + \delta \\
      & = \sum_{k=1}^m \measure{\entspace^{m}\times\auxspace^{m}} (\set{(\enta,\auxa)\in \entspace^{m}\times\auxspace^m \mid (\enta^{1\dots k},\auxa^{1\dots k}) \in \inv{\marg}(A)\cap \validstates_k}) + \delta \\
      & = \measure{\entspace^{m}\times\auxspace^{m}} (\bigcup_{k=1}^m \set{(\enta,\auxa)\in \entspace^{m}\times\auxspace^m \mid (\enta^{1\dots k},\auxa^{1\dots k}) \in \inv{\marg}(A)\cap \validstates_k}) + \delta \\
      & \leq \measure{\entspace^{m}\times\auxspace^{m}}(\set{(\zip(\traceb, \traceb')\concat \entb, \auxa) \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}, \auxa \in \auxspace^m}) + \delta \\
      & = \tmeasure(A) + \delta.
    \end{align*}
    Then the proof proceeds as in (1). Note that since $\tree$ is AST, $\marg_*\measure{\states}(\support{\tree}) = \measure{\traces}(\support{\tree}) = 1$

  \end{enumerate}
\end{proof}

\cm{Still need revising!}

\subsection{Convergence}
\label{app: convergence}

Last but not least, we check for the convergence of the marginalised chain to the target distribution $\tdist$.

\begin{description}
  \item[\cass\label{cass: very strong irreducible}]
  $\ninvo{n}$ is \defn{very strong irreducible}.
  %i.e.~for all $n\in\Nat$, $\enta \in \entspace^n$ and $\entseta \in \algebra{\entspace^n}$ where $\enta \in \support{\trunc{n}} $ and $\tdist_n(\entseta) > 0$, there exists a non-null measurable set $\auxseta \in \algebra{\auxspace^n} $ where for all $\auxa \in \auxseta$, $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $,
  %where $\tdist_n$ is the distribution with pdf $1/Z_n\cdot\trunc{n}$ where $Z_n$ is the normalising constant.
  \changed[cm]{i.e.~for all $n\in\Nat$, $\enta \in \entspace^n$ and $\entseta \in \algebra{\entspace^n}$,
  if $\enta \in \support{\trunc{n}} $ and $\tdist_n(\entseta) > 0$ then there exists a non-null $\auxseta \in \algebra{\auxspace^n} $ such that for all $\auxa \in \auxseta$, $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $},
  where $\tdist_n$ is the distribution with pdf $1/Z_n\cdot\trunc{n}$ where $Z_n$ is the normalising constant.

\lo{This is a rather strong assumption.}

  \item[\cass\label{cass: everywhere positive aux density}] $\auxkernel{n}$ is \defn{everywhere positive}, i.e.~for all $\enta \in \entspace$ and $\auxa \in \auxspace$, $\auxpdf{n}(\enta,\auxa) > 0$.
\end{description}


Recall the conditions on the transition kernel to ensure convergence.

\begin{lemma}[\cite{Tierney94}, Theorem 1 and Corollary 2]
  \label{lemma: Tieryney}
  If the transition kernel $\transkernel{}$ with invariant distribution $\tdist$
  is $\tdist$-irreducible and $\tdist$-aperiodic, then
  for all $\state$, $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$ with $\norm{\cdot}$ denoting total variation distance.
\end{lemma}

\lo{Forget what I said about convergence in distribution -- I must have misremembered.
You are right: standard convergence results for Markov chains over continuous sample space are given in terms of total variational distance. See e.g.~\cite[Thm.~4]{Roberts2004} and \cite[Thm 11.3.1]{DoucMPS18}.}

% In our setting, we show that the irreducibility and aperiodicity of the \emph{fixed} dimension transition kernels w.r.t.~the \emph{fixed} dimension target distributions implies the same for the \emph{unbounded} transition kernel $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}$.
We assume that \allvass{} and \allcass{} are satisfied.

\cm{\cref{cass: very strong irreducible} is slightly stronger than saying that the fixed dimension transition kernels are strongly irreducible. If the conclusion is $\ninvo{n}(\enta,\auxa) \in \entseta \times \auxspace^n $ or ($\accept(\enta,\auxa) \not=1$ and $\enta \in \entseta$), then it will be exactly strongly irreducibility.}

\cm{I would like to relax this assumption to assuming the fixed dimension transition kernels are just irreducible. But more work would need to be done.}

\begin{proposition}
  \label{prop: acceptance > 0}
  $\accept \not= 0$ on $\validstates$.
\end{proposition}

\begin{proof}
  Assume for contradiction that $(\enta,\auxa) \in \validstates$ is such that
  $\accept(\enta,\auxa) = 0$.
  Then for $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$,
  we must have either
  $\trunc{\len{\enta}}(\enta') = 0$ or
  $\nauxpdf{\len{\enta}}(\enta',\auxa') = 0$ or
  $\det(\grad{\ninvo{\len{\enta}}}(\enta,\auxa)) = 0$.
  By the definition of $\validstates$ and \cref{cass: everywhere positive aux density},
  $\trunc{\len{\enta}}(\enta') \not= 0$ and
  $\nauxpdf{\len{\enta}}(\enta',\auxa') \not= 0$.
  Moreover, since $\ninvo{\len{\enta}}$ is a continuously differentiable involution, by chain rule we have
  $\grad{(\ninvo{\len{\enta}} \circ \ninvo{\len{\enta}})}(\state) = \grad{\ninvo{\len{\enta}}}(\ninvo{\len{\enta}}(\state)) \cdot \grad{\ninvo{\len{\enta}}}(\state) = \id(\state)$.
  Hence $\det(\grad{\ninvo{\len{\enta}}}(\ninvo{\len{\enta}}(\state))) \cdot \det(\grad{\ninvo{\len{\enta}}}(\state)) = 1$ which tells us that
  $\det(\grad{\ninvo{\len{\enta}}}(\state)) \not= 0$.
\end{proof}

\begin{lemma}
  \label{lemma: strong irreducible}
  Let $\trace \in \traces$ and $\traceset \in \algebra{\traces}$ where $\tree(\trace) > 0$ and $\tdist(\traceset) > 0$.
  Then $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\trace,\traceset) > 0$.
\end{lemma}

\begin{proof}
  Let $\trace \in \traces$ and $\traceset \in \algebra{\traces}$ where $\tree(\trace) > 0$ and $\tdist(\traceset) > 0$. We want to show that $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\trace,\traceset) > 0$. Note that we have
  \begin{align*}
    \transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}(\trace,\traceset) & := \transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(\traceset)) \tag{for $\state \in \inv{\marg}(\{\trace\})$} \\
    & = \int_{\states}\ \transkernel{2}(\state',\inv{\marg}(\traceset))\ \transkernel{1}(\state,\dif\state')\\
    & = \int_{\validstates}\ \transkernel{2}(\state',\inv{\marg}(\traceset))\ \transkernel{1}(\state,\dif\state').
    \tag{$\transkernel{1}(\state,\validstates) = 1 $}
  \end{align*}
  Hence we need to prove that there exists a measurable subset $\stateset \subseteq \validstates$ where (1) $\transkernel{1}(\state,\stateset) >0$ and (2) for all $\state' \in \stateset$, $\transkernel{2}(\state',\inv{\marg}(\traceset)) > 0 $.

  For sufficiently large $n \in \Nat$, we must have
  $\tdist_n(\proj{1}{\inv{\marg}(\traceset)\cap \validstates_n}) > 0$.
  By \cref{cass: very strong irreducible}, for any $\enta \in \entspace^n$ where $\NPempty(\enta,\tree) = \trace$, there exists a non-null measurable set $\auxseta_{\enta} \in \algebra{\auxspace^n} $ where for all $\auxa \in \auxseta_{\enta}$, $(\enta',\auxa') := \ninvo{n}(\enta,\auxa) \in \proj{1}{\inv{\marg}(\traceset)\cap \validstates_n} \times \auxspace^n $.
  Since $\enta, \enta' \in \support{\trunc{n}}$, there exists $k$ such that $(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \validstates$.

  We claim that $\stateset := \set{(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \validstates \mid \NPempty(\enta,\tree) = \trace \text{ and } \auxa \in \auxseta_{\enta}}$ satisfies (1) and (2).
  \begin{enumerate}[(1)]
    \item Consider $\transkernel{1}(\state,\stateset)$. Since $\auxseta_{\enta}$ is non-null for all $\enta \in \entspace^n$ where $\NPempty(\enta,\tree) = \trace$, by \cref{cass: everywhere positive aux density}
    \begin{align*}
      &\transkernel{1}(\state,\stateset) \\
      & =
      \sum_{n=1}^\infty
      \int_{\auxspace^n}
      \int_{\traces}
      [(\valuefn{\NPfill(\trace)}(\traceb') \concat\traceb'' ,\auxa) \in \stateset \cap \validstates_n]
      \nonumber \\
      & \qquad\qquad\qquad \nauxpdf{n}(\valuefn{\NPfill(\trace)}(\traceb') \concat\traceb'' ,\auxa)\
      {\measure{\traces}}{(\dif(\traceb' \concat\traceb''))}\
      {\measure{\auxspace^n}}{(\dif\auxa)} \\
      & =
      \sum_{k=1}^n
      \int_{\auxseta_{\enta}}
      \int_{\traces}
      [\enta = \valuefn{\NPfill(\trace)}(\traceb') \concat\traceb''] \cdot
      \nauxpdf{k}(\range{\enta}{1}{k},\range{\auxa}{1}{k})\
      {\measure{\traces}}{(\dif(\traceb' \concat\traceb''))}\
      {\measure{\auxspace^n}}{(\dif\auxa)} \\
      & > 0
    \end{align*}

    \item
    Let $(\entb,\auxb) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \stateset$ where $\NPempty(\enta,\tree) = \trace$ and $\auxa \in \auxseta_{\enta}$.
    \begin{align*}
      \transkernel{2}((\entb,\auxb), \inv{\marg}(\traceset))
      & :=
      \accept(\entb,\auxb)\cdot [\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)] \\
      & +
      (1-\accept(\entb,\auxb))\cdot [(\entb,\auxb) \in \inv{\marg}(\traceset)]
    \end{align*}
    By \cref{prop: acceptance > 0}, $\accept(\entb,\auxb) \not= 0$. So, it is enough to show $\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)$.

    Let $(\enta',\auxa') := \ninvo{n}(\enta,\auxa) \in \proj{1}{\inv{\marg}(\traceset)\cap \validstates_n} \times \auxspace^n $.
    Then, we have $\NPempty(\enta',\tree) \in A$.
    Since $\entb \in \support{\trunc{k}}$, applying \cref{vass: partial block diagonal inv} gives $\ninvo{k}(\entb,\auxb) = (\range{\enta'}{1}{k},\range{\auxa'}{1}{k})$.
    Since $(\entb,\auxb) \in \stateset \subseteq \validstates$, by \cref{prop: valid states are preserved by involutions} $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k}) \in \validstates$ and hence $\NPempty(\range{\enta'}{1}{k},\tree) = \NPempty(\enta',\tree) \in \traceset $.
    So $\ninvo{k}(\entb,\auxb) \in \inv{\marg}(\traceset)$ and
    $\transkernel{2}((\entb,\auxb), \inv{\marg}(\traceset)) > 0$.
  \end{enumerate}
\end{proof}

\begin{lemma}[\cite{DBLP:conf/icfp/BorgstromLGS16}, Corollary~2 and Lemma~33]
  \label{lemma: strong irred implies irred and aperiodic}
  A strong $\tdist$-irreducible transition kernel is also $\tdist$-irreducible and $\tdist$-aperiodic.
\end{lemma}

Finally by Tierney's Theorem (\cref{lemma: Tieryney}), the
$\tdist$-irreducible and $\tdist$-aperiodic (\cref{lemma: strong irreducible,lemma: strong irred implies irred and aperiodic}) transition kernel $\transkernel{\cref{alg: NP-iMCMC with hybrid parameter space}}$ with invariant distribution $\tdist$ (\cref{lemma: marginalised distribution is the target distribution}) generates a Markov chain that converges to the target distribution $\tdist$.

\convergence*

==> section/equiv-code.tex <==
% !TEX root = ./../icml2022.tex

\begin{code}[caption={Code for the equivalent program},label={code: e np-imcmc}]
def eNPiMCMCstep((x0,v0),w,inv,aux,pdfaux,auxstock,pdfauxstock):
  # step 1: initialisation
  #   find the instance of x0 which is in the support of w
  t0 = filter(lambda x: w(x) > 0, instance(x0))[0]
  #   sample partners for each value in the trace t0 to form an entropy trace x0
  x* = []
  for i in range(len(t0)):
    if Type(t0[i]) in Real:
      x*.append((t0[i],coin))
    else:
      x*.append((normal,t0[i]))
  #   sample v* from the auxiliary kernel applied to x*
  v* = [aux[i](x*[i]) for i in range(len(x*))]
  #   form a valid state (x*, v*)
  (x,v) = inv(x*,v*)
  while extree(w,x) == 0:
    r = normal; a = coin; p = auxstock; x*.append((r,a)); v*.append(p);
    (x,v) = inv(x*,v*)
  # step 2: involution on (x*,v*)
  (x,v) = inv(x*,v*)
  # step 3: acceptance
  if uniform < accept((x,v),(x*,v*),w,inv,pdfaux,pdfauxstock):
    return (x,v)
  else:
    return (x*,v*)
\end{code}

\begin{code}[caption={Code for helper functions},label={code:helper}]
# extension of w
extree(w,x) = max([w(t) for t in instance(x)])

# pdf of extended auxiliary kernel
def expdfaux(w, pdfaux, x, v):
  for t in instance(y):
    if w(t) > 0:
      return pdfaux(x[0:len(t)], v[0:len(t)])
  return 1

# list of all instances of y
def instance(y):
  instances = [t[:k+1]
    for t in [[y[i][p[i]] for i in range(len(y))] for p in product([0,1],len(y))]
    for k in range(len(t))]
  return instances

# the acceptance ratio
def accept((x,v),(x0,v0),w,inv,pdfaux,pdfauxstock):
  weight = ( extree(w,x) * expdfaux(w, pdfaux, x, v) * pdfnormal([e[0] for e in x]) * pdfauxstock(v) )
         / ( extree(w,x0) * expdfaux(w, pdfaux, x0, v0) * pdfnormal([e[0] for e in x0]) * pdfauxstock(v0) )
        * abs(det(grad(inv,(x0,v0))))
  return min(1,weight)
\end{code}

==> section/imcmc.tex <==
% !TEX root = ./../icml2022.tex

The \defn{involutive Markov chain Monte Carlo} (iMCMC), introduced by \citet{DBLP:conf/icml/NeklyudovWEV20,cusumanotowner2020automating}, is a framework for describing MCMC inference algorithms.
Given a (not necessarily normalised) target density $\tpdf$ on the measurable space $(X,\algebra{X},\measure{X})$, the iMCMC algorithm constructs a Markov chain of samples $\{\enta^{(i)}\}_{i\in\Nat}$ by generating the next sample $\enta$ using the current sample $\enta_0$ in three steps:
%\lo{I have suppressed the 3-step description of iMCMC because of repetition.}
\begin{enumerate}[1.]
  \item Sample a value $\auxa_0$ on the measurable space $(Y,\algebra{Y},\measure{Y})$ from the auxiliary kernel $\ikernel:X \kernelto Y$ applied to the current sample $\enta_0$;

  \item Compute the new state $(\enta,\auxa)$ by applying an involution $\iinv :X \times Y \to X\times Y$ (i.e.~$\iinv = \inv{\iinv}$) starting from $(\enta_0,\auxa_0)$ to obtain a new state $(\enta,\auxa)$;

  \item Accept this new sample $\enta$ with the Hastings' ratio.
\end{enumerate}

\begin{algorithm}
\caption{Involutive MCMC}
\label{alg: imcmc}
\begin{algorithmic}[1]
  \STATE \Input{Current sample $\enta_0:X$, density function $\tpdf:X \to \pReal$, involution $\invo:X \times Y\to X \times Y$, auxiliary kernel $\ikernel:X \kernelto Y$}
  \STATE \Output{Next sample $\enta:X$}
  \STATE $\auxa_0 \sim \ikernel(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \invo(\enta_0,\auxa_0)$
  \STATE $P := \min \left\{1,
    \tfrac
      {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa}) }
      {\tpdf(\enta_0)\cdot \pdf{\ikernel}({\enta_0},{\auxa_0})}
    \abs{\det{\big(\grad{\invo}(\enta_0,\auxa_0)\big)}}
    \right\}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return ${\enta}$
  \ELSE
    \STATE \Return ${\enta_0}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

Formally, we write it as \cref{alg: imcmc} and denote it as an iMCMC update (as it updates the sample from $\enta_0$ to $\enta$).

The probability for the next sample to be in a measurable set $U$ given the current sample $\enta$ is
the integral over the auxiliary space consisting the sum of
the probability of accepting the proposed sample and that it is in $U$ and
the probability of rejecting the proposed sample and the current sample $\enta$ is in $U$.
Hence, the transition kernel $\imcmca$ on the parameter space $X$ induced by the iMCMC update can be written as
\[
  \imcmca(\enta, U)
  :=
  \int_{Y}\
  \Big(
  \accept(\enta, \auxa)\cdot [\invo(\enta, \auxa) \in U \times Y] +
  (1-\accept(\enta, \auxa))\cdot [(\enta, \auxa) \in U \times Y]
  \Big)\
  \ikernel(\enta, \dif \auxa)
\]
where $\accept(\enta, \auxa)$ is the acceptance ratio of the state $(\enta, \auxa)$, i.e.~
\[
  \accept(\enta, \auxa)
  := \min \left\{1,
    \tfrac
      {\tpdf(\enta')\cdot \pdf{\ikernel}({\enta'},{\auxa'}) }
      {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa})}
    \abs{\det{\big(\grad{\invo}(\enta,\auxa)\big)}}
    \right\}
  \quad\text{ where }
  ({\enta'},{\auxa'}) = \invo(\enta, \auxa).
\]

Since we are interested in constructing a Markov chain to sample from the target distribution using the iMCMC update, we require the update to preserve the target distribution, i.e.~the distribution of the current sample and that of the next sample are both the target distribution.
The following proposition ensures the iMCMC update satisfies this property.

\begin{proposition}[\cite{DBLP:conf/icml/NeklyudovWEV20}, Proposition 2]
  \label{prop: imcmc is reversible and invariant}
  The Markov chain generated by iterating the iMCMC update (\cref{alg: imcmc}) is reversible w.r.t.~the target distribution $\tdist(U):= \frac{1}{Z}\shortint{U}{\tpdf}{\measure{X}}$, where $Z := \shortint{X}{\tpdf}{\measure{X}}$ is the normalising constant, i.e.~
  \begin{equation}
    \label{eq: detailed balance}
    \forall U, V \in \algebra{X}\quad
    \expandint{U}{\imcmca(\enta, V)}{\tdist}{\enta}
    = \expandint{V}{\imcmca(\enta, U)}{\tdist}{\enta}.
  \end{equation}
  This implies the target distribution is preserved by the iMCMC update.
\end{proposition}

\paragraph{Example (MH)}
\label{app: mh}

\paragraph{Example (Gibbs)}
\label{app: gibbs}

Beside the iMCMC framework, \citet{DBLP:conf/icml/NeklyudovWEV20} also gave a bag of ``tricks'' for combining iMCMC updates to ``facilitates the derivation of powerful extensions''.
These tricks can be summarised into three categories:
\begin{itemize}
  \item State-dependent mixture of iMCMC updates, which perform a different sampler depending on the current state;
  \item Clever involutions, which contains clever constructions of new involutions that better explore the parameter space.
  \item Composition of iMCMC updates, which compose iMCMC updates to make nonreversible chains which has better mixing time.
\end{itemize}

\subsection{State-dependent mixture of iMCMC updates}
\label{app: state-dependent mixture of imcmc}

Say $\set{\imcmca_a}_{a\in A}$ is a family of transition kernels of iMCMC updates for the target density function $\tpdf$ on $X$, each with involution $\invo_a$ and auxiliary kernel $\ikernel_a$.
A \defn{mixture} of $\set{\imcmca_a}_{a\in A}$ runs a random one of these updates by generating $a$ from some distribution and run $\imcmca_a$.
A mixture is \defn{state-dependent} if the distribution of $a$ depends on the current sample.
Let $\mixkernel: X \kernelto A$ be the mixture kernel where given the current sample $\enta$, $a$ is generated from $\mixkernel(\enta)$.
The acceptance ratio includes the mixture kernel $\mixkernel$ and becomes
\[
  \accept(\enta, \auxa, a)
  := \min \left\{1,
    \tfrac
      {\tpdf(\enta')\cdot \pdf{\ikernel_a}({\enta'},{\auxa'}) \cdot \pdf{\mixkernel}(\enta', a) }
      {\tpdf(\enta)\cdot \pdf{\ikernel_a}({\enta},{\auxa}) \cdot \pdf{\mixkernel}(\enta, a) }
    \abs{\det{\big(\grad{\invo_a}(\enta,\auxa)\big)}}
    \right\}
  \quad\text{ where }
  ({\enta'},{\auxa'}) = \invo_a(\enta, \auxa).
\]
Putting everything together, we have the \cref{alg: state dependent mixture of imcmc}.

\begin{algorithm}
\caption{State-dependent mixture of involutive MCMC}
\label{alg: state dependent mixture of imcmc}
\begin{algorithmic}[1]
  \STATE \Input{Current sample $\enta_0:X$, family of iMCMC updates $\set{\imcmca_a:X \kernelto X}_{a\in A}$, mixture kernel $\mixkernel: X \kernelto A$}
  \STATE \Output{Next sample $\enta:X$}
  \STATE $a \sim \mixkernel(\enta_0, \placeholder)$
  \STATE $\auxa_0 \sim \ikernel_a(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \invo_a(\enta_0,\auxa_0)$
  \STATE $P := \min \left\{1,
    \tfrac
      {\tpdf(\enta)\cdot \pdf{\ikernel_a}({\enta},{\auxa}) \cdot \pdf{\mixkernel}(\enta, a) }
      {\tpdf(\enta_0)\cdot \pdf{\ikernel_a}({\enta_0},{\auxa_0}) \cdot \pdf{\mixkernel}(\enta_0, a) }
    \abs{\det{\big(\grad{\invo_a}(\enta_0,\auxa_0)\big)}}
    \right\}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return ${\enta}$
  \ELSE
    \STATE \Return ${\enta_0}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

We can form a mixture distribution (Trick 1 in \cite{DBLP:conf/icml/NeklyudovWEV20}) by a state-dependent mixture of iMCMC updates with the same involution but different auxiliary kernels; similarly a mixture of involutions (Trick 2) by a state-dependent mixture of iMCMC updates with the same auxiliary kernel but different involutions.

\cm{Cite all the papers that use these tricks as in \cite{DBLP:conf/icml/NeklyudovWEV20}}

\subsection{Clever involutions in iMCMC updates}

\subsubsection{Auxiliary direction}
\label{app: auxiliary direction}

Given a non-involutive bijection $f$ on the state space $X \times Y$,
and an auxiliary kernel $\ikernel:X \kernelto Y$,
we can construct an iMCMC update by randomly choosing to apply $f$ or its inverse $\inv{f}$ depending on an auxiliary direction, as presented as Trick 3 in \cite{DBLP:conf/icml/NeklyudovWEV20}.

To formulate it as an iMCMC update with transition kernel $\imcmca$, we expand the auxiliary space $Y$ with the direction space $\dirspace := \set{+, -} $ and have involution
\begin{align*}
  \invo_{\imcmca}: X \times (Y \times \dirspace) & \to X \times (Y \times \dirspace) \\
  (\enta, (\auxa, \dira)) & \mapsto \begin{cases}
    (\enta', (\auxa', -)) & \text{if }\dira = + \text{ and } (\enta', \auxa') = f(\enta, \auxa) \\
    (\enta'', (\auxa'', +)) & \text{if }\dira = - \text{ and }(\enta'', \auxa'') = \inv{f}(\enta, \auxa)
  \end{cases}
\end{align*}
(It is standard to show that $\invo$ is indeed involutive.)
Moreover, the auxiliary kernel becomes $\ikernel_\imcmca: X \kernelto Y \times \dirspace$ where $\ikernel_\imcmca(\enta) := \ikernel(\enta) \times \Bern(0.5)$, where $\Bern(0.5)$ is the Bernoulli distribution on $\dirspace$.
Then, the new sample is accepted with the new acceptance ratio
\[
  \accept(\enta, (\auxa, \dira))
  := \min \left\{1,
    \tfrac
      {\tpdf(\enta')\cdot \pdf{\ikernel}({\enta'},{\auxa'})}
      {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa}) }
    \abs{\det{\big(\grad{\invo}(\enta, (\auxa, \dira))\big)}}
    \right\}
  \quad\text{ where }
  (\enta', (\auxa', \dira')) = \invo(\enta, (\auxa, \dira)).
\]

Putting it together, we have \cref{alg: imcmc with auxiliary direction}.
\begin{algorithm}
\caption{Involutive MCMC with Auxiliary Direction}
\label{alg: imcmc with auxiliary direction}
\begin{algorithmic}[1]
  \STATE \Input{Current sample $\enta_0:X$, density function $\tpdf:X \to \pReal$, bijection $f:X \times Y\to X \times Y$, auxiliary kernel $\ikernel:X \kernelto Y$}
  \STATE \Output{Next sample $\enta:X$}
  \STATE $\auxa_0 \sim \ikernel(\enta_0, \placeholder)$
  \STATE $\dira_0 \sim \Bern(0.5)$
  \IF{$\dira_0 = +$}
    \STATE $(\enta,\auxa) = f(\enta_0,\auxa_0)$
    \STATE $P := \min \left\{1,
      \tfrac
        {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa}) \cdot \pdf{\dirkernel}((\enta, \auxa), -) }
        {\tpdf(\enta_0)\cdot \pdf{\ikernel}({\enta_0},{\auxa_0}) \cdot \pdf{\dirkernel}((\enta_0,\auxa_0), +) }
      \abs{\det{\big(\grad{f}(\enta_0,\auxa_0)\big)}}
      \right\}$
  \ELSE
    \STATE $(\enta,\auxa) = \inv{f}(\enta_0,\auxa_0)$
    \STATE $P := \min \left\{1,
        \tfrac
          {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa}) \cdot \pdf{\dirkernel}((\enta, \auxa), +) }
          {\tpdf(\enta_0)\cdot \pdf{\ikernel}({\enta_0},{\auxa_0}) \cdot \pdf{\dirkernel}((\enta_0,\auxa_0), -) }
        \abs{\det{\big(\grad{\inv{f}}(\enta_0,\auxa_0)\big)}}
        \right\}$
  \ENDIF
  \IF{$\Uni(0,1) < P$}
    \STATE \Return ${\enta}$
  \ELSE
    \STATE \Return ${\enta_0}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\paragraph{Example (HMC)}
\label{app: hmc}

Recall the leapfrog method $\leapfrog$ of the Hamiltonian Monte Carlo (HMC) sampler which simulates the Hamiltonian motion of a particle on a surface derived from the density function.
This method $\leapfrog$ is bijective but not involutive.
Hence, to ensure reversibility, HMC implicitly samples a direction variable $\dira \in \dirspace$
from the discrete uniform distribution, alongside with the auxiliary variable $\auxa$ from the symmetric (i.e.~$\pdf{\Gau_n}(\auxa) = \pdf{\Gau_n}(-\auxa)$) multi-variate normal distribution $\Gau_n$.
If the direction $\dira$ is positive, it runs $\leapfrog(\enta, \auxa)$, else
it runs $\inv{\leapfrog}(\enta,\auxa)$ which is equal to $\leapfrog(\enta, -\auxa)$.
To see why this algorithm can be simplified to the standard presentation of HMC,
i.e.~no direction variable is sampled,
we consider the probability of applying the leapfrog method $\leapfrog$ to the state $(\enta, \auxa)$ when the direction is $+$ and $-$:
\[
  \pdf{\Uni\set{+,-}}(+)\cdot\pdf{\Gau_n}(\auxa) +
  \pdf{\Uni\set{+,-}}(-)\cdot\pdf{\Gau_n}(-\auxa)
  =
  0.5\cdot\pdf{\Gau_n}(\auxa)+
  0.5\cdot\pdf{\Gau_n}(\auxa)
  =
  \pdf{\Gau_n}(\auxa).
\]


\cm{Explain further.}

\subsubsection{Embedded involutions}

One can embed an involution $\invo$ in a bijection $f$ by considering
$\inv{f} \circ \invo \circ f$ to enhance exploration of the parameter space.

\subsection{Composition of iMCMC updates}
\label{eg: composition of imcmc udpates}

It is known that nonreversible Markov chains (those that does not satisfy \cref{eq: detailed balance}) have better mixing times, i.e.~more efficient convergence to the target distribution, compared to reversible Markov chains.
However, most MCMC samplers are reversible as it implies the update preserves the target distribution.
Indeed, the iMCMC update is also reversible (\cref{prop: imcmc is reversible and invariant}).

There has been more research on making MCMC algorithms nonreversible, for instance
Look ahead HMC (\cm{cite}) and Persistent HMC (\cm{cite}) are nonreversible extensions of the standard HMC algorithm, and nonreversible Jump MCMC (\cm{cite}) is the nonreversible extension of RJMCMC.
While Lifted MH (\cm{cite}) gives rise to many nonreversible MCMC algorithms, \cite{DBLP:conf/icml/NeklyudovWEV20} gives a cleaner and clearer framework for how to construct nonreversible MCMC algorithms in Trick 5 and 6.

The key observation in \citet{DBLP:conf/icml/NeklyudovWEV20} is that the composition of reversible iMCMC updates need not be reversible but will still preserves the target distribution (\cref{prop: invariant is closed under composition}).

\begin{proposition}
  \label{prop: invariant is closed under composition}
  Composition of transition kernels preserves invariant distribution.
\end{proposition}

\begin{proof}
  Let $\transkernel{1},\transkernel{2}$ be transition kernels on the measurable space $(X,\algebra{X},\measure{X})$ with invariant measure $\mu$.
  Then for any $U \in \algebra{X}$,
  \begin{align*}
    \mu(U)
    &= \expandint{X}{\transkernel{2}(x',U)}{\mu}{x'} \\
    &= \expandint{X}{\transkernel{2}(x',U)}{\int_{X}\ {\transkernel{1}(x,\dif x')\ \mu}}{x} \\
    &= \expandint{X}{\int_X\ \transkernel{2}(x',U)\cdot \transkernel{1}(x,\dif x')}{\mu}{x} \\
    &= \expandint{X}{(\transkernel{2}\circ \transkernel{1})(x,U)}{\mu}{x}.
  \end{align*}
  Hence $\mu$ is also invariant against the composition $\transkernel{2} \circ \transkernel{1}$.
\end{proof}

\citet{DBLP:conf/icml/NeklyudovWEV20} provided two ways of composing reversible updates to make them nonreversible.

\subsubsection{Persistent Involution}
\label{app: persistent involution}

First we assume that we have a non-involutive bijection $f$ on the state space $X \times Y$ and an auxiliary kernel $\ikernel:X \kernelto Y$.
Unlike in \cref{alg: imcmc with auxiliary direction} where we randomly choose to apply the bijection $f$ or its inverse $\inv{f}$ for each sample update, in persistent involution we keep applying $f$ in multiple sample updates until a proposed sample is rejected.
In that case, $\inv{f}$ is used instead and is kept for further sample updates until the proposed sample is rejected.

To formulate such an update, we consider two iMCMC updates $\imcmca$ and $\imcmcb$ on the parameter space $X \times \dirspace$, both aims to sample from the joint density function $(\enta, \dira) \mapsto \tpdf(\enta)$.
The first iMCMC update $\imcmca$ takes as involution
\begin{align*}
  \invo_{\imcmca}: (X \times \dirspace) \times Y & \to (X \times \dirspace) \times Y \\
  ((\enta, \dira), \auxa) & \mapsto \begin{cases}
    ((\enta', -), \auxa') & \text{if }\dira = + \text{ and } (\enta', \auxa') = f(\enta, \auxa) \\
    ((\enta'', +), \auxa'') & \text{if }\dira = - \text{ and }(\enta'', \auxa'') = \inv{f}(\enta, \auxa)
  \end{cases}
\end{align*}
and auxiliary kernel
$\ikernel_{\imcmca}: X \times \dirspace \kernelto Y$
defined as
$\ikernel_{\imcmca}(\enta, \dira) := \ikernel(\enta)$.
This means given a current sample, say $(\enta, +)$, the iMCMC update $\imcmca$ proposes the next sample by running $f$ on the state $(\enta, \auxa)$ with a randomly drawn auxiliary value $\auxa$ from $\ikernel(\enta)$ to obtain $(\enta', \auxa')$ and accepts $(\enta',-)$ as the next sample with probability
\[
  % \min \left\{1,
  %   \tfrac
  %     {\tpdf(\enta)\cdot \pdf{\Bern(0.5)}(+)\cdot \pdf{\ikernel}({\enta},{\auxa}) }
  %     {\tpdf(\enta_0)\cdot \pdf{\Bern(0.5)}(-)\cdot \pdf{\ikernel}({\enta_0},{\auxa_0})}
  %   \abs{\det{\big(\grad{f}(\enta_0,\auxa_0)\big)}}
  %   \right\}
  % =
  \min \left\{1,
    \tfrac
      {\tpdf(\enta)\cdot \pdf{\ikernel}({\enta},{\auxa}) }
      {\tpdf(\enta_0)\cdot \pdf{\ikernel}({\enta_0},{\auxa_0})}
    \abs{\det{\big(\grad{f}(\enta_0,\auxa_0)\big)}}
    \right\}.
\]

Notice that if we simply use $\imcmca$ to generate the Markov chain, it will remain reversible.
To make it nonreversible, it is composed with another iMCMC update $\imcmcb$ that given the current sample, say $(\enta', -)$, just flips the direction and proposes $(\enta', +)$, which is accepted with probability one.

By \cref{prop: imcmc is reversible and invariant}, the two transition kernels $\imcmca$ and $\imcmcb$ are reversible and hence preserves the joint target density $(\enta, \dira) \mapsto \tpdf(\enta)$.
As shown in \cref{prop: invariant is closed under composition}, their composition $\imcmcb \circ \imcmca$ also preserves the joint target density.
Finally, it is easy to see that the projection of $(\enta, \dira)$ to $\enta$ preserves the target distribution $\tpdf$.

\subsubsection{Persistent auxiliary kernel}

Assume we have two (distinct) auxiliary kernels $\ikernel_1, \ikernel_2 : X \kernelto Y$ and an involution $\invo: X \times Y \to X \times Y$.
To construct an nonreversible Markov chain, we keep on sampling from an auxiliary kernel, say $\ikernel_1$, until a proposed sample is rejected. In that case, the other auxiliary kernel $\ikernel_2$ is used instead and is kept until the proposed sample is rejected.

Similar to \cref{app: persistent involution}, we formulate this sampler by extending the parameter space to $X \times \dirspace$ and composing a iMCMC update $\imcmcc$ with the sampler $\imcmcb$ that flips the direction.
Both are sampling from the joint target distribution with density $(\enta, \dira) \mapsto \tpdf(\enta)$.

The first iMCMC update $\imcmcc$ takes as involution
$\invo_{\imcmcc}: (X \times \dirspace) \times Y \to (X \times \dirspace) \times Y$ with
\[
  \invo_{\imcmcc}((\enta, +), \auxa) := ((\enta', -), \auxa')
  \quad\text{ and }\quad
  \invo_{\imcmcc}((\enta, -), \auxa) := ((\enta', +), \auxa')
\]
where $(\enta', \auxa') = \invo(\enta, \auxa)$,
and auxiliary kernel
$\ikernel_{\imcmcc}: X \times \dirspace \kernelto Y$
defined as
\[
  \ikernel_{\imcmcc}(\enta, +) := \ikernel_1(\enta)
  \quad\text{ and }\quad
  \ikernel_{\imcmcc}(\enta, -) := \ikernel_2(\enta).
\]
This means given a current sample, say $(\enta_0, +)$, the iMCMC update $\imcmcc$ proposes the next sample by running $\invo$ on the state $(\enta_0, \auxa_0)$ with a randomly drawn auxiliary value $\auxa_0$ from $\ikernel_1(\enta_0)$ to obtain $(\enta, \auxa)$ and accepts $(\enta,-)$ as the next sample with probability
\[
  % \min \left\{1,
  %   \tfrac
  %     {\tpdf(\enta)\cdot \pdf{\Bern(0.5)}(+)\cdot \pdf{\ikernel_2}({\enta},{\auxa}) }
  %     {\tpdf(\enta_0)\cdot \pdf{\Bern(0.5)}(-)\cdot \pdf{\ikernel_1}({\enta_0},{\auxa_0})}
  %   \abs{\det{\big(\grad{\invo}(\enta_0,\auxa_0)\big)}}
  %   \right\}
  % =
  \min \left\{1,
    \tfrac
      {\tpdf(\enta)\cdot \pdf{\ikernel_2}({\enta},{\auxa}) }
      {\tpdf(\enta_0)\cdot \pdf{\ikernel_1}({\enta_0},{\auxa_0})}
    \abs{\det{\big(\grad{\invo}(\enta_0,\auxa_0)\big)}}
    \right\}.
\]

Composing $\imcmcc$ with the sampler $\imcmcb$ that given the current sample, say $(\enta, -)$, just flips the direction and proposes $(\enta, +)$, which is accepted with probability one, we have the nonreversible sampler.

Moreover, the argument that the marginalised Markov chain obtained by projecting the chain induced by $\imcmcc$ preserves the target distribution $\tpdf$ follows from \cref{app: persistent involution}.


==> section/invariant.tex <==
% !TEX root = ./../icml2022.tex

Now we identify the invariant distribution of the Markov chain induced by iterating
\cref{alg: np-imcmc (hybrid)}, and show that
it is indeed the target distribution $\tdist$.

\paragraph{State Distribution}

Recall
we consider a state to be an entropy-auxiliary pair which is traversed to
explore the target distribution via involutions.
We now define the \defn{state distribution} $\sdist$ on the
state space $\states := \bigcup_{n\in\Nat} (\entspace^n \times \auxspace^n)$
to be a distribution with density $\spdf$ (with respect to $\smeasure$) given by
\begin{align} \label{eq: defn of state distribution}
  \spdf(\enta,\auxa) :=
  \begin{cases}
    \displaystyle\frac{1}{Z} \trunc{\len{\enta}}(\enta) \cdot
    \exauxpdf(\enta, \auxa)
    % \prod_{i=1}^{\len{\enta}} \nauxpdf{i}(\seqindex{\enta}{i},\seqindex{\auxa}{i})
    & \text{if }(\enta,\auxa)\in \validstates \\
    {0} & \text{otherwise}
  \end{cases}
\end{align}
where
$Z := \shortint{\states}{\tree}{\measure{\states}}$ is the normalising constant and
$\validstates$ is %a subset of $\states$ which contains all valid states.
\changed[lo]{the subset of $\states$ consisting of all \emph{valid states}.}
We say a state $(\enta,\auxa)$ is \defn{valid} if
\begin{enumerate}[1.]
  \item $\enta \in \support{\trunc{\len{\enta}}}$, and

  \item $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$ implies
  $\enta' \in\support{\trunc{\len{\enta}}}$, and

  \item $(\range{\enta}{1}{k},\range{\auxa}{1}{k})
   % = \proj{\len{\enta}}{k}(\enta, \auxa)
  \not\in \validstates$ for all $k <\len{\enta}$.
\end{enumerate}
Intuitively, valid states are the states which,
when transformed by the involution $\ninvo{\len{\enta}}$,
(the first component of which) does not ``fall beyond'' the support of $\trunc{\len{\enta}}$.

We write $\validstates_n := \validstates \cap (\entspace^n \times \auxspace^n)$ to denote the the set of all $n$-dimensional valid states.
The following proposition shows that involutions preserve the validity of states.

\begin{proposition}
  \label{prop: valid states are preserved by involutions}
  $\ninvo{n}(\validstates) = \validstates$ for all $n\in\Nat$.
\end{proposition}

\begin{proof}
  First we show that
  $\ninvo{n}(\validstates) \subseteq \validstates$.
  Let $(\enta,\auxa) \in \validstates$ and $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$.
  Then we want to show that $(\enta',\auxa') \in \validstates$
  and consider the requirements for $(\enta',\auxa')$ being a valid state.

  (1) $\enta' \in \support{\trunc{\len{\enta'}}}$ and
  (2) $(\enta'',\auxa'') = \ninvo{\len{\enta'}}(\enta',\auxa')$ implies $\enta'' \in\support{\trunc{\len{\enta}}}$ are immediate
  as $\ninvo{\len{\enta}}$ is involutive and $(\enta,\auxa)$ is a valid state.
  We prove (3) by induction on $\len{\enta}$, i.e.~$(\enta,\auxa) \in \validstates$ and $(\enta',\auxa') = \ninvo{\len{\enta}}(\enta,\auxa)$ implies
  $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k})\not\in \validstates$ for all $k <\len{\enta}$.

  The base case where $\len{\enta} = 1$ trivially holds.
  Assuming the statement (3) holds
  for all $(\entb,\auxb) \in \validstates$ where $\len{\entb} < \len{\enta}$ and
  for contradiction that there exists some $k < \len{\enta}$ where
  $(\range{\enta'}{1}{k},\range{\auxa'}{1}{k})\in \validstates$.
  We now aim to show that
  $(\range{\enta}{1}{k},\range{\auxa}{1}{k})\in \validstates$.
  Since $\ninvo{\len{\enta}}$ is an involution, we have
  $\ninvo{\len{\enta}}(\enta',\auxa') = (\enta,\auxa)$.
  Moreover since $\range{\enta'}{1}{k} \in \support{\trunc{k}}$,
  i.e.~$\nsupport{k}{\tree} \cap \instances{\enta'} \not=\varnothing$,
  the \invoass{} (\cref{vass: partial block diagonal inv}) tells us that
  $\ninvo{k}(\range{\enta'}{1}{k},\range{\auxa'}{1}{k}) = (\range{\enta}{1}{k},\range{\auxa}{1}{k})$.
  By inductive hypothesis,
  for all $\ell < k$,
  $(\range{\enta}{1}{\ell},\range{\auxa}{1}{\ell}) \not\in \validstates$ and hence
  $(\range{\enta}{1}{k},\range{\auxa}{1}{k})$ is a valid state,
  which contradicts with the fact that $(\enta,\auxa)$ is a valid state.

  Now we have
  $\ninvo{n}(\validstates) \subseteq \validstates$.
  Since $\ninvo{n}$ is involutive, applying it give us
  $\validstates = \ninvo{n}(\ninvo{n}(\validstates)) \subseteq \ninvo{n}(\validstates)$.
  Hence
  $\ninvo{n}(\validstates) = \validstates$.
\end{proof}

Since the the entropy component of all valid states must be supported by
the extension $\extree$ of the target density, the set of valid states can be written as
\[
  \validstates =
  \bigcup_{m=1}^{\infty}
  \{
    (\enta,\auxa) \in \validstates_m \mid
    \enta \in \support{\trunc{\len{\enta}}},
    \auxa \in \auxspace^m
  \}.
\]

\paragraph{Transition kernel}
\label{par: transition kernel}
% definition of transition kernel

Say there is an encoding $\church{\placeholder}$ for the auxiliary space $\auxspace$ in SPCF. i.e.~there is a type $\church{\auxspace}$ in SPCF such that for each $\auxa \in \auxspace$, there is a unique SPCF program $\church{\auxa}$ with type $\church{\auxspace}$.

Following the Church encodings of pairs and lists in SPCF
discussed in \cref{sec: church encodings},
we can extend $\church{\placeholder}$ to represent a state $(\enta,\auxa) \in \states$ in SPCF as
\[
\church{(\enta,\auxa)}
:=
\anbr
{[\anbr{\pcf{\seqindex{(\seqindex{\enta}{1})}{1}},\pcf{\seqindex{(\seqindex{\enta}{1})}{2}}}, \dots
\anbr{\pcf{\seqindex{(\seqindex{\enta}{\len{\enta}})}{1}},\pcf{\seqindex{(\seqindex{\enta}{\len{\enta}})}{2}}}],
[\church{\seqindex{\auxa}{1}}, \dots,
\church{\seqindex{\auxa}{\len{\enta}}}]}
\]
of type $\tystate := \typair{\tylist{\typair{\tyreal}{\tybool}}}{\tylist{\church{\auxspace}}}$.
Take a SPCF term $\set{x:\tystate} \vdash \terma:\tystate $,
its \defn{transition kernel}
$\transkernel{\terma}: \states \kernelto \states$ is given by
\begin{align*}
  \transkernel{\terma} ({\state},\stateset) :=
  \shortint{\inv{v_{\terma}({\state},-)}(\stateset)}
  {\weightfn{\terma[\church{\state}/x]}}{\tmeasure}
\end{align*}
where the function $v_{\terma} :\states \times \traces \to \states$ is such that
$\church{v_{\terma}(\state,\traceb)} = \valuefn{\terma[\church{\state}/x]}(\traceb) $.
Intuitively,
$\transkernel{\terma} ({\state},\stateset)$ gives the probability of the term $\terma$
returning a state in $\stateset$ with the current state $\state$.

We say a distribution $\mu$ on states $\states$ is \defn{invariant}
w.r.t.~a SPCF term $\set{x:\tystate} \vdash \terma:\tystate $ if
$\mu$ is not altered after applying $\terma$, formally:
$\expandint{\states}{\transkernel{\terma}(\state,\stateset)}{\mu}{\state} = \mu(\stateset)$.

\paragraph{Equivalent Program}

Though the Hybrid NP-iMCMC algorithm (\cref{alg: np-imcmc (hybrid)}) traverses state,
it takes and returns \emph{samples} $\traceb \in \traces$.
This makes it awkward to ask the question
whether the state distribution $\sdist$ is invariant against it.
Instead, we consider a program (\codeinline{eNPiMCMCstep} in \cref{code: e np-imcmc})
which takes and returns \emph{states} and
prove $\sdist$ is invariant against it (\cref{lemma: e-np-imcmc invariant}).
After that, we show how this implies that
the target distribution $\tdist$ on $\traces$ is invariant against \cref{alg: np-imcmc (hybrid)}.

Helper functions \codeinline{extree(w)}, \codeinline{expdfaux}, \codeinline{instance} and \codeinline{accept} are given in \cref{code:helper}.
We assume the following primitive functions are implemented:
\codeinline{normal} is a sampler that draws from the standard normal distribution $\Gau$.
\codeinline{uniform} is a sampler that draws from the standard uniform distribution $\Uni(0,1)$.
\codeinline{coin} is a fair coin sampler.
\codeinline{grad(f,x)} gives the gradient of the function \codeinline{f} at \codeinline{x}.
Standard primitives such as
\codeinline{sum(list)}, \codeinline{abs(x)}, \codeinline{type(t)},
\codeinline{product(list,n)}\footnote{\codeinline{product(list,n)} gives the list of all (ordered) permutation of \codeinline{n} elements over the set \codeinline{list}.}, and
\codeinline{filter(f,list)}\footnote{\codeinline{filter(f,list)} gives the list containing elements of the set \codeinline{list} which return \codeinline{True} when applied to the function \codeinline{f}.} are assumed to be implemented.

Program \codeinline{eNPiMCMCstep} in \cref{code: e np-imcmc} is similar to the
Hybrid NP-iMCMC algorithm (\cref{alg: np-imcmc (hybrid)}).
It takes an initial state \codeinline{(x0,v0)},
a target density function \codeinline{w},
a family of involutions \codeinline{inv} where
\codeinline{inv(x,v)} gives the result of
$\ninvo{n}$ applied to the state \codeinline{(x,v)} for the $n$-length trace \codeinline{x},
a family of auxiliary kernels \codeinline{aux} where \codeinline{aux(x)} samples from the distribution $\nauxkernel{n}(x, \placeholder)$ for the $n$-length trace \codeinline{x},
their densities \codeinline{pdfaux} where \codeinline{pdfaux(x,v)} gives the result of $\nauxpdf{n}$ applied to the state \codeinline{(x,v)},
a stock auxiliary measure \codeinline{auxstock} which samples from the auxiliary stock measure $\measure{\auxspace}$, and
the density \codeinline{pdfauxstock} where \codeinline{pdfauxstock(v)} returns the result of $\nauxstockpdf{n}$ applies to the $n$-length auxiliary variable \codeinline{v}.

\codeinline{eNPiMCMCstep} then generates the next state \codeinline{(x,v)} in three steps --- Initialisation, Involution and Acceptance.
We now discuss each step in detail,
define its transition kernel and
demonstrate that the state distribution $\sdist$ is invariant against each step.

\input{section/equiv-code}

\begin{remark}
  Programs in \cref{code: e np-imcmc,code:helper} are given in Python syntax,
  but they can be translated into SPCF via Church encodings
  as discussed in \cref{sec: church encodings,par: transition kernel}.
\end{remark}

\paragraph{Initialisation (Step 1)}

Assuming the initial state \codeinline{(x0,v0)} is valid,
the initiation step (Line 2 to 18) in \codeinline{eNPiMCMCstep}
aims to construct a valid state \codeinline{(x*,v*)}
where the instance \codeinline{t*} of \codeinline{x*} that is in the support of the density \codeinline{w}
is the same as that of \codeinline{x0}.

It first finds the instance \codeinline{t0} of \codeinline{x0}
which is in the support of \codeinline{w} (Line 4).
Note that this step is deterministic and does not affect the transition kernel.

After that, it constructs a state \codeinline{(x*,v*)} by
first sampling partners for each value in the trace \codeinline{t0}
to form a entropy trace \codeinline{x*} of the same length (Line 6 to 11).
Say \codeinline{t} are the samples drawn,
then we can write the trace \codeinline{x*} as $\zip(\codeinline{t0},\codeinline{t})$.
Next, it samples the auxiliary variable \codeinline{v*} from \codeinline{aux(x*)} (Line 13).

Finally, it finds a \emph{valid} state by
keep appending \codeinline{x*} with samples from \codeinline{normal} and \codeinline{coin},
and \codeinline{v*} with samples from the auxiliary stock measure \codeinline{auxstock}
until the state \codeinline{(x*,v*)} is valid (Line 15 to 18).
If \codeinline{t} are the samples drawn for the entropy trace,
then we can write \codeinline{x*} as
$\zip(\codeinline{t0},\codeinline{t}) \concat \reshape(\codeinline{t})$,
where $\reshape(\traceb) :=
[(\seqindex{\traceb}{1},\seqindex{\traceb}{2}),
(\seqindex{\traceb}{3},\seqindex{\traceb}{4}),
\dots,
(\seqindex{\traceb}{n-1},\seqindex{\traceb}{n})] $
where $n = \floor{\frac{\len{\traceb}}{2}}*2$.

The transition kernel of the initialisation step is then
\begin{align*}
  \transkernel{1}((\enta_0,\auxa_0),\stateset)
  :=
  \sum_{n=1}^{\infty}
  \int_{\auxspace^n}
  \int_{\traces}
  \int_{\traces}
  &
  [(\zip(\traceb_0, \traceb) \concat\reshape(\traceb') ,\auxa) \in \stateset \cap \validstates]
  \nonumber \\
  & \exauxpdf(\zip(\traceb_0, \traceb) \concat\reshape(\traceb') ,\auxa)\
  {\measure{\traces}}{(\dif\traceb')}\
  {\measure{\traces}}{(\dif\traceb)}\
  {\measure{\auxspace^n}}{(\dif\auxa)}
\end{align*}
if $(\enta_0,\auxa_0) \in \validstates$ and $\traceb_0 \in \instances{\enta_0} \cap \support{\tree}$; and $0$ otherwise.

For any input initial state $(\enta_0,\auxa_0)$,
the following proposition ensures that
a valid state is almost surely be found in the initialisation step.

\begin{proposition}
  \label{prop: step 1 is probabilistic}
  For any $(\enta_0,\auxa_0) \in \validstates$, we have
  $\transkernel{1}((\enta_0,\auxa_0),\states) = 1$.
\end{proposition}

\begin{proof}
  Given all inputs to \codeinline{eNPiMCMC} with
  initial state $\codeinline{(x0,v0)}:= \church{(\enta_0,\auxa_0)}$,
  step 1 of \codeinline{eNPiMCMC} can be described by a closed SPCF term
  that does not contain $\score{\placeholder}$ as a subterm
  (following \cref{app: primitive functions,sec: church encodings}) and
  thus by \cref{theorem: np-imcmc is ast} terminates almost surely.
  By \cref{prop: AST SPCF term gives probability measure},
  the value measure of this term must be probabilistic. Hence
  $\transkernel{1}((\enta_0,\auxa_0),\states) = 1$.
\end{proof}

Before showing that the state distribution $\sdist$ is invariant against $\transkernel{1}$,
we consider a partition of the set of valid states to make the proof easier.
Let $(\enta, \auxa)$ be a valid state.
Then, $\enta$ can be uniquely partitioned into three traces
$\traceb_1, \traceb_2, \traceb_3$ where
\begin{itemize}
  \item $\traceb_1$ is the instance of $\enta$ that is in the support of $\tree$;

  \item $\traceb_2$ is the part of $\enta$ where $\zip(\traceb_1, \traceb_2) = \range{\enta}{1}{\len{\traceb_1}}$,
  % where $\zip$ is a function that takes two sequences of equal length and return a sequence with pairs of elements from each input sequence;

  \item $\traceb_3$ is the list containing all values in the suffix of $\enta$ where
  $\zip(\traceb_1, \traceb_2) \concat \reshape(\traceb_3) = \enta$.
\end{itemize}
\iffalse
For instance, say $[\true, 2.9]$ is in the support of the tree representable function $\tree$.
Then, the entropy trace $[(-0.2,\true), (2.9, \true), (1.3, \false)]$ can be partitioned into
$[\true, 2.9]$,
$[-0.2, \true]$ and
$[1.3, \false]$.
\fi

Hence the state distribution $\sdist$ applied to the measurable set $\stateset \in \algebra{\states}$ can be written as
\begin{align} \label{eq: state distribution}
  &
  \expandint{\stateset}{
  [(\enta,\auxa) \in \validstates] \cdot
  \frac{1}{Z} \trunc{\len{\enta}}(\enta) \cdot \exauxpdf(\enta,\auxa)
  }{\smeasure}{(\enta,\auxa)} \nonumber \\
  & =
  \displaystyle
  \sum_{n=1}^{\infty}
  \int_{\auxspace^n}
  \int_{\traces}
  \int_{\traces}
  \int_{\traces}
  [(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa) \in \stateset \cap \validstates]\cdot
  \frac{1}{Z} \tree(\traceb_1) \cdot
  \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa)\
  \nonumber\\
  & \displaystyle
  \qquad
  {\measure{\traces}}{(\dif\traceb_3)}\
  {\measure{\traces}}{(\dif\traceb_2)}\
  {\measure{\traces}}{(\dif\traceb_1)}\
  {\measure{\auxspace^n}}{(\dif\auxa)}
\end{align}


\begin{proposition}
  \label{prop: step 1 is invariant}
  The state distribution $\sdist$ is invariant against the initialisation step of
  \codeinline{eNPiMCMC}.
\end{proposition}

\begin{proof}
  We aim to show: \(\expandint{\states}{\transkernel{1}((\enta_0,\auxa_0),U)}{\sdist}{(\enta_0,\auxa_0)} = \sdist(U)\) for any measurable set $U \in \Sigma_{\states}$.
  (Changes are underlined for readability.)
  \begin{calculation}
    \displaystyle
    \expandint{\underline{\states}}{\transkernel{1}((\enta_0,\auxa_0),U)}{\sdist}{(\enta_0,\auxa_0)}
    %
    \step[=]{
      $\transkernel{1}((\enta_0,\auxa_0),U) = 0$ for all $(\enta_0,\auxa_0) \not\in \validstates$
    }
    \displaystyle
    \underline{\int_{\validstates}}\ {\transkernel{1}((\underline{\enta_0},\auxa_0),U)}\
    \underline{{\sdist}{(\dif(\enta_0,\auxa_0))}}
    %
    \step[=]{Formulation of $\sdist$ in \cref{eq: state distribution} writing $\enta_0$ as $\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3)$ where $\tree(\traceb_1) > 0$}
    \displaystyle
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}\
    \int_{\traces}\
    \int_{\traces}\
    \int_{\traces}\
    \underline{\transkernel{1}((\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0),U)}\cdot
    \\
    \displaystyle
    \qquad\qquad\qquad\qquad
    \Big(
    [(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0) \in \validstates] \cdot
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0)\Big)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}
    %
    \step[=]{Definition of $\transkernel{1}$}
    \displaystyle
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \Big(\displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa) \in U \cap \validstates]
    \\
    \qquad\qquad\qquad\qquad\qquad\qquad
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa)\
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    \Big)\cdot
    \\
    \displaystyle
    \qquad\qquad\qquad\qquad
    [(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0) \in \validstates] \cdot
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0)\Big)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}
    %
    \step[=]{Rearranging (allowed because everything is non-negative)}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \Big(\displaystyle
    \underline{
    \sum_{n=1}^{\infty}
    \int_{\auxspace^n}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0) \in \validstates] \cdot}
    \\
    \qquad\qquad\qquad\qquad\qquad\qquad
    \underline{
    \exauxpdf(\zip(\traceb_1, \traceb_2) \concat\reshape(\traceb_3) ,\auxa_0)\Big)\
    {\measure{\traces}}{(\dif\traceb_3)}\
    {\measure{\traces}}{(\dif\traceb_2)}\
    {\measure{\auxspace^n}}{(\dif\auxa_0)}}
    \Big)\cdot
    \\
    \displaystyle
    \qquad\qquad\qquad\qquad
    [(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa) \in U \cap \validstates]
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    %
    \step[=]{Definition of $\transkernel{1}$ where
    $(\hat{\enta_0}, \hat{\auxa_0})$ is an arbitrary valid state such that
    $\traceb_0 \in \instances{\hat{\enta_0}}$}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    \underline{\transkernel{1}((\hat{\enta_0}, \hat{\auxa_0}), \validstates)}\cdot
    \\
    \displaystyle
    \qquad\qquad\qquad\qquad
    [(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa) \in U \cap \validstates]
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    %
    \step[=]{By \cref{prop: step 1 is probabilistic}, $\transkernel{1}((\hat{\enta_0},\hat{\auxa_0}),\validstates) = \transkernel{1}((\hat{\enta_0},\hat{\auxa_0}),\states) = 1$}
    \displaystyle
    \sum_{m=1}^{\infty}
    \int_{\auxspace^m}
    \int_{\traces}
    \int_{\traces}
    \int_{\traces}
    [(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa) \in U \cap \validstates]
    \cdot
    \frac{1}{Z} \tree(\traceb_1) \cdot
    \exauxpdf(\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3') ,\auxa)\
    \\
    \displaystyle
    \quad
    {\measure{\traces}}{(\dif(\traceb_3'))}\
    {\measure{\traces}}{(\dif(\traceb_2'))}\
    {\measure{\traces}}{(\dif\traceb_1)}\
    {\measure{\auxspace^m}}{(\dif\auxa)}
    \step[=]{Formulation of $\sdist$ in \cref{eq: state distribution} writing $\enta_0$ as $\zip(\traceb_1, \traceb_2') \concat\reshape(\traceb_3')$ where $\tree(\traceb_0) > 0$}
    \sdist(U)
  \end{calculation}
\end{proof}

\paragraph{Involution (Step 2) and Acceptance (Step 3)}

After constructing a valid state \codeinline{(x*,v*)},
\codeinline{eNPiMCMCstep} traverses the state distribution
via the involution \codeinline{inv} to obtain a proposal state \codeinline{(x,v)} (Step 2: Line 20)
which is accepted with
probability specified by \codeinline{accept} (Step 3: Line 22 to 25).

The transition kernel for Steps 2 and 3 is given by
\[
  \transkernel{2,3}((\enta^*, \auxa^*),U) :=
  \begin{cases}
    {
      \accept(\enta^*, \auxa^*)\cdot[\ninvo{n}((\enta^*, \auxa^*)) \in U] +
      (1-\accept(\enta^*, \auxa^*))\cdot [(\enta^*, \auxa^*) \in U]
    } & \text{if }{(\enta^*, \auxa^*) \in \validstates_n} \\
    {0}
    & \text{otherwise,}
  \end{cases}
\]
where letting $(\enta,\auxa) = \ninvo{n}(\enta^*,\auxa^*)$ the acceptance ratio can be written as
\begin{align*}
  \accept(\enta^*, \auxa^*)
  & := \min\bigg\{1; \;
    \displaystyle\frac
      {\extree{(\enta)}\cdot\exauxpdf(\enta, \auxa)\cdot\nstockpdf{n}(\enta, \auxa)}
      {\extree{(\enta^*)}\cdot\exauxpdf(\enta^*, \auxa^*)\cdot\nstockpdf{n}(\enta^*, \auxa^*)}
    \cdot \abs{\det(\grad{\ninvo{n}(\enta^*, \auxa^*)})}\bigg\}
    \\
  & = \min\bigg\{1; \;
    \displaystyle\frac
      {\spdf(\enta,\auxa)\cdot\nstockpdf{n}(\enta, \auxa)}
      {\spdf(\enta^*,\auxa^*)\cdot\nstockpdf{n}(\enta^*, \auxa^*)}
    \cdot \abs{\det(\grad{\ninvo{n}(\enta^*, \auxa^*)})}\bigg\}.
\end{align*}

Before we show that the state distribution is invariant against $\transkernel{2,3}$,
we consider a partition of the set of valid states.
Let $\stateij{\boolveca}{\boolvecb}{n}$ be the set of $n$-dimensional valid states
$(\enta, \auxa) \in \validstates_n$ where
$\boolveca \in \Bool^n $ is the boolean values in $\enta$ and
$\ninvo{n}$ maps the state $(\enta, \auxa)$ to a (valid) state with boolean values $\boolvecb \in \Bool^n$.
Formally,
\[
\stateij{\boolveca}{\boolvecb}{n} := \set{(\enta, \auxa) \in \validstates_n \mid
  \enta = \zip(\realveca, \boolveca)\text{ and }
  (\zip(\realvecb, \boolvecb), \auxb) = \ninvo{n}(\enta, \auxa)
  \text{ for some }\realveca, \realvecb \in \Real^n, \auxb \in \auxspace^n
}.
\]
Then, the set of valid state can be partitioned to
\[
  \validstates
  =
  \displaystyle
  \bigcup_{n\in\Nat}
  \bigcup_{\boolveca, \boolvecb \in \Bool^n} \stateij{\boolveca}{\boolvecb}{n}.
\]

\begin{proposition}
  \label{prop: acceptance ratio is correct}
  Let $(\enta, \auxa) \in \validstates_n$ be a valid state and
  $(\enta', \auxa') = \ninvo{n}(\enta, \auxa)$.
  Then, we have
  \[
    \accept(\enta', \auxa')\cdot\spdf(\enta', \auxa')\cdot\nstockpdf{n}(\enta', \auxa')\cdot
    \abs{\det{(\grad{\ninvo{n}}(\enta, \auxa))}} =
    \accept(\enta, \auxa)\cdot\spdf(\enta, \auxa)\cdot\nstockpdf{n}(\enta, \auxa).
  \]
\end{proposition}

\begin{proof}
  Let $n\in\Nat$, $\boolveca, \boolvecb \in \Bool^n$ be such that
  $(\enta,\auxa) \in \stateij{\boolveca}{\boolvecb}{n}$, i.e.~
  $\enta = \zip(\realveca, \boolveca)$ and
  $(\enta', \auxa') = (\zip(\realvecb, \boolvecb), \auxa') = \ninvo{n}(\enta, \auxa)$
  for some
  $\realveca, \realvecb \in \Real^n$.
  Then
  taking the Jacobian determinant of
  $({\ninvoij{\boolvecb}{\boolveca}{n}} \circ {\ninvoij{\boolveca}{\boolvecb}{n}})(\realveca, \auxa) =
  (\realveca, \auxa)$
  and
  $(\realvecb, \auxa') = \ninvoij{\boolveca}{\boolvecb}{n}(\realveca, \auxa)$
  implies that
  \[
    \abs{\det{\big(\grad{\ninvo{n}}(\enta',\auxa')\big)}}
    =
    \abs{\det{\big(\grad{\ninvoij{\boolvecb}{\boolveca}{n}}(\realvecb,\auxa')\big)}}
    =
    \frac{1}{\abs{\det{\big(\grad{\ninvoij{\boolveca}{\boolvecb}{n}}(\realveca,\auxa)\big)}}}
    =
    \frac{1}{\abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}}.
  \]
  Hence,
  \begin{align*}
    & \accept(\enta', \auxa')\cdot\spdf(\enta', \auxa')\cdot\nstockpdf{n}(\enta', \auxa')\cdot
    \abs{\det{(\grad{\ninvo{n}}(\enta, \auxa))}} \\
    & = \begin{cases}
      \multicolumn{2}{@{}l@{\quad}}{\displaystyle\frac
        % accept
        {\spdf(\enta,\auxa)\cdot\nstockpdf{n}(\enta,\auxa)}
        {\spdf(\enta',\auxa')\cdot\nstockpdf{n}(\enta',\auxa')} \cdot
        \abs{\det{(\grad{\ninvo{n}}(\enta', \auxa'))}}
        %
        \cdot\spdf(\enta', \auxa')\cdot\nstockpdf{n}(\enta', \auxa')\cdot
        \abs{\det{(\grad{\ninvo{n}}(\enta, \auxa))}}} \\
      & \text{if }
        \displaystyle\frac
        {\spdf(\enta,\auxa)\cdot\nstockpdf{n}(\enta,\auxa)}
        {\spdf(\enta',\auxa')\cdot\nstockpdf{n}(\enta',\auxa')} \cdot
        \abs{\det{(\grad{\ninvo{n}}(\enta', \auxa'))}} < 1 \\
      % 1
      \spdf(\enta', \auxa')\cdot\nstockpdf{n}(\enta', \auxa')\cdot
      \abs{\det{(\grad{\ninvo{n}}(\enta, \auxa))}} & \text{otherwise}
    \end{cases}
    \tag{$\ninvo{n}$ is involutive} \\
    & = \begin{cases}
        % accept
        {\spdf(\enta,\auxa)\cdot\nstockpdf{n}(\enta,\auxa)}
      & \text{if }
        \displaystyle\frac
        {\spdf(\enta,\auxa)\cdot\nstockpdf{n}(\enta,\auxa)}
        {\spdf(\enta',\auxa')\cdot\nstockpdf{n}(\enta',\auxa')} \cdot
        \displaystyle\frac{1}{\abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}} < 1 \\
      % 1
      \spdf(\enta', \auxa')\cdot\nstockpdf{n}(\enta', \auxa')\cdot
      \abs{\det{(\grad{\ninvo{n}}(\enta, \auxa))}} & \text{otherwise}
    \end{cases}
    \tag{$\abs{\det{\big(\grad{\ninvo{n}}(\enta',\auxa')\big)}}
    = \displaystyle\frac{1}{\abs{\det{\big(\grad{\ninvo{n}}(\enta,\auxa)\big)}}}$} \\
    & = \accept(\enta, \auxa)\cdot\spdf(\enta, \auxa)\cdot\nstockpdf{n}(\enta, \auxa).
  \end{align*}
\end{proof}

\begin{proposition}
  \label{prop: step 2 is invariant}
  The state distribution $\sdist$ is invariant against the involution and acceptance steps
  of \codeinline{eNPiMCMC}.
\end{proposition}

\begin{proof}
  We aim to show:
  $\expandint{\states}{\transkernel{2}(\state,\stateset)}{\sdist}{\state} = \sdist(\stateset)$
  for all $\stateset \in \Sigma_{\states}$.

  We first show the following two integrals are the same.
  Let $\rmbool:\validstates \to \bigcup_{n\in\Nat} \Real^n \times \Bool^n $ be the function
  that remove all boolean components in a valid state,
  i.e.~$\rmbool(\zip(\realveca, \boolveca), \auxa) := (\realveca, \auxa)$.
  For any $\boolveca \in \Bool^n$,
  let $\addbool{\boolveca}:\bigcup_{n\in\Nat} \Real^n \times \Bool^n \to \states $ be the function
  that add the boolean vector $\boolveca$ to make a state,
  i.e.~$\addbool{\boolveca}(\realveca, \auxa) := (\zip(\realveca, \boolveca), \auxa)$.
  Then,
  we have
  $
    \ninvoij{\boolveca}{\boolvecb}{n}
    (\rmbool(\stateij{\boolveca}{\boolvecb}{n}))
  = \rmbool(\ninvo{n}(\stateij{\boolveca}{\boolvecb}{n}))
  = \rmbool(\stateij{\boolvecb}{\boolveca}{n})$
  for all ${\boolveca}, {\boolvecb} \in \Bool^n$.
  Hence, for any $\stateset \in \algebra{\states}$,
  we have
  \begin{align*}
    & \expandint{\stateij{\boolvecb}{\boolveca}{n}}{
      [(\enta, \auxa) \in \stateset \cap \validstates_n] \cdot
      \accept(\enta, \auxa) \cdot
      \spdf(\enta, \auxa)
    }{\measure{\entspace^n \times \auxspace^n}}{(\enta, \auxa)} \\
    & = \expandint{\stateij{\boolvecb}{\boolveca}{n}}{
      [(\enta, \auxa) \in \stateset \cap \validstates_n] \cdot
      \accept(\enta, \auxa) \cdot
      \spdf(\enta, \auxa) \cdot
      \nstockpdf{n}(\enta, \auxa)
    }{\measure{\leb_{2n}}}{(\realveca, \auxa)}
    \tag{$\enta = \zip(\realveca, \boolvecb)$} \\
    & = \expandint{\stateij{\boolveca}{\boolvecb}{n}}{
      [\ninvo{n}(\entb, \auxb) \in \stateset \cap \validstates_n] \cdot
      \accept(\ninvo{n}(\entb, \auxb)) \cdot
      \spdf(\ninvo{n}(\entb, \auxb)) \cdot
      \nstockpdf{n}(\ninvo{n}(\entb, \auxb)) \cdot
      \abs{\det{(\grad{\ninvoij{\boolveca}{\boolvecb}{n}}(\realvecb, \auxb))}}
    }{\measure{\leb_{2n}}}{(\realvecb, \auxb)}
    \tag{Integration by substitution with
      $(\enta, \auxa) = \ninvo{n}(\entb, \auxb)$ and
      $(\realveca, \auxa) = \ninvoij{\boolveca}{\boolvecb}{n}(\realvecb, \auxb)$
    } \\
    & = \expandint{\stateij{\boolveca}{\boolvecb}{n}}{
      [\ninvo{n}(\entb, \auxb) \in \stateset \cap \validstates_n] \cdot
      \accept(\entb, \auxb) \cdot
      \spdf(\entb, \auxb) \cdot
      \nstockpdf{n}(\entb, \auxb)
    }{\measure{\leb_{2n}}}{(\realvecb, \auxb)}
    \tag{\cref{prop: acceptance ratio is correct}} \\
    & = \expandint{\stateij{\boolveca}{\boolvecb}{n}}{
      [\ninvo{n}(\entb, \auxb) \in \stateset \cap \validstates_n] \cdot
      \accept(\entb, \auxb) \cdot
      \spdf(\entb, \auxb)
    }{\measure{\entspace^n \times \auxspace^n}}{(\realvecb, \auxb)}
  \end{align*}
  \iffalse
  \begin{align*}
    & \expandint{\stateij{\boolvecb}{\boolveca}{n}}{
      [(\enta, \auxa) \in \stateset \cap \validstates_n] \cdot
      \accept(\enta, \auxa) \cdot
      \spdf(\enta, \auxa)
    }{\measure{\entspace^n \times \auxspace^n}}{(\enta, \auxa)} \\
    & = \expandint{\rmbool(\stateij{\boolvecb}{\boolveca}{n})}{
      [(\realveca, \auxa) \in \rmbool(\stateset \cap \validstates_n)]
      \cdot
      \accept(\addBool{\realvecb}(\realveca, \auxa)) \cdot
      \spdf(\addBool{\realvecb}(\realveca, \auxa))
    }{\measure{\Real^n \times \auxspace^n}}{(\realveca, \auxa)} \\
    & = \expandint{\rmbool(\stateij{\boolvecb}{\boolveca}{n})}{
      [(\realveca, \auxa) \in \rmbool(\stateset \cap \validstates_n)]
      \cdot
      \accept(\addBool{\realvecb}(\realveca, \auxa)) \cdot
      \spdf(\addBool{\realvecb}(\realveca, \auxa)) \cdot
      \
    }{\measure{\Real^n \times \auxspace^n}}{(\realveca, \auxa)} \\
    %
    & = \int_{\rmbool(\stateij{\boolveca}{\boolvecb}{n})}\
      [\ninvoij{\boolveca}{\boolvecb}{n}(\realvecb, \auxb) \in
        \rmbool(\stateset \cap \validstates_n)]
      \cdot
      \accept(\ninvoij{\boolveca}{\boolvecb}{n}(\zip(\realvecb,\boolveca), \auxb)) \cdot
      \spdf(\ninvoij{\boolveca}{\boolvecb}{n}(\zip(\realvecb,\boolveca), \auxb)) \cdot
      \abs{\det{\grad{\ninvoij{\boolveca}{\boolvecb}{n}(\realvecb,\auxb) }}}\
      \\
    & \qquad
    {\measure{\Real^n \times \auxspace^n}}{\dif(\realvecb, \auxb)}
    \tag{Change of variable where $
      (\realveca,\auxa) = \ninvoij{\boolveca}{\boolvecb}{n}(\realvecb,\auxb)
    $} \\
    & = \expandint{\rmbool(\stateij{\boolveca}{\boolvecb}{n})}{
      [\ninvoij{\boolveca}{\boolvecb}{n}(\realvecb, \auxb) \in
        \rmbool(\stateset \cap \validstates_n)]
      \cdot
      \accept(\zip(\realvecb,\boolveca), \auxb) \cdot
      \spdf(\zip(\realvecb,\boolveca), \auxb)}
    {\measure{\Real^n \times \auxspace^n}}{(\realvecb, \auxb)}
    \tag{By above} \\
    & = \expandint{\stateij{\boolveca}{\boolvecb}{n}}{
      [\ninvo{n}(\entb, \auxb) \in \stateset \cap \validstates_n]
      \cdot
      \accept(\entb, \auxb) \cdot
      \spdf(\entb, \auxb)}
    {\measure{\entspace^n \times \auxspace^n}}{(\entb, \auxb)}
  \end{align*}
  \fi
  Finally we have
  \begin{align*}
    &\expandint{\states}{\transkernel{2}(\state,U)}{\sdist}{\state} \\
    & =
    \expandint{\validstates}{\transkernel{2}(\state,U)}{\sdist}{\state}
    \tag{$\transkernel{2}(\state, U) = 0$ for all $\state \in \states\setminus\validstates$}
    \\
    & =
    \sum_{n=1}^{\infty} \expandint{\validstates_n}{\transkernel{2}(\state,U)\cdot \spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & =
    \shortint{U}{\spdf}{\smeasure}
    +
    \sum_{n=1}^{\infty}
      \expandint{\validstates_n}{[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & \qquad\qquad\qquad\qquad\qquad\qquad -
      \sum_{n=1}^{\infty}
      \expandint{\validstates_n}{[\state \in U \cap \validstates_n]\cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state}
      \tag{Definition of $\transkernel{2}$} \\
    & =
    \shortint{U}{\spdf}{\smeasure}
      +
      \sum_{n=1}^{\infty}
      \sum_{\boolveca, \boolvecb \in \Bool^n}
      \expandint{\stateij{\boolveca}{\boolvecb}{n}}
      {[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & \qquad\qquad\qquad\qquad\qquad\qquad -
      \sum_{n=1}^{\infty}
      \sum_{\boolveca, \boolvecb \in \Bool^n}
      \expandint{\stateij{\boolvecb}{\boolveca}{n}}
      {[\state \in U \cap \validstates_n]\cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & =
    \shortint{U}{\spdf}{\smeasure}
      +
      \sum_{n=1}^{\infty}
      \sum_{\boolveca, \boolvecb \in \Bool^n}
      \expandint{\stateij{\boolveca}{\boolvecb}{n}}
      {[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    & \qquad\qquad\qquad\qquad\qquad\qquad -
      \sum_{n=1}^{\infty}
      \sum_{\boolveca, \boolvecb \in \Bool^n}
      \expandint{\stateij{\boolveca}{\boolvecb}{n}}
      {[\ninvo{n}(\state) \in U \cap \validstates_n]\cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \tag{By above} \\
    % & =
    % \shortint{U}{\spdf}{\smeasure}
    % +
    % \sum_{n=1}^{\infty}
    % \bigg(
    %   \expandint{\validstates_n}{[\ninvo{n}(\state) \in U \cap \validstates_n] \cdot \accept(\state) \cdot\spdf(\state)}{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state} \\
    % & \qquad\qquad\qquad\qquad
    %   -
    %   \expandint{\validstates_n}{
    %   [\ninvo{n}(\state) \in U \cap \validstates_n]\cdot \accept(\ninvo{n}(\state)) \cdot\spdf(\ninvo{n}(\state)) \cdot
    %   \abs{\det{\big(\grad{\ninvo{n}}(\state)\big)}}
    %   }{(\measure{\entspace_n}\times\measure{\auxspace_n})}{\state}
    % \bigg)
    % \tag{$\accept(\ninvo{n}(\state))\cdot \spdf(\ninvo{n}(\state))\cdot \abs{\det{\big(\grad{\ninvo{n}}(\state)\big)}} = \accept(\state) \cdot \spdf(\state)$ for all $\state \in \validstates$}
    % \\
    & =
    \shortint{U}{\spdf}{\smeasure}.
  \end{align*}
\end{proof}

Since the transition kernel $\transkernel{\cref{code: e np-imcmc}}$ of \codeinline{eNPiMCMCstep} is
the composition of $\transkernel{1}$ and $\transkernel{2}$,
i.e.~$
\transkernel{\cref{code: e np-imcmc}}(\state,U)
:= \int_{\states} \transkernel{2}(\state',U)\ \transkernel{1}(\state,\dif \state') $
for $\state \in \states$ and $U \in \algebra{\states}$,
and both $\transkernel{1}$ and $\transkernel{2}$ are invariant against $\sdist$
(\cref{prop: step 1 is invariant,prop: step 2 is invariant}).
Hence, with the following proposition, we deduce that
$\sdist$ is the invariant distribution of the Markov chain
generated by iterating \codeinline{eNPiMCMCstep}.

\begin{proposition}
  \label{prop: invariant is closed under composition}
  Composition of transition kernels preserves invariant distribution.
\end{proposition}

\begin{proof}
  Let $\transkernel{1},\transkernel{2}$ be transition kernels on the measurable space $(X,\algebra{X},\measure{X})$ with invariant measure $\mu$.
  Then for any $U \in \algebra{X}$,
  \begin{align*}
    \mu(U)
    &= \expandint{X}{\transkernel{2}(x',U)}{\mu}{x'} \\
    &= \expandint{X}{\transkernel{2}(x',U)}{\int_{X}\ {\transkernel{1}(x,\dif x')\ \mu}}{x} \\
    &= \expandint{X}{\int_X\ \transkernel{2}(x',U)\cdot \transkernel{1}(x,\dif x')}{\mu}{x} \\
    &= \expandint{X}{(\transkernel{2}\circ \transkernel{1})(x,U)}{\mu}{x}.
  \end{align*}
  Hence $\mu$ is also invariant against the composition $\transkernel{2} \circ \transkernel{1}$.
\end{proof}

\begin{lemma}
  \label{lemma: e-np-imcmc invariant}
  $\sdist$ is the invariant distribution of the Markov chain
  generated by iterating \codeinline{eNPiMCMCstep}.
\end{lemma}

\paragraph{Marginalised Markov Chains}

As discussed above, the Markov chain $\set{(\enta^{(i)},\auxa^{(i)})}_{i\in\Nat}$ on $\states$ generated by iterating \codeinline{eNPiMCMCstep} (which has invariant distribution $\sdist$) is \emph{not} the samples generated by \cref{alg: np-imcmc (hybrid)}.
The chain we are in fact interested in is the \emph{marginalised} chain $\set{\marg(\enta^{(i)},\auxa^{(i)})}_{i\in\Nat}$ where the measurable function $\marg:\validstates \to \traces$ takes a valid state $(\enta,\auxa)$ and returns the instance of the entropy trace $\enta$ that is in the support of the tree representable function $\tree$.

In this section we show that this marginalised chain has the target distribution $\tdist$ as its invariant distribution.
Let $\transkernel{\cref{alg: np-imcmc (hybrid)}}: \support{w} \kernelto {\traces}$ be the transition kernel of this marginalised chain, defined as $\transkernel{\cref{alg: np-imcmc (hybrid)}}(\traceb, A) := \transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))$ where $\state \in \inv{\marg}(\set{\traceb})$
for $\traceb \in \traces$ and $A \in \algebra{\traces}$.

\begin{proposition}
  \label{prop: properties about marg}
  Writing $\validstates_{\leq n} := \bigcup_{k=1}^n \validstates_k$,
  we let $\sdist_n$ be a probability distribution on
  the measurable space $\entspace^n \times \auxspace^n$ where
  \[
    \sdist_n(U) := \shortint{U}{\spdf_n}{\measure{\entspace^n \times \auxspace^n}}
    \quad
    \text{ and }
    \quad
    \spdf_n(\enta,\auxa) := \frac{1}{Z_n} \trunc{n}(\enta) \cdot \exauxpdf(\enta,\auxa)
  \]
  and $Z_n := \shortint{\entspace^n \times \auxspace^n}{\trunc{n}}{\measure{\entspace^n \times \auxspace^n}}$.
  \begin{enumerate}[1.]
    \item $\transkernel{\cref{alg: np-imcmc (hybrid)}}$ is well-defined.

    \item $\transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(A)) = \transkernel{\cref{alg: np-imcmc (hybrid)}}(\marg(\state),A)$ for all $\state \in \validstates$ and $A \in \algebra{\traces}$.

    \item $\sdist(\states \setminus {\validstates_{\leq n}}) \to 0$ as $n\to \infty$.

    \item $\exauxpdf(\enta, \auxa) = \expandint{\entspace \times \auxspace}{\exauxpdf(\enta \concat \enta', \auxa \concat \auxa')}{\measure{\entspace \times \auxspace}}{(\enta', \auxa')} $ for all $(\enta, \auxa) \in \validstates$.

    \item For $n \geq k$, $Z_k\cdot\sdist_k = Z_n\cdot {\proj{n}{k}}_*\sdist_n$ on $\validstates_k$.
    Recall $\proj{n}{k}(\enta,\auxa) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) $.

    \item $Z\cdot\sdist = Z_n\cdot g^{(n)}_*\sdist_n$ on ${\validstates_{\leq n}}$ where
    $g^{(n)} : \entspace^n \times \auxspace^{n}\partialto {\validstates_{\leq n}}$ such that
    $g^{(n)}(\enta,\auxa) = (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in {\validstates_{\leq n}}$.
  \end{enumerate}
\end{proposition}

\begin{proof}
  \begin{enumerate}[1.]

    \item Let $\traceb \in \traces$ and $\state,\state' \in \inv{\marg}(\set{\traceb})$.
    By the definition of $\transkernel{1}$,
    we must have $\transkernel{1}(\state, \placeholder) = \transkernel{1}(\state',\placeholder)$.
    Hence
    $
    \transkernel{\cref{code: e np-imcmc}}(\state, \placeholder)
    = (\transkernel{2} \circ \transkernel{1})(\state, \placeholder)
    = (\transkernel{2} \circ \transkernel{1})(\state', \placeholder)
    = \transkernel{\cref{code: e np-imcmc}}(\state', \placeholder).
    $ and
    $\transkernel{\cref{alg: np-imcmc (hybrid)}}$ is well-defined.

    \item Let $\state \in \validstates$ and $A \in \algebra{\traces}$. Then,
    $\transkernel{\cref{alg: np-imcmc (hybrid)}}(\marg(\state),A)
    = \transkernel{\cref{code: e np-imcmc}}(\state',\inv{\marg}(A))$
    for some $\state' \in \inv{\marg}(\set{\marg(\state)})$.
    Since $\state \in \inv{\marg}(\set{\marg(\state)})$,
    by above we have $
    \transkernel{\cref{code: e np-imcmc}}(\state,\inv{\marg}(A))
    = \transkernel{\cref{code: e np-imcmc}}(\state',\inv{\marg}(A))
    = \transkernel{\cref{alg: np-imcmc (hybrid)}}(\marg(\state),A)$.

    \item First note that $\sdist$ is an invariant distribution and hence is probabilistic.
    The sum $\sum_{n=1}^{\infty} \sdist(\validstates_n)$ which equals $\sdist(\bigcup_{n=1}^{\infty} \validstates_n) = \sdist(\validstates)$ must converge.
    Moreover, $\sdist(\states \setminus \validstates) = \expandint{}{[\state \in (\states\setminus\validstates) \cap \validstates] \cdot \spdf(\state)}{\measure{\states}}{\state} = 0$.
    Hence
    $
    \sdist(\states \setminus {\validstates_{\leq n}})
    = \sdist(\validstates \setminus {\validstates_{\leq n}})
    = \sum_{i=n+1}^{\infty} \sdist(\validstates_i)
    \to 0
    $ as $n\to \infty$.

    \item Simple application.

    \item Let $\stateset \in \algebra{\states}$ where $ \stateset \subseteq {\validstates_k}$. Then,
    for any $(\enta, \auxa) \in \stateset$,
    $
    Z_n \cdot \sdist_n(\enta, \auxa)
    = \extree(\enta)\cdot \exauxpdf(\enta, \auxa)
    = \extree(\range{\enta}{1}{k})\cdot \exauxpdf(\range{\enta}{1}{k}, \range{\auxa}{1}{k})
    = Z_k \cdot \sdist_k(\range{\enta}{1}{k}, \range{\auxa}{1}{k}).
    $
    Hence,
    \begin{align*}
      & Z_n \cdot ({\proj{n}{k}}_*\sdist_n)(\stateset) \\
      & = Z_n \cdot \sdist_n(\inv{{\proj{n}{k}}}{(\stateset)}) \\
      & = \expandint{\entspace^n \times \auxspace^n}
      {[(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \stateset] \cdot Z_n \spdf_n(\enta,\auxa)}
      {\measure{\entspace^n \times \auxspace^n}}{(\enta,\auxa)} \\
      & = \expandint{\entspace^n \times \auxspace^n}{
        [(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in \stateset] \cdot Z_k \spdf_k(\range{\enta}{1}{k},\range{\auxa}{1}{k}) \cdot
        \frac{\exauxpdf(\enta,\auxa)}{\exauxpdf(\range{\enta}{1}{k},\range{\auxa}{1}{k})}
      }{\measure{\entspace^n \times \auxspace^n}}{(\enta,\auxa)} \\
      & =
      \int_{\entspace^k \times \auxspace^k}\
      [(\enta',\auxa') \in \stateset] \cdot Z_k \spdf_k(\enta',\auxa') \cdot
      \Big(\expandint{\entspace^{n-k} \times \auxspace^{n-k}}{
        \frac
          {\exauxpdf(\enta'\concat\enta'',\auxa'\concat\auxa'')}
          {\exauxpdf(\enta',\auxa')}
        % \prod_{j=1}^{n-k}\auxpdf{k+j}(\seqindex{\enta''}{j},\seqindex{\auxa''}{j})
      }{\measure{\entspace^{n-k} \times \auxspace^{n-k}}}{(\enta'',\auxa'')}\Big) \\
      &\qquad\qquad
      \ {\measure{\entspace^k \times \auxspace^k}}{(\dif(\enta',\auxa'))}
      \tag{
      $(\enta', \auxa') = (\range{\enta}{1}{k}, \range{\auxa}{1}{k})$ and
      $(\enta'', \auxa'') = (\range{\enta}{k+1}{n}, \range{\auxa}{k+1}{n})$}
      \\
      % & =
      % \int_{\entspace^k \times \auxspace^k}\
      % [(\enta',\auxa') \in \stateset] \cdot Z_k \spdf_k(\enta',\auxa') \cdot \\
      % &\qquad
      % \Big(\expandint{\entspace^{n-k} \times \auxspace^{n-k}}{
      %   \auxpdf{n-k}(\enta'',\auxa'')
      % }{\measure{\entspace^{n-k} \times \auxspace^{n-k}}}{(\enta'',\auxa'')}\Big)
      % \ {\measure{\entspace^k \times \auxspace^k}}{(\dif(\enta',\auxa'))} \\
      & =
      \expandint{\entspace^k \times \auxspace^k}{
      [(\enta',\auxa') \in \stateset] \cdot Z_k \spdf_k(\enta',\auxa')
      }{\measure{\entspace^k \times \auxspace^k}}{(\enta',\auxa')}
      \tag{Part 4} \\
      & =
      Z_k\sdist_k(\stateset)
    \end{align*}
    \label{item: partial pointwise auxiliary kernel is used}

    \item Let $U \in \algebra{\states}$ where $ U \subseteq {\validstates_{\leq n}}$. Then,
    \begin{align*}
      Z\cdot \sdist(U)
      & = \expandint{U}{\extree(\enta)\cdot\exauxpdf(\enta, \auxa)}{\measure{\states}}{(\enta, \auxa)} \\
      & = \sum_{k=1}^n \expandint{U\cap\validstates_k}{\extree(\enta)\cdot\exauxpdf(\enta, \auxa)}{\measure{\entspace^k\times\auxspace^k}}{(\enta, \auxa)} \\
      & = \sum_{k=1}^n Z_k \cdot \sdist_k(U\cap \validstates_k) \\
      & = Z_n \sum_{k=1}^n {\proj{n}{k}}_* \sdist_n (U\cap \validstates_k) \tag{Part 5} \\
      & = Z_n \cdot \sdist_n (\bigcup_{k=1}^n
          \set{ (\enta,\auxa) \in \entspace^n \times \auxspace^n \mid (\range{\enta}{1}{k},\range{\auxa}{1}{k}) \in U\cap \validstates_k}) \\
      & = Z_n \cdot g^{(n)}_*\sdist_n (U).
    \end{align*}
  \end{enumerate}
\end{proof}


% \begin{lemma}
%   \label{lemma: marginalised distribution is the target distribution}
%   Given \allvass{}, $\tdist$ is the invariant distribution of the Markov chain generated by iterating \cref{alg: np-imcmc (hybrid)}.
% \end{lemma}
\hinvariant

\lo{Check: $\nu$ is the unique(?) invariant distribution of the induced Markov chain.}

%\lo{Note the standard result about existence and uniqueness of invariant distribution:}
\begin{proof}
  Assuming (1) $\tdist = \marg_*\sdist$ on $\traces$ and (2) $\tmeasure = \marg_*\smeasure$ on $\support{w}$, then for any $A \in \algebra{\traces}$,
  \begin{align*}
    \tdist(A) & = \marg_*\sdist(A) \tag{1} \\
    & = \expandint{\states}{\transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))}{\smeasure}{\state} \tag{\cref{lemma: e-np-imcmc invariant}} \\
    & = \expandint{\validstates}{\transkernel{\cref{code: e np-imcmc}}(\state, \inv{\marg}(A))}{\smeasure}{\state} \\
    & = \expandint{\validstates}{\transkernel{\cref{alg: np-imcmc (hybrid)}}(\marg(\state), A)}{\smeasure}{\state} \tag{\cref{prop: properties about marg}.2} \\
    & = \expandint{\support{\tree}}{\transkernel{\cref{alg: np-imcmc (hybrid)}} (\traceb, A)}{\marg_*\smeasure}{\traceb} \\
    & = \expandint{\support{\tree}}{\transkernel{\cref{alg: np-imcmc (hybrid)}} (\traceb, A)}{\tmeasure}{\traceb} \tag{2} \\
    & = \expandint{\traces}{\transkernel{\cref{alg: np-imcmc (hybrid)}} (\traceb, A)}{\tmeasure}{\traceb}.
  \end{align*}
  Hence, it is enough to show (1) and (2).

  \begin{enumerate}[1.]
    \item
    Let $A \in \algebra{\traces}$ where $A \subseteq \nsupport{n}{\tree} $ and $\delta > 0$.
    Then partitioning $\inv{\marg}(A)$ using $\validstates_k$, we have {for sufficiently large $m$},
    \begin{align*}
      \marg_*\sdist(A)
      & = \sdist\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right)
        + \sdist\left(\bigcup_{k=m+1}^\infty \inv{\marg}(A)\cap \validstates_k\right) \\
      & < \frac{Z_m}{Z} \cdot
        g^{(m)}_*\sdist_m\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right) + \delta
      \tag{by \cref{prop: properties about marg}.3 and \cref{prop: properties about marg}.6} \\
      & \leq \frac{Z_m}{Z} \cdot \sdist_m(
      \set{(\zip(\traceb, \traceb')\concat \reshape(\entb), \auxa) \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}, \auxa \in \auxspace^m}
      ) + \delta \\
      & = \frac{1}{Z} \expandint{\set{\zip(\traceb, \traceb')\concat \entb \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}}}{
        \trunc{m}(\enta)\cdot
        \big(\expandint{\auxspace^m}{\exauxpdf(\enta,\auxa)}{\measure{\auxspace^m}}{\auxa}\big)
      }{\measure{\entspace^m}}{\enta}
      + \delta \\
      & = \frac{1}{Z} \expandint{A}{\tree(\traceb)}{\measure{\traces}}{\traceb}
      + \delta
      \tag{$A \subseteq \nsupport{n}{\tree}$}
      \\
      & = \tdist(A) + \delta.
    \end{align*}
    For any measurable set $A \in \Sigma_{\traces}$,
    we have
    $
    \marg_*\sdist(A)
    = \marg_*\sdist(A \cap \support{\tree})
    = \sum_{n=1}^\infty \marg_*\sdist(A \cap \nsupport{n}{\tree})
    \leq \sum_{n=1}^\infty \tdist(A \cap \nsupport{n}{\tree})
    = \tdist(A \cap \support{\tree})
    = \tdist(A)$.
    Since both $\tdist$ and $\sdist$ are {probability} distributions, we also have
    $\tdist(A) = 1 - \tdist(\traces \setminus A)
    \leq 1 - \marg_*\sdist(\traces \setminus A)
    = 1 - (1- \marg_*\sdist(A))
    = \marg_*\sdist(A)$.
    Hence
    $\marg_*\sdist = \tdist$ on $\traces$.

    \item
    Similarly, let $A \in \algebra{\traces}$ where $A \subseteq \nsupport{n}{\tree} $ and $\delta > 0$.
    Then by \cref{prop: properties about marg}.3, {for sufficiently large $m$}, we must have
    $\smeasure(\bigcup_{k=m+1}^\infty \validstates_k) = \smeasure(\validstates \setminus \validstates_{\leq m}) < \delta$.
    Hence,
    \begin{align*}
      & \marg_*\smeasure(A) \\
      & = \smeasure\left(\bigcup_{k=1}^m \inv{\marg}(A)\cap \validstates_k\right)
        + \smeasure\left(\bigcup_{k=m+1}^\infty \inv{\marg}(A)\cap \validstates_k\right) \\
      & < \sum_{k=1}^m \measure{\entspace^{k}\times\auxspace^{k}} (\inv{\marg}(A)\cap \validstates_k) + \delta \\
      & = \sum_{k=1}^m \measure{\entspace^{m}\times\auxspace^{m}} (\set{(\enta,\auxa)\in \entspace^{m}\times\auxspace^m \mid (\enta^{1\dots k},\auxa^{1\dots k}) \in \inv{\marg}(A)\cap \validstates_k}) + \delta \\
      & = \measure{\entspace^{m}\times\auxspace^{m}} (\bigcup_{k=1}^m \set{(\enta,\auxa)\in \entspace^{m}\times\auxspace^m \mid (\enta^{1\dots k},\auxa^{1\dots k}) \in \inv{\marg}(A)\cap \validstates_k}) + \delta \\
      & \leq \measure{\entspace^{m}\times\auxspace^{m}}(\set{(\zip(\traceb, \traceb')\concat \entb, \auxa) \mid \traceb \in A, \traceb'\in \traces, \entb \in \entspace^{m-n}, \auxa \in \auxspace^m}) + \delta \\
      & = \tmeasure(A) + \delta.
    \end{align*}
    Then the proof proceeds as in (1).
    Note that since $\tree$ is almost surely terminating (\cref{vass: almost surely terminating tree}),
    $\marg_*\measure{\states}(\support{\tree}) = \measure{\traces}(\support{\tree}) = 1$
  \end{enumerate}
\end{proof}

As a consequence,
the Markov chain generated by iterating the NP-iMCMC algorithm described in \cref{fig:np-imcmc algo},
where the parameter space of the target density is $\bigcup_{n\in\Nat} \Real^n$,
also preserves the target distribution $\tdist$.

\invariant


==> section/new-convergence.tex <==
% !TEX root = ./../icml2022.tex

Last but not least, we check for
the convergence of the marginalised chain to the target distribution $\tdist$.

We first define a few helper functions.
\begin{itemize}
  \item
  Let $\etot: \bigcup_{n\in\Nat} \entspace^n \to \traces \cup \set{\bot} $ be a map where
  $\etot(\enta) := \begin{cases}
    \traceb \in \instances{\enta} \cap \support{\tree} \\
    \bot & \text{otherwise.}
  \end{cases} $
  Hence, $\etot(\enta)$ returns the instance of $\enta$ that is in the support of $\tree$ if it exists.

  \item
  Let $\tdist_n$ be a probability distribution on $\entspace^n$ with pdf
  $\tpdf_n:\enta \mapsto \frac{1}{Z_n} \extree(\enta)$
  where $Z_n$ is the normalising constant.

  \item
  Let $\transkernel{(n)}: \entspace^n \kernelto \entspace^n $ be the
  transition kernel of a iMCMC sampler for the target density $\tpdf_n$
  with a auxiliary kernel with pdf
  $\exauxpdf|_{\entspace^n \times \auxspace^n}$ and
  a involution $\ninvo{n}$,
  i.e.\[
    \transkernel{(n)}(\enta, \entseta)
    :=
    \expandint{\auxspace^n}{
      \accept(\enta, \auxa)\cdot
      [\ninvo{n}(\enta, \auxa) \in \entseta \times \auxspace^n] +
      (1-\accept(\enta, \auxa))\cdot
      [\enta \in \entseta]
    }{\measure{\auxspace^n}}{\auxa}.
  \]
  Recall
  $\accept(\enta, \auxa) :=
  \min\set{1,
    \frac{\extree(\enta') \cdot \exauxpdf(\enta', \auxa')}
    {\extree(\enta) \cdot \exauxpdf(\enta, \auxa)}
    \cdot
    \abs{\det{\grad{\ninvo{n}(\enta, \auxa)}}}
  }
  $
  for $(\enta', \auxa') := \ninvo{n}(\enta, \auxa)$.

  \item
  Let $\transkernel{(n)}^k$ be the result of $k$ compositions of $\transkernel{(n)}$ for all $k \in \Nat$,
  i.e.~$\transkernel{(n)}^0(\enta, \entseta) :=
  [\enta \in \entseta]$ and
  $\transkernel{(n)}^{k+1}(\enta, \entseta) :=
  \int_{\entspace^n}\ \transkernel{(n)}^{k}(\entb, \entseta)\ \transkernel{(n)}(\enta, \dif \entb)$
  for all $k \in \Nat$.
\end{itemize}

Now we can give the assumptions required for the convergence result.

\begin{description}
  \item[\cass\label{cass: irreducible}]
  For all $n \in\Nat$,
  $\transkernel{(n)} $ is $\tdist_n$-irreducible,
  i.e.~for any $\enta \in \nsupport{n}{\extree}$ and
  $\entseta \in \algebra{\entspace^n}$,
  $\tdist_n(\entseta) > 0$ implies
  there is a $k \in \Nat$ where
  $\transkernel{(n)}^k(\enta, \entseta) > 0$.

  \item[\cass\label{cass: exchange starting point}]
  Let $\traceb \in \traces$ and $\traceset \in \algebra{\traces}$.
  Then for any $\enta, \entb \in \inv{\etot}(\set{\traceb}) \cap \entspace^n $,
  $\transkernel{(n)}^k(\enta, \inv{\etot}(\traceset) \cap \entspace^n) > 0$
  implies
  $\transkernel{(n)}^k(\entb, \inv{\etot}(\traceset) \cap \entspace^n) > 0$.

  \item[\cass\label{cass: positive aux kernel}]
  For any $(\enta, \auxa) \in \validstates$,
  $\exauxpdf(\enta, \auxa) > 0$.
\end{description}

Recall the conditions on the transition kernel to ensure convergence.

\begin{lemma}[\cite{Tierney94}, Theorem 1 and Corollary 2]
  \label{lemma: Tieryney}
  If the transition kernel $\transkernel{}$ with invariant distribution $\tdist$
  is $\tdist$-irreducible and $\tdist$-aperiodic, then
  for all $\state$, $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$ with $\norm{\cdot}$ denoting total variation distance.
\end{lemma}

We assume that \allvass{} and \allcass{} are satisfied.

\begin{proposition}
  \label{prop: prop for convergence}
  We have the following results.
  \begin{enumerate}
    \item $\etot_*\measure{\entspace^n} = \measure{\traces} $
    on $\bigcup_{i=1}^n \nsupport{i}{\tree} $.

    \item $Z\cdot \tdist = Z_n \cdot (\etot_*\tdist_n)$
    on $\bigcup_{i=1}^n \nsupport{i}{\tree} $.

    \item For any $\entseta \in \algebra{\entspace^n}$,
    $\tdist_n(\entseta) > 0 $ implies
    $\tdist(\etot(\entseta) \cap \traces) > 0 $.
  \end{enumerate}
\end{proposition}

\begin{proof}
  \begin{enumerate}
    \item
    Let $\traceset \subseteq \bigcup_{i=1}^n \nsupport{i}{\tree} $.
    \begin{align*}
      (\etot_*\measure{\entspace^n})(\traceset)
      & = \measure{\entspace^n}(\inv{\etot}(\traceset) \cap \entspace^n)
       = \measure{\entspace^n}(\inv{\etot}(\bigcup_{i=1}^n \traceset \cap \nsupport{i}{\tree}) \cap \entspace^n) \\
      & = \measure{\entspace^n}(\bigcup_{i=1}^n \inv{\etot}(\traceset \cap \nsupport{i}{\tree}) \cap \entspace^n)
      = \measure{\entspace^n}(\bigcup_{i=1}^n (\inv{\etot}(\traceset \cap \nsupport{i}{\tree}) \cap \entspace^n)) \\
      & = \measure{\entspace^n}(\bigcup_{i=1}^n (
        \inv{\etot}(\traceset \cap \nsupport{i}{\tree}) \cap \entspace^i
      ) \times \entspace^{n-i})
      = \sum_{i=1}^n \measure{\entspace^n}((
        \inv{\etot}(\traceset \cap \nsupport{i}{\tree}) \cap \entspace^i
      ) \times \entspace^{n-i}) \\
      & = \sum_{i=1}^n \measure{\entspace^i}(
        \inv{\etot}(\traceset \cap \nsupport{i}{\tree}) \cap \entspace^i
      ) \\
      & = \sum_{i=1}^n \measure{\traces}(\traceset \cap \nsupport{i}{\tree}) \tag{\cm{Find cref}} \\
      & = \measure{\traces}(\traceset)
    \end{align*}

    \item
    Let $\traceset \subseteq \bigcup_{i=1}^n \nsupport{i}{\tree} $.
    \begin{align*}
      Z \cdot \tdist(\traceset)
      & = \expandint{\traceset}{\tree(\traceb)}{\measure{\traces}}{\traceb} \\
      & = \expandint{\inv{\etot}(\traceset)}
      {\tree(\etot(\enta))}
      {\measure{\entspace^n}}{\enta}
      \tag{Change of variable with $\traceb = \etot(\enta)$ and Part 1} \\
      & = \expandint{\inv{\etot}(\traceset)}
      {\extree(\enta)}
      {\measure{\entspace^n}}{\enta}
      \tag{$\extree(\enta) = \tree(\etot(\enta))$ for all $\enta$ such that $\etot(\enta) \not=\bot$} \\
      & = Z_n \cdot \tdist_n({\inv{\etot}(\traceset)})
      = Z_n \cdot (\etot_*\tdist_n)(\traceset)
    \end{align*}

    \item For any $\entseta \in \algebra{\entspace^n}$
    where $\tdist_n(\entseta) > 0$,
    we must have $\entseta \subseteq \nsupport{n}{\extree}$
    and $\etot(\entseta) \cap \traces \subseteq \bigcup_{i=1}^n \nsupport{i}{\tree} $, so by Part 2 and integrable assumption (\cref{vass: integrable tree}) we have
    \[
      \tdist(\etot(\entseta) \cap \traces)
      =
      \frac{Z_n}{Z} (\etot_*\tdist_n)(\etot(\entseta) \cap \traces)
      =
      \frac{Z_n}{Z} \tdist_n(\inv{\etot}(\etot(\entseta) \cap \traces))
      \geq
      \frac{Z_n}{Z} \tdist_n(\entseta)
      > 0
    \]
  \end{enumerate}
\end{proof}

\begin{lemma}
  Let $\traceb \in \support{\tree}$ and
  $\traceset \in \algebra{\traces}$ such that
  $\tdist(\traceset) > 0$ and
  let $\state \in \inv{\marg}(\set{\traceb})$.

  For all $k \in \Nat$,
  if there is a $N \in \Nat$ and
  $\stateset \subseteq \inv{\marg}(\set{\traceb}) \cap \validstates_{\leq N}$ such that
  $\transkernel{1}(\state, \stateset) > 0 $,
  $\tdist_N(\inv{\etot}(\traceset) \cap \entspace^n) > 0$ and
  for all $(\enta, \auxa) \in \stateset$ and all
  $\entb \in \entspace^{N-\len{\enta}}$,
  $\transkernel{(N)}^k(\enta \concat \entb, \inv{\etot}(\traceset) \cap \entspace^N) > 0 $,
  then
  $\transkernel{\cref{alg: np-imcmc (hybrid)}}^{k'}(\traceb, \traceset) > 0 $
  for some $k' \leq k$.
\end{lemma}

\begin{proof}
  We prove the statement by induction on $k\in\Nat$.
  \begin{description}
    \item[($k = 0$)]
    $\transkernel{(N)}^0(\enta \concat \entb, \inv{\etot}(\traceset) \cap \entspace^N)
    = [\enta \concat \entb \in \inv{\etot}(\traceset) \cap \entspace^N] > 0$
    implies that
    $\enta \concat \entb \in \inv{\etot}(\traceset) \cap \entspace^N$.
    Applying $\etot$ gives us
    \[
      \traceb
      = \etot(\enta \concat \entb)
      \in \etot (\inv{\etot}(\traceset) \cap \entspace^N)
      \subseteq \traceset.
    \]
    Hence, we have
    $\transkernel{\cref{alg: np-imcmc (hybrid)}}(\traceb, \traceset) = [\traceb \in \traceset] > 0 $.

    \item[($k = 1$)]
    Now we have
    \begin{align*}
      \transkernel{(N)}^1(\enta \concat \entb, \inv{\etot}(\traceset) \cap \entspace^N)
      & =
      \int_{\auxspace^N}\
      \accept(\enta \concat \entb, \auxa) \cdot
      [\ninvo{N}(\enta \concat \entb, \auxa) \in \inv{\etot}(\traceset) \cap \entspace^N \times \auxspace^N] \\
      & \qquad\qquad +
      (1-\accept(\enta \concat \entb, \auxa)) \cdot
      [\enta \concat \entb \in \inv{\etot}(\traceset) \cap \entspace^N]
      \ {\measure{\auxspace^N}}{(\dif\auxa)} \\
      & > 0.
    \end{align*}
    If $\enta \concat \entb \in \inv{\etot}(\traceset) \cap \entspace^N$,
    then using the same argument as the $k = 0$ case, we have
    $\transkernel{\cref{alg: np-imcmc (hybrid)}}^0(\traceb, \traceset) > 0 $.

    For the case where
    $\enta \concat \entb \not\in \inv{\etot}(\traceset) \cap \entspace^N$, i.e.~
    $\int_{\auxspace^N}\
      \accept(\enta \concat \entb, \auxa) \cdot
      [\ninvo{N}(\enta \concat \entb, \auxa) \in \inv{\etot}(\traceset) \cap \entspace^N \times \auxspace^N]
      \ {\measure{\auxspace^N}}{(\dif\auxa)} > 0$,
    there must exists a non-null subset $\auxseta_{\enta, \entb} $ of $\auxspace^N$ such that
    for all $\auxa' \in \auxseta_{\enta, \entb}$,
    $\accept(\enta \concat \entb, \auxa') > 0$ and
    $\ninvo{N}(\enta \concat \entb, \auxa') \in (\inv{\etot}(\traceset) \cap \entspace^N) \times \auxspace^N$.
    There must exists a $\ell \geq \len{\traceb}$ where
    $\proj{N}{\ell}(\enta \concat \entb, \auxa') \in \validstates$.
    Let $\stateset'$ be the set containing all each projections.

    Then, $\transkernel{1}(\state,\stateset') >0 $ as
    $\exauxpdf(\state') > 0$
    for all $\state' \in \stateset'$,
    $\transkernel{1}(\state, \stateset) > 0 $ (\cref{cass: positive aux kernel}), and
    $\entspace^{N-\len{\enta}}$ and $\auxseta_{\enta, \entb}$ are non-null sets.

    Moreover, for any $\state' \in \stateset'$,
    \[
      \transkernel{2}(\state', ((\inv{\etot}(\traceset) \cap \entspace^N)\times \auxspace^N) \cap \validstates)
      \geq
      \accept(\state')\cdot
      [\ninvo{N}(\state') \in ((\inv{\etot}(\traceset) \cap \entspace^N)\times \auxspace^N) \cap \validstates]
      > 0
    \]
    as $\accept(\enta \concat \entb, \auxa') > 0$ implies
    $\accept(\proj{N}{\ell}(\enta \concat \entb, \auxa')) > 0$ as long as $\proj{N}{\ell}(\enta \concat \entb, \auxa') \in \validstates$.

    Hence,
    $
    \transkernel{\cref{alg: np-imcmc (hybrid)}}
    (\traceb, \traceset)
    =
    \transkernel{\cref{code: e np-imcmc}}
    (\state, \inv{\marg}(\traceset))
    \geq
    (\transkernel{2} \circ \transkernel{1})
    (\state, ((\inv{\etot}(\traceset) \cap \entspace^N) \times \auxspace^N) \cap \validstates )
    > 0
    $

    \item
  \end{description}
\end{proof}


Finally by Tierney's Theorem (\cref{lemma: Tieryney}), the
$\tdist$-irreducible and $\tdist$-aperiodic transition kernel $\transkernel{\cref{alg: np-imcmc (hybrid)}}$ with invariant distribution $\tdist$ (\cref{theorem: marginalised distribution is the target distribution}) generates a Markov chain that converges to the target distribution $\tdist$.

\convergence


==> section/new-correctness.tex <==
% !TEX root = ./../icml2022.tex

In this section,
we present the \defn{Hybrid Nonparametric involutive Markov Chain Monte Carlo} (NP-iMCMC)
for the Statistical PCF language,
a universal (Turing-complete) probabilistic programming language with
\emph{both} discrete and continuous sampler constructs,
discussed in \cref{app: spcf}.
We first identify the conditions and properties of the inputs,
then present the Hybrid NP-iMCMC method and
finally give a three-step proof for its correctness.

\subsection{State Space, Target Density and Assumptions}
\label{app: assumptions}

\paragraph{Entropy Space}

Recall an execution trace $\traceb \in \traces := \bigcup_{n\in\Nat} (\Real \cup \Bool)^n$,
the input of the target density function $\tree$,
is a record of drawn values in a particular run of a probabilistic program.
For probabilistic programs that samples from both discrete and continuous distributions,
like SPCF,
the positions and numbers of discrete and continuous random variables
in an execution trace may vary, because of branching.
This is a problem because most hybrid MCMC inference algorithms
has a parameter space where
the position and the number of discrete and continuous random variables are both fixed.
\cm{Check if this is true.}

Luckily there is a simple solution.
We can pair each value $\seqindex{\traceb}{i}$ in a trace $\traceb$
with a random variable $\trace$ of the other type
to make a pair $(\seqindex{\traceb}{i},\trace)$ (or $(\trace, \seqindex{\traceb}{i})$).
For instance, the trace $[\true, -3.1]$ can be made into a
(two-dimensional) \emph{entropy trace} $[(1.5,\true),(-3.1,\true)]$
with randomly drawn value $1.5$ from the normal distribution and $\true$ from a coin toss.
Then, the position of discrete and continuous random variable does not matter and
the number of discrete and continuous random variables are fixed
for each dimension.

Formally, we define the \defn{entropy space} $\entspace := \Real \times \Bool$ to be the product space of
the Real probability space and
the Boolean probability space,
i.e.~equipped with
$\algebra{\entspace} := \sigma\big(\set{\realset \times \boolset \mid \realset \in \Borel, \boolset \in \algebra{\Bool}}\big)$
and $\measure{\entspace}(\entseta) := \expandint{\Bool}{\Gau(\set{\reala \in \Real \mid (\reala,\boola) \in \entseta})}{\measure{\Bool}}{\boola}$.
Since $\Gau$ and $\measure{\Bool}$ are probability measures,
so is $\measure{\entspace}$.
Moreover, it has a derivative $\entstockpdf$ defined as
$\entstockpdf(\reala, \boola) := \frac{1}{2}\pdfGau(\reala)$, w.r.t.~the Lebesgue measure.
An \defn{entropy trace} is an list of values from the entropy space,
i.e.~it is an element in the list measure space
$({\bigcup_{n\in\Nat}\entspace^n}, \algebra{\bigcup_{n\in\Nat}\entspace^n}, \measure{\bigcup_{n\in\Nat}\entspace^n})$ of the entropy space.
% The product of $n$ copies of entropy space is
% the \defn{$n$-dimensional entropy space} and denoted as
% $(\entspace^n, \algebra{\entspace^n}, \measure{\entspace^n})$.

The transformation from trace to entropy trace must be reversible,
i.e.~we can recover the trace we started with,
in order for us to work with entropy traces instead of traces.
Though not all traces have this property,
we found that those in the support of a tree representable function does.

Let $\enta \in \bigcup_{n\in\Nat} (\Real \times \Bool)^n$ be an entropy trace.
We can form traces $\traceb$ in $\bigcup_{n\in\Nat} (\Real \cup \Bool)^n$
by selecting either a real or boolean value
from each ordered pair of a prefix of $\enta$.
For example,
from the entropy trace $[(-0.2,\true), (2.9, \true), (1.3, \false)]$,
traces like $[-0.2,\true, \false]$, $\emptytrace$, $[\true, 2.9]$ and $[\true]$ can be formed.
We call these traces \defn{instances} of the entropy trace.
Formally, a trace $\traceb \in \traces$ is an instance of an entropy trace
$\enta \in \bigcup_{n\in\Nat} \entspace^n$ if
$\len{\traceb} \leq \len{\enta}$ and
$\seqindex{\traceb}{i} \in \set{\reala,\boola \mid (\reala,\boola) = \seqindex{\enta}{i}}$ for all $i = 1,\dots, \len{\traceb}$.
We denote the set of all instance of $\enta$ as
$\instances{\enta} \subseteq \traces$.
There is a simple proposition between instances and tree representable functions.

\begin{proposition}
  \label{prop: instances and tree representable}
  For any entropy trace $\enta \in \bigcup_{n\in\Nat} \entspace^n$ and
  any tree representable function $\tree$ on $\traces$,
  there is at most one trace $\traceb\in \traces$ that is both
  an instance of $\enta$ and in the support of $\tree$.
\end{proposition}

The trace we started with must be an instance of $\enta$.
Since $\tree$ is tree representable,
by \cref{prop: instances and tree representable},
\emph{at most one} trace $\traceb \in \instances{\enta}$
is in the support of a tree representable function $\tree$.
Hence, even though the transformation from trace to entropy trace
can have infinite possibilities,
we can always recover the trace that is in the support of
a tree representable function.

\paragraph{Auxiliary Space}

We assume the \defn{auxiliary space} $\auxspace := \Real$ to be
the Real probability measure space,
equipped with a $\sigma$-algebra $\algebra{\auxspace}$ and
a probability measure $\measure{\auxspace}$
with a derivative $\auxstockpdf$ w.r.t.~the Lebesgue measure.
Moreover, $\auxspace$
is a one-dimensional differential manifold,
equipped with an atlas.
Then,
$\auxspace^n$ is the $n$-dimensional Real space;
$\algebra{\auxspace^n}$ is the $\sigma$-algebra generated by subsets of the form $\prod_{i=1}^n \auxseta_i$ where $\auxseta_i \in \algebra{\auxspace}$; and
$\measure{\auxspace^n}$ is the product of $n$ copies of $\measure{\auxspace}$;
Note that $(\auxspace^n,\algebra{\auxspace^n},\measure{\auxspace^n})$ is a
probability measure space, and
$\auxspace^n$ is a $n$-dimensional differential manifold,
equipped with the product atlas.

\paragraph{State Space}

We consider a \defn{state} to be a pair of \emph{equal length} entropy trace and auxiliary variable.
The \defn{state space} $\states$ is thus the countable (disjoint) union of the product of finite dimensional entropy and auxiliary spaces.
Formally the state space $\states := \bigcup_{n\in\Nat} (\entspace^n \times \auxspace^n)$
is equipped with the $\sigma$-algebra
$\algebra{\states} := \sigma\set{\entseta_n \times \auxseta_n \mid \entseta_n \in \algebra{\entspace^n}, \auxseta_n \in \algebra{\auxspace^n}, n\in\Nat}$ and
measure
$\measure{\states}(\stateset) := \sum_{i=1}^n \expandint{\auxspace^n}{\measure{\entspace^n}(\set{\enta\in\entspace^n\mid (\enta,\auxa)\in\stateset})}{\measure{\auxspace^n}}{\auxa}$.

\subsubsection{Target Density function}

We assume our target density function $\tree$ is specified by a SPCF program.
Hence the density function $\tree$ has
the trace space $\traces := \bigcup_{n\in\Nat} (\Real \cup \Bool)^n $ as parameter space and
is tree representable (\cref{prop: all spcf terms have TR weight function}).
Moreover, we assume the followings.
\begin{itemize}
  \item[(\cref{vass: integrable tree})]
  $\tree$ is \defn{integrable},
  i.e.~$\shortint{\traces}{\tree}{\measure{\traces}} =: Z < \infty$
  (otherwise, the inference problem is undefined).

  \item[(\cref{vass: almost surely terminating tree})]
  $\tree$ is \defn{almost surely terminating (AST)},
  i.e.~\changed[cm]{$\measure{\traces}(\set{\traceb\in \traces \mid \tree(\traceb) > 0}) = 1$}
  (otherwise, the \changed[lo]{loop of the Hybrid NP-iMCMC algorithm in \cref{alg: np-imcmc (hybrid)} may} not terminate almost surely).
\end{itemize}

\subsubsection{Inputs}

Recall besides the target density function $\tree$,
there are two additional inputs to the iMCMC algorithm:
\defn{auxiliary kernel} (to introduce additional randomness) and
\defn{involution} (to move around the \emph{state space}).
Here we explore the conditions on and properties of all three inputs
in preparation for the NP-iMCMC transformation.

\paragraph{Auxiliary kernels}

For each dimension $n\in\Nat$,
there is an \defn{auxiliary kernel}
$\nauxkernel{n}: \entspace^n \kernelto \auxspace^n$
that is probabilistic, i.e.~$\nauxkernel{n}(\enta, \auxspace^n) = 1$ for all $\enta \in \entspace^n$,
and has probability density function (pdf) $\nauxpdf{n}:\entspace^n \times \auxspace^n \to \pReal$ such that
$\nauxkernel{n}(\enta, \auxseta) = \expandint{\auxseta}{\nauxpdf{n}(\enta, \auxa)}{\measure{\auxspace^n}}{\auxa}$ for all $\enta \in \entspace^n$ and $\auxseta \in \algebra{\auxspace^n}$.

\paragraph{Involutions}

We say an endofunction $\ninvo{n}$ on $\entspace^n \times \auxspace^n$
is \defn{differentiable} if
for all $\boolveca, \boolvecb \in \Bool^n$, the function
$\ninvoij{\boolveca}{\boolvecb}{n}$ on $\Real^n \times \auxspace^n$
defined as
$\ninvoij{\boolveca}{\boolvecb}{n}(\realveca, \auxa) := (\realvecb, \auxb)$
where
$\ninvo{n}(\zip(\realveca, \boolveca), \auxa) := (\zip(\realvecb, \boolvecb), \auxb)$\footnote{
We write $\zip(\ell_1, \ell_2) $ to be the list
$[(\seqindex{\ell_1}{1}, \seqindex{\ell_2}{1}),
(\seqindex{\ell_1}{2}, \seqindex{\ell_2}{2}), \dots,
(\seqindex{\ell_1}{n}, \seqindex{\ell_2}{n})] $
for any lists $\ell_1, \ell_2$ with $n := \min{\set{\len{\ell_1}, \len{\ell_2}}}$.
},
is almost surely differentiable on the set
$\set{ (\realveca, \auxa) \in \Real^n \times \auxspace^n \mid
\ninvo{n}(\zip(\realveca, \boolveca), \auxa) = (\zip(\realvecb, \boolvecb), \auxb)}$.
Hence, the Jacobian of $\ninvo{n}$ on $(\zip(\realveca, \boolveca), \auxa)$ is
$\grad{\ninvo{n}}(\zip(\realveca, \boolveca), \auxa) :=
\grad{\ninvoij{\boolveca}{\boolvecb}{n}}(\realveca, \auxa)$.

We assume there is a differentiable
endofunction $\ninvo{n}$ on $\entspace^n \times \auxspace^n$ for each dimension $n \in\Nat$
that is involutive,
i.e.~$\ninvo{n} = \inv{\ninvo{n}}$ and satisfies the \changed[lo]{\emph{\invoass{}}}:
\begin{compactitem}
  \item[(\cref{vass: partial block diagonal inv})]
  For all $(\enta, \auxa) \in \states$ where $\len{\enta} = m$,
  if $\nsupport{n}{\tree} \cap \instances{\enta} \not= \varnothing$ for some $n$,
  then for all $k = n, \dots, m$,
  $\proj{m}{k}(\ninvo{m}(\enta, \auxa)) = \ninvo{k}(\proj{m}{k}(\enta, \auxa)) $
\end{compactitem}
where $\proj{k_1}{k_2}$ is the projection that takes a state $(\enta,\auxa)$
with components of length $k_1$ and returns the state
$(\range{\enta}{1}{k_2},\range{\auxa}{1}{k_2})$ with
the first $k_2$ coordinates of each component.

\subsection{Algorithm}
\label{app: hybrid np-imcmc}

Henceforth, we assume that there is a tree representable function $\tree$ that is
integrable (\cref{vass: integrable tree}) and
almost surely terminating (\cref{vass: almost surely terminating tree}),
a family of auxiliary kernels $\set{\nauxkernel{n}:\entspace^n \kernelto \auxspace^n}$ and
a family of involutions $\set{\ninvo{n}}_n$ that is
\invoass{} (\cref{vass: partial block diagonal inv}).

Before presenting the algorithm for the Hybrid NP-iMCMC sampler,
we introduce two helper functions.

\paragraph{Extension of Target Density}

The \defn{extension} of a tree representable function $\tree$ on $\traces$ is a map
$\extree: \bigcup_{n\in\Nat}\entspace^n \to \pReal $ where
given an entropy space $\enta \in \bigcup_{n\in\Nat}\entspace^n$
returns the weight of the instance $\traceb \in \instances{\enta}$ in the support of $\tree$,
if it exists; and returns $0$ otherwise.
Formally,
\[
  \extree:\enta \mapsto \max\{ \tree(\traceb) \mid \traceb \in \instances{\enta} \}
\]
Note that by \cref{prop: instances and tree representable},
there is at most one instance of $\enta$ that is in the support of $\tree$.


\begin{proposition}
  \label{prop: tree and extree}
  For any $n\in\Nat$ and any tree representable function $\tree$,
  $\measure{\entspace^n}(\nsupport{n}{\extree})
  = \measure{\traces}(\bigcup_{i=1}^n \nsupport{i}{\tree})$.
\end{proposition}

\begin{proof}
  Let $\pi:\set{1, \dots, n} \to \set{\Real, \Bool}$ denote the measurable set
  $\pi(1) \times \pi(2) \times \dots \times \pi(n) \subseteq (\Real \cup \Bool)^n$, and
  $\inv{\pi}$ be the ``inverse'' of $\pi$,
  i.e.~for all $i$, $\inv{\pi}(i) = (\Real \cup \Bool) \setminus \pi(i)$.
  Let $S$ be the set containing all such subsets of $(\Real \cup \Bool)^n$.
  Then, for any $\traceset \in \algebra{(\Real \cup \Bool)^n}$,
  $\bigcup_{\pi \in S} \zip(\traceset \cap \pi, \inv{\pi})
  = \bigcup_{\pi \in S} \set{\zip(\traceb, \traceb') \in \entspace^n \mid
  \traceb \in \traceset \cap \pi, \traceb' \in \inv{\pi})}$\footnote{
  We write
  $\zip(L_1,L_2) := \set{\zip(\ell_1, \ell_2) \mid \ell_1 \in L_1, \ell_2 \in L_2} $
  for any sets $L_1, L_2$ of lists.
  }
  is the set containing all $n$-length entropy traces which has at least one instance
  that is in $\traceset$.

  Let $i \in \Nat$.
  We first show that for all $\pi \in S$,
  $\zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})$ are disjoint.
  Let $\pi_1, \pi_2 \in S$ be such that
  $\enta \in \zip(\nsupport{i}{\tree} \cap \pi_1, \inv{\pi_1}) \cap
  \zip(\nsupport{i}{\tree} \cap \pi_2, \inv{\pi_2})$.
  Then, at least one instance $\traceb_1$ of $\enta$ is in $\nsupport{i}{\tree} \cap \pi_1$ and
  similarly at least one instance $\traceb_2$ of $\enta$ is in $\nsupport{i}{\tree} \cap \pi_2$.
  By \cref{prop: instances and tree representable}, $\traceb_1 = \traceb_2$
  and hence $\pi_1 = \pi_2$.

  Since {$\zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})$ are disjoint} for all $\pi \in S$,
  we have
  \begin{align*}
    \measure{\entspace^i}(\bigcup_{\pi \in S} \zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi}))
    & =
    \sum_{\pi \in S} \measure{\entspace^i}(\zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})) \\
    & =
    \sum_{\pi \in S} \measure{\pi}(\nsupport{i}{\tree} \cap \pi) \cdot \measure{\inv{\pi}}(\inv{\pi}) \\
    & =
    \sum_{\pi \in S} \measure{\pi}(\nsupport{i}{\tree} \cap \pi) \\
    & =
    \sum_{\pi \in S} \measure{(\Real \cup \Bool)^i}(\nsupport{i}{\tree} \cap \pi) \\
    & =
    \measure{(\Real \cup \Bool)^i}(\nsupport{i}{\tree}).
  \end{align*}

  Finally, for any $n\in\Nat$,
  we can write $\nsupport{n}{\extree}$ as the disjoint union
  $\bigcup_{i=1}^n
  (\bigcup_{\pi \in S} \zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})) \times \entspace^{n-i}$
  and have
  \begin{align*}
    \measure{\entspace^n}(\nsupport{n}{\extree})
    & =
    \measure{\entspace^n}\Big(\bigcup_{i=1}^n
      (\bigcup_{\pi \in S} \zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})) \times \entspace^{n-i}
    \Big) \\
    & =
    \sum_{i=1}^n
    \measure{\entspace^n}\Big(
      (\bigcup_{\pi \in S} \zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})) \times \entspace^{n-i}
    \Big) \\
    & =
    \sum_{i=1}^n
    \measure{\entspace^i}\Big(
      \bigcup_{\pi \in S} \zip(\nsupport{i}{\tree} \cap \pi, \inv{\pi})
    \Big) \\
    & =
    \sum_{i=1}^n \measure{(\Real \cup \Bool)^i}(\nsupport{i}{\tree}) \tag{By above} \\
    & =
    \sum_{i=1}^n \measure{\traces}(\nsupport{i}{\tree}) \\
    & =
    \measure{\traces}(\bigcup_{i=1}^n \nsupport{i}{\tree}) \\
    & =
    \measure{\traces}(\support{\tree})
  \end{align*}
\end{proof}

\paragraph{Extension of Auxiliary Kernels}

Secondly, we also define an \defn{extension} of the family
$\set{\nauxkernel{n}:\entspace^n \kernelto\auxspace^n}$ of auxiliary kernels
as the kernel $\exauxkernel:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} \auxspace^n$
which given an entropy trace $\enta \in \bigcup_{n\in\Nat} \entspace^n$ with
$\traceb \in \instances{\enta} \cap \support{\tree}$,
returns an auxiliary variable $\auxa$ where
the first $\len{\traceb}$-th components of $\auxa$ has distribution
$\nauxkernel{\len{\traceb}}(\range{\enta}{1}{\len{\traceb}}, \placeholder)$ and
the rest of the components has the stock distribution $\measure{\auxspace}$.
Formally,
\[
  \exauxkernel: (\enta, \auxseta) \mapsto
  \begin{cases}
    \expandint{\auxseta}{\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}{\measure{\auxspace^{n}}}{\auxa} & \text{if } \traceb \in \instances{\enta} \cap \support{\tree} \text{ and } k = \len{\traceb} \\
    \measure{\auxspace^n}(\auxseta) & \text{otherwise.}
  \end{cases}
\]

With these extensions,
we present the pseudocode of the Hybrid NP-iMCMC sampler in \cref{alg: np-imcmc (hybrid)}.

Line 3 to 10 forms an entropy trace $\enta_0 \in \bigcup_{n\in\Nat}\entspace^n$ by
  pairing each value $\seqindex{\traceb_0}{i}$ in $\traceb_0$ with
  a randomly drawn value $\trace$ of the other type to make a pair
  $(\seqindex{\traceb_0}{i}, \trace)$ or $(\trace, \seqindex{\traceb_0}{i})$.
Line 11 samples a value $\auxa_0$ in the auxiliary space $\auxspace^n$
  from the auxiliary kernel $\nauxkernel{n}:\entspace^n \kernelto \auxspace^n$
  applied to the current sample $\enta_0$ where $n = \len{\enta_0}$.
Line 12 computes the new state $(\enta,\auxa)$
  by applying the involution $\ninvo{n}$ on $\entspace^n\times \auxspace^n$
  to the \emph{initial state} $(\enta_0,\auxa_0)$ where $n = \len{\enta_0}$.
Line 13 to 17 tests whether the program $\terma$ terminates (and returns a value)
  on the trace specified by one of the instances $\traceb$ of the sample-component $\enta$
  of the new state.
  (This can be done by checking if $\enta$ is in the support of the extension $\extree$.)
  If so, proceed to the next step;
  otherwise
  it extends the initial state to $(\enta_0 \concat [\entelem],\auxa_0 \concat [\auxelem])$
  where $\entelem$ and $\auxelem$ are values drawn randomly
  from $\measure{\entspace}$ and $\measure{\auxspace}$ and
  computes the proposal state $(\enta, \auxa)$ by
  applying the involution $\ninvo{n+1}$
  to the extended initial state $(\enta_0 \concat [\entelem],\auxa_0 \concat [\auxelem])$.
Line 18 to 23 accepts and propose $\traceb \in \nsupport{k}{\tree} \cap \instances{\enta}$
  as the next sample with probability given by
  \begin{align*}
  \min\bigg\{1; \;
  &\frac
    {\tree{(\traceb)}\cdot\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})\cdot\nstockpdf{n}(\enta, \auxa)}
    {\tree{(\traceb_0)}\cdot\nauxpdf{k_0}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0})\cdot\nstockpdf{n}(\enta_0, \auxa_0)}
  \cdot \abs{\det(\grad{\ninvo{\len{\enta_0}}(\enta_0, \auxa_0)})}\bigg\} \\
  =
  \min\bigg\{1; \;
  &\frac
    {\extree{(\enta)}\cdot\exauxpdf(\enta, \auxa)\cdot\nstockpdf{n}(\enta, \auxa)}
    {\extree{(\enta_0)}\cdot\exauxpdf(\enta_0, \auxa_0)\cdot\nstockpdf{n}(\enta_0, \auxa_0)}
  \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}
  \end{align*}
  where $k = \len{\traceb}$, $k_0 = \len{\traceb_0}$, and $n = \len{\enta_0}$;
  otherwise reject the proposal and repeat $\traceb_0 \in \support{\tree}$.

\begin{algorithm}
\caption{Hybrid NP-iMCMC}
\label{alg: np-imcmc (hybrid)}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0 : \traces$,
    tree representable function $\tree :\traces \to \pReal$,
    family of involutions $\set{\ninvo{n} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    family of auxiliary kernels $\set{\nauxkernel{n} : \entspace^n \kernelto \auxspace^n}_n$ }
  \STATE \Output{Next sample $\traceb : \traces$}
  % \BlankLine
  \STATE $\enta_0 = \emptytrace$ \label{alg line: fill start}
  \FOR{$i = 1$ to $\len{\traceb_0}$}
    \IF{$\seqindex{\traceb_0}{i} \in \Real$}
      \STATE $\boola \sim \measure{\Bool}$; $\enta_0 = \enta_0 \concat [(\seqindex{\traceb_0}{i}, \boola)] $
    \ELSE[$\seqindex{\traceb_0}{i} \in \Bool$]
      \STATE $\reala \sim \measure{\Real}$; $\enta_0 = \enta_0 \concat [(\reala, \seqindex{\traceb_0}{i})] $
    \ENDIF
  \ENDFOR \label{alg line: fill end}
  % \COMMENT{$\enta_0$ is the entropy trace formed from $\traceb_0$ by pairing each value with randomly drawn ``partner''}
  \STATE $\auxa_0 \sim \cauxkernel{\len{\enta_0}}(\enta_0, \placeholder)$
  % \COMMENT{sample a value $\auxa_0 \in \auxspace^n$ from the cumulative auxiliary kernel $\cauxkernel{n}$ applied to $\enta_0$ (\cref{np-imcmc step: aux sample})}
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  % \COMMENT{compute the new state $(\enta,\auxa)$ by applying the involution $\ninvo{n}$ to the \emph{initial state} $(\enta_0,\auxa_0)$ where $n = \len{\enta_0}$. (\cref{np-imcmc step: involution})}
  \WHILE{$\enta \not\in\support{\extree} $}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % $\auxelem \sim \nauxkernel{\len{\enta_0}+1}(\entelem, \placeholder)$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    \label{line: Vanilla NP-iMCMC extend initial state}
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {\extree{(\enta)}\cdot\exauxpdf(\enta, \auxa)\cdot\nstockpdf{n}(\enta, \auxa)}
      {\extree{(\enta_0)}\cdot\exauxpdf(\enta_0, \auxa_0)\cdot\nstockpdf{n}(\enta_0, \auxa_0)}
    \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}
    $ where $n = \len{\enta_0}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\traceb \in \instances{\enta} \cap \support{\tree}$
  \ELSE
    \STATE \Return $\traceb \in \instances{\enta_0} \cap \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

% Flow diagram for np-imcmc
\iffalse
\begin{tikzpicture}[node distance = 3cm, scale=0.8, every node/.style={scale=0.8}]
  % Place nodes
  \node [] (input) {};
  % \node [block, below of=input, node distance = 1.5cm] (fill) {fill $\traceb_0$};
  \node [block, below of=input, node distance = 2cm] (aux)
    {Sample auxiliary variable $\auxa_0$ (\cref{line: Vanilla NP-iMCMC initialise aux var})};
  \node [block, below of=aux, node distance = 3.5cm] (inv)
    {Run involution $\ninvo{\len{\enta_0}}$ (\cref{line: Vanilla NP-iMCMC run involution,line: Vanilla NP-iMCMC loop run involution})};
  \node [decision, below of=inv] (good)
    {$\trunc{\len{\enta}}(\enta) > 0$? (\cref{line: Vanilla NP-iMCMC loop start})};
  \node [block, right of=good, yshift=1.5cm] (extend)
    {Extend initial state $(\enta_0,\auxa_0)$ with randomly drawn values (\cref{line: Vanilla NP-iMCMC extend initial state})};
  \node [draw=blue, algblock, fit= (inv) (good) (extend),
    label=north:{\hspace{2cm} \color{blue} Proposal (\cref{line: Vanilla NP-iMCMC run involution} to \cref{line: Vanilla NP-iMCMC loop end})}] (np-inv) {};
  \node [block, below of=good, node distance = 4cm] (mh)
    {Compute acceptance ratio (\cref{line: Vanilla NP-iMCMC acceptance})};
  \node [block, below of=mh] (empty)
    {Accept $\range{\enta}{1}{k}$ where $\tree(\range{\enta}{1}{k}) > 0$ with probability $P$};
  \node [right of=empty,node distance = 2.5cm] (output) {};

  % Draw edges
  \path [line] (input) edge node [label={0:$\enta_0 := \traceb_0$}] {} (aux);
  \path [line] (aux) edge node [label={10:$(\enta_0,\auxa_0)$}] {} (inv);
  \path [line] (inv) edge node [label=0:{$(\enta,\auxa)$}] {} (good);
  \path [line] (good) -| node [label={0:$(\enta_0,\auxa_0)$}] {} (extend);
  \path [line] (extend) |- node [label={0:$(\enta_0,\auxa_0)$}] {} (inv);
  \path [line] (good) -- node [label={0:$(\enta,\auxa)$ and $(\enta_0,\auxa_0)$}] {} (mh);
  \path [line] (mh) -- node [label={0:$P$}] {} (empty);
  \path [line] (empty) -- node [label=above:{$\traceb$}] {} (output);
\end{tikzpicture}
\fi

\subsection{Correctness}
\label{app: correctness}

We show that the Hybrid NP-iMCMC algorithm (\cref{alg: np-imcmc (hybrid)}) is correct,
in the sense that
the invariant distribution of the Markov chain
generated by iterating \cref{alg: np-imcmc (hybrid)} coincide with the target distribution,
specified by
\begin{align*}
  {\tdist:}\
  {\Sigma_{\traces}}& \longrightarrow {\pReal} \\
  {U} & \longmapsto {\frac{1}{Z}\shortint{U}{\tree}{\measure{\traces}}}
  \qquad\text{where }
  Z := \shortint{\traces}{\tree}{\measure{\traces}}.
\end{align*}

We justify the Hybrid NP-iMCMC sampler (\cref{alg: np-imcmc (hybrid)}) by
proving the following three theorems in \cref{sec: almost sure termination,sec: invariant distribution}:

\begin{restatable*}[AST]{theorem}{ast}
  \label{theorem: np-imcmc is ast}
  Given all inputs satisfy \allvass{},
  \cref{alg: np-imcmc (hybrid)} almost surely terminates.
\end{restatable*}

\begin{restatable*}[Invariant]{theorem}{hinvariant}
  \label{theorem: marginalised distribution is the target distribution}
  Given all inputs satisfy \allvass{},
  $\tdist$ is the invariant distribution of the Markov chain generated by iterating the \cref{alg: np-imcmc (hybrid)}.
\end{restatable*}

% \begin{restatable*}[Convergence]{theorem}{convergence}
% % \begin{theorem}
%   \label{thm: np-imcmc correct}
%   Given all inputs satisfy \allvass{} and \allcass{},
%   the Markov chain generated by
%   iterating \cref{alg: np-imcmc (hybrid)} converges
%   to the target distribution $\tdist$,
%   i.e.~for all $\state$,
%   $\lim_{n\to\infty} \norm{\transkernel{}^n(\state,\placeholder)-\tdist} = 0$
%   with $\norm{\placeholder}$ denoting total variation distance
%   and $\transkernel{}$ is the transition kernel described by \cref{alg: np-imcmc (hybrid)}.
% % \end{theorem}
% \end{restatable*}

\subsubsection{Almost sure termination}
\label{sec: almost sure termination}
\input{section/almost-sure-termination}

\subsubsection{Invariant Distribution}
\label{sec: invariant distribution}
\input{section/invariant}

% \subsubsection{Convergence}
% \label{sec: convergence}
% \input{section/convergence}
% \input{section/new-convergence}


==> section/np-la-hmc.tex <==
% !TEX root = ./../icml2022.tex

Here we use the NP-iMCMC framework described in \cref{sec: np-imcmc}
and some of the special ingredients presented in \cref{sec: combination}
to construct a nonparametric extension of the Lookahead HMC algorithm \cite{DBLP:conf/icml/Sohl-DicksteinMD14}.

\subsection{Look Ahead HMC}

Given the previous sample-momentum state $(x_0, v_0)$,
the Look Ahead HMC proposes the next state $(x,v)$ using Hamiltonian motions with three special ingredients:
\begin{itemize}
    \item The initial momentum $v_0'$ is set to be a sample
    from some distribution conditioned on the previous momentum $v_0$.

    \item After \emph{each} leapfrog step, the current state $(x,v)$ is proposed
    and accepted with the usual acceptance probability.
    Hence more steps are taken only if the current state is rejected.
    If all proposals are rejected, within $L$ steps, then the previous state $(x_0, v_0)$ will be re-used.

    \item The momentum $v$ of an accepted proposal $(x,v)$ is preserved but the momentum $v_0$ of the previous state $(x_0, v_0)$ is flipped.
\end{itemize}

Each of these can be represented as an iMCMC kernel, and thus
Look Ahead HMC can been as a composition of three iMCMC kernel as explained in Section B.13 in \cite{DBLP:conf/icml/NeklyudovWEV20}.

\subsection{Nonparametric}

To consider the nonparametric extension of Look Ahead HMC,
we extend all three of these iMCMC kernels.

\paragraph{NP-iMCMC kernel $\kappa_1$}

The first kernel corresponds to the first ``special ingredient'' of Look Ahead HMC

\begin{example}[LMH]
Using the state-dependent mixture method, we can design a version of
the Lightweight Metropolis Hastings (LMH) (also known as single-site MH or random database sampling) \cite{DBLP:journals/jmlr/WingateSG11},
the popular trans-dimensional sampler in probabilistic programming,
that updates a single site of the current sample.

For each $i \in \Nat$, let $\imcmca_i$ be an NP-iMCMC update with
the single site swap $\ninvo{n}_i(\enta, \auxa) := (\rindex{\enta}{i}{\seqindex{\auxa}{i}},\rindex{\auxa}{i}{\seqindex{\enta}{i}})$ for $n \leq i$ and $\ninvo{n}(\enta, \auxa) := (\enta, \auxa)$ otherwise,
as involution and the multivariate normal distribution
$\nauxkernel{n}_i(\enta) := \Gau_{\len{\enta}}$ as the auxiliary kernel.

Then, the state-dependent mixture of $\set{\imcmca_i}_{i\in\Nat}$ with the mixture kernel
$\mixkernel(\enta) := \Uni(\set{1, \dots, \len{\enta}})$ updates the current sample $\enta_0$ as follows:
\begin{compactenum}[1.]
  \item $i \sim \Uni(\set{1,\dots, \len{\enta_0}})$: pick a site $i$ to update.

  \item $\auxa_0 \sim \Gau_{\len{\enta}}$: sample a value $\auxa_0$ to update the site $i$.

  \item $(\enta,\auxa) \leftarrow (\rindex{\enta_0}{i}{\seqindex{\auxa_0}{i}},\rindex{\auxa_0}{i}{\seqindex{\enta_0}{i}})$: swap the $i$-th site of $\enta_0$ and $\auxa_0$.

  \item Test whether the program $\terma$ terminates \changed[lo]{(and returns a value)} with \changed[cm]{a trace specified by} the sample-component $\enta$ of the new state, or one of its prefixes. This can be done by checking if $\enta$ is in the support of the extension $\extree$.
  If so, proceed to the next step;
  otherwise
  \begin{compactitem}
    \item $(\enta_0, \auxa_0) \leftarrow (\enta_0 \concat [\entelem],\auxa_0 \concat [\auxelem])$: extend the initial state to $(\enta_0 \concat [\entelem],\auxa_0 \concat [\auxelem])$ where $\entelem$ and $\auxelem$ are values drawn randomly from $\measure{\entspace}$ and $\measure{\auxspace}$,
    \item goto Step 3.
  \end{compactitem}

  \item Accept the proposed sample $\range{\enta}{1}{k} \in \support{\tree}$ as the next step with probability given by
  \begin{align*}
  \min\bigg\{1; \;
  &\frac
    {\tree{(\range{\enta}{1}{k})}\cdot\pdfGau_{k}(\range{\auxa}{1}{k}) \cdot 1/k}
    {\tree{(\range{\enta_0}{1}{k_0})}\cdot\pdfGau_{k_0}(\range{\auxa_0}{1}{k_0}) \cdot 1/k_0}
  \bigg\}
  \end{align*}
  otherwise
  \changed[fz]{reject the proposal and repeat $\range{\enta_0}{1}{k_0} \in \support{\tree}$.}
\end{compactenum}
% After randomly picking a variable (site) to resample from a given trace, the most basic version of LMH would run the program afresh from that point onwards, dropping all subsequent samples.
% The algorithm is still correct if the remainder is sampled afresh whenever the path changes or the change leaves the trace with zero density.
% A more efficient implementation would reuse samples (with rescoring) whenever possible.
% By contrast, \cref{alg: LMH} is a variant of LMH that reuses \emph{all} remainder samples from the given trace.
\end{example}

\begin{example}[NP-Gibbs with fixed scan]
\label{eg: np-gibbs with fixed scan}
Recall in \cref{eg: np-gibbs} we show how the Gibbs sampler can be extended to update the $i$-th component of a sample from nonparametric models.
In order to update all components of the sample, it is common for a Gibbs sampler to iterate through every component of the current sample.\footnote{Here, we consider the so-called ``fixed scan'' Gibbs sampler. There are other common Gibbs samplers, such as the ``random scan'', which is a state-independent mixture of the Gibbs updates.}
We can apply the same idea to NP-Gibbs by iterating through every component of the current sample.
As noted in \cref{eg: np-gibbs}, it is important that the position of updated component to be smaller than or equal to the size of the sample.
Hence, a fixed scan NP-Gibbs updates the current sample $\enta_0$ as follows:
\begin{compactenum}[1.]
  \item Initialise the position $i$ of the updated component to be $1$ and $\enta = \enta_0$.

  \item Test whether $i > \len{\enta}$. If so, return $\enta$ as the next sample; otherwise
  \begin{compactitem}
    \item Update the $i$-th component of $\enta$ via the NP-Gibbs (\cref{eg: np-gibbs}) method to obtain a new sample $\enta$
    \item Increment $i$ to $i+1$
    \item goto 2.
  \end{compactitem}
\end{compactenum}
\end{example}


==> section/proofs.tex <==
% !TEX root = ./../icml2022.tex


==> section/variants.tex <==
% !TEX root = ./../icml2022.tex

In this section, we look at different variants of the NP-iMCMC sampler (\cref{alg: np-imcmc});
all aims to sample from
the tree representable,
integrable (\cref{vass: integrable tree}) and
almost surely terminating (\cref{vass: almost surely terminating tree})
target density function $\tree$ on $\traces$.

\iffalse
Recall the definition of the extension
$\extree:\traces \to \pReal$ of a tree representable function $\tree$ is
$\extree(\traceb) := \max\{ \tree(\range{\traceb}{1}{i}) \mid i=1, \dots,\len{\traceb}\}$;
and
the definition of the extended auxiliary kernel
$\exauxkernel:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} \auxspace^n$ is
$\exauxkernel(\enta, \auxseta) := \expandint{\auxseta}{\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}{\measure{\auxspace^{n}}}{\auxa}$ for $\range{\enta}{1}{k} \in \support{\tree}$ and
$\exauxkernel(\enta, \auxseta) := \measure{\auxspace^n}(\auxseta)$ otherwise.
\fi

\begin{algorithm}
\caption{NP-iMCMC}
\label{alg: np-imcmc}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of involutions $\set{\ninvo{n} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    a family of auxiliary kernels $\set{\nauxkernel{n} : \entspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $\auxa_0 \sim \nauxkernel{\len{\enta_0}}(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {\tree{(\range{\enta}{1}{k})}\cdot\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k}) \cdot \nstockpdf{n}({\enta},{\auxa}) }
      {\tree{(\range{\enta_0}{1}{k_0})}\cdot\nauxpdf{k_0}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0}) \cdot \nstockpdf{n}({\enta_0},{\auxa_0}) }
    \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$ and
    $n = \len{\enta}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\subsection{State-dependent mixture}
\label{app: state dependent mixture of np-imcmc}

Let $\set{\imcmca_\mixa}_{\mixa\in \mixspace}$ be a family of NP-iMCMC updates for the target density function $\tree$.
We can see each $\imcmca_\mixa$ as an instance of \cref{alg: np-imcmc} with inputs:
$\tree$;
a family of involutions $\set{\ninvo{n}_\mixa:\entspace^n \times\auxspace^n \to \entspace^n \times\auxspace^n }_{n\in\Nat}$ that satisfies the \invoass{} (\cref{vass: partial block diagonal inv}); and
a family of auxiliary kernels $\set{\nauxkernel{n}_\mixa:\entspace^n \kernelto\auxspace^n}_{n\in\Nat}$ where each is probabilistic and has pdf $\nauxpdf{n}_\mixa$.

\iffalse
In this case, for each $\mixa \in \mixspace$, we can define an extended auxiliary kernel $\exauxkernel_\mixa:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} \auxspace^n$ as
$\exauxkernel_\mixa(\enta, \auxseta) := \expandint{\auxseta}{\nauxpdf{k}_\mixa(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}{\measure{\auxspace^{n}}}{\auxa}$ for $\range{\enta}{1}{k} \in \support{\tree}$ and
$\exauxkernel_\mixa(\enta, \auxseta) := \measure{\auxspace^n}(\auxseta)$ otherwise.
\fi

Let $(\mixspace, \algebra{\mixspace}, \measure{\mixspace})$ be a probability measure space;
and $\mixkernel: \support{\tree} \kernelto \mixspace$ be a probability kernel, i.e.~$\mixkernel(\traceb, \mixspace) = 1$ for each $\traceb \in \support{\tree}$, and has pdf $\mixpdf:\support{\tree} \times \mixspace \to \pReal$.

A \defn{state-dependent mixture} of NP-iMCMC updates $\set{\imcmca_\mixa}_{\mixa\in \mixspace}$ runs a random one of these updates by generating a mixture variable $\mixa\in \mixspace$ from the distribution $\mixkernel(\traceb, \placeholder)$ on $\mixspace$, and run $\imcmca_\mixa$ with an acceptance ratio
\[
  \min \left\{1,
    \displaystyle\frac
      {
        \tree{(\range{\enta}{1}{k})}\cdot\nauxpdf{k}_{\mixa}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})
        \cdot \mixpdf(\range{\enta}{1}{k}, \mixa)
      }
      {
        \tree{(\range{\enta_0}{1}{k_0})}\cdot\nauxpdf{k_0}_{\mixa}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0})
        \cdot \mixpdf(\range{\enta_0}{1}{k_0}, \mixa)
      }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta}}_{\mixa}(\enta_0, \auxa_0)})}
    \right\}
\]
where
$(\enta_0, \auxa_0)$ is the current state with
$\range{\enta_0}{1}{k_0} \in \support{\tree}$, and
$({\enta},{\auxa})$ (which is equals to $\invo_\mixa(\enta_0, \auxa_0)$) is the proposed state with
$\range{\enta}{1}{k} \in \support{\tree}$.
Putting everything together, \cref{alg: state dependent mixture of np-imcmc} gives the pseudocode for a state-dependent mixture of NP-iMCMC updates.

\begin{algorithm}
\caption{State-dependent mixture of NP-iMCMC}
\label{alg: state dependent mixture of np-imcmc}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    tree representable function $\tree :\traces \to \pReal$,
    family of NP-iMCMC updates $\set{\imcmca_\mixa}_{\mixa\in \mixspace}$
    (where $\imcmca_\mixa$ is an instance of \cref{alg: np-imcmc} with inputs:
    a family of involutions $\set{\ninvo{n}_\mixa : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    a family of auxiliary kernels $\set{\nauxkernel{n}_\mixa : \entspace^n \kernelto \auxspace^n}_n$ ),
    mixture kernel $\mixkernel: \support{\tree} \kernelto \mixspace$
  }
  \STATE \Output{Next sample $\traceb:\traces$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $\mixa \sim \mixkernel(\enta_0, \placeholder)$
  \STATE $\auxa_0 \sim \nauxkernel{\len{\enta_0}}_\mixa(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}_\mixa(\enta_0,\auxa_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}_\mixa(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min \left\{1,
      \displaystyle\frac
        {
          \tree{(\range{\enta}{1}{k})}\cdot\nauxpdf{k}_{\mixa}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})
          \cdot \nstockpdf{n}(\enta, \auxa)
          \cdot \mixpdf(\range{\enta}{1}{k}, \mixa)
        }
        {
          \tree{(\range{\enta_0}{1}{k_0})}\cdot\nauxpdf{k_0}_{\mixa}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0})
          \cdot \nstockpdf{n}(\enta_0, \auxa_0)
          \cdot \mixpdf(\range{\enta_0}{1}{k_0}, \mixa)
        }
      \cdot \abs{\det(\grad{\ninvo{n}_{\mixa}(\enta_0, \auxa_0)})}
      \right\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
    and $n = \len{\enta}$
    % \min \left\{1,
    %   \displaystyle\frac
    %     {\extree(\enta)\cdot \exauxpdf({\enta},{\auxa}) \cdot \mixpdf(\traceb, \mixa) }
    %     {\extree(\enta_0)\cdot \exauxpdf({\enta_0},{\auxa_0}) \cdot \mixpdf(\traceb_0, \mixa) }
    %   \abs{\det{\big(\grad{\ninvo{\len{\enta_0}}_\mixa}(\enta_0,\auxa_0)\big)}}
    %   \right\}$ where $\traceb = \range{\enta}{1}{k} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\iffalse
\subsubsection*{Correctness}

We show the correctness of the mixture update (\cref{alg: state dependent mixture of np-imcmc}) in two steps:
(1) define an instance of NP-iMCMC update (\cref{alg: np-imcmc with mixture inputs}),
which is shown to be correct (\cref{thm: np-imcmc correct}) as long as the assumptions stated in \cref{sec: assumptions} are satisfied;
(2) argue that the mixture update is a simplified version of \cref{alg: np-imcmc with mixture inputs}.

The instance of NP-iMCMC update argument the auxiliary space $\auxspace$ with the mixture space $\mixspace$,
making $(\enta, \auxa, \mixb) \in \entspace^n \times \auxspace^n \times \mixspace^n$ a state which the first component of $\mixb$ indicates which update in $\set{\imcmca_\mixa}_{\mixa \in \mixspace} $ will be used.

Formally, this update takes as involution $\new{\ninvo{n}}$ on $\entspace^n \times \auxspace^n \times \mixspace^n$
such that
$\new{\ninvo{n}}(\enta, \auxa, \mixb) = (\enta', \auxa', \mixb)$ where $(\enta', \auxa') = \ninvo{n}_{\seqindex{\mixb}{1}} (\enta, \auxa)$ for each dimension $n\in\Nat$; and
auxiliary kernel $\new{\nauxkernel{n}}:\entspace^n \kernelto \auxspace^n \times \mixspace^n$ such that
\[
  \new{\nauxkernel{n}}(\enta, \auxseta) :=
  \begin{cases}
    \expandint{\auxseta}{
      \mixpdf(\range{\enta}{1}{k}, \seqindex{\mixb}{1}) \cdot \nauxpdf{n}_{\seqindex{\mixb}{1}}(\enta, \auxa)
    }{(\measure{\auxspace^n}\times\measure{\mixspace^n})}{(\auxa, \mixb)}
    & \text{if }\range{\enta}{1}{k} \in \support{\tree} \\
    (\measure{\auxspace^n}\times\measure{\mixspace^n})(\auxseta) & \text{otherwise.}
  \end{cases}
\]
Since $\mixpdf$ and $\nauxpdf{n}$ are pdfs, $\new{\nauxkernel{n}}$ is a probability kernel with pdf $\new{\nauxpdf{n}} : \entspace^n \times \auxspace^n \times \mixspace^n \to \pReal$ such that
\[
  \new{\nauxpdf{n}}(\enta, \auxa, \mixb) :=
  \begin{cases}
    \mixpdf(\range{\enta}{1}{k}, \seqindex{\mixb}{1}) \cdot \nauxpdf{n}_{\seqindex{\mixb}{1}}(\enta, \auxa)
    & \text{if } \range{\enta}{1}{k} \in \support{\tree} \\
    1 & \text{otherwise.}
  \end{cases}
\]
\fi

\iffalse
We follow the procedure and define the extended auxiliary kernel
$\new{\exauxkernel}:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} (\auxspace^n\times\mixspace^n)$ as
\[
  \new{\exauxkernel}(\enta, \auxseta) :=
  \begin{cases}
    \expandint{\auxseta}{
    \mixpdf(\range{\enta}{1}{k}, \seqindex{\mixb}{1}) \cdot
    \nauxpdf{k}_{\seqindex{\mixb}{1}}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})
    }{(\measure{\auxspace^{n}} \times \measure{\mixspace^{n}})}{\auxa}
    & \text{if } \range{\enta}{1}{k} \in \support{\tree} \\
    (\measure{\auxspace^n}\times\measure{\mixspace^n})(\auxseta)
    & \text{otherwise.}
  \end{cases}
\]
\fi
\iffalse
It is easy to check that $\new{\ninvo{n}}$ satisfies the \invoass{}.
With these inputs, we can write the NP-iMCMC update (\cref{alg: np-imcmc with mixture inputs}) which, by \cref{thm: np-imcmc correct}, correctly samples from the target density function $\tree$.

To see why the mixture of NP-iMCMC updates (\cref{alg: state dependent mixture of np-imcmc}) is a simplified version of \cref{alg: np-imcmc with mixture inputs}, consider the mixture variable $\mixb \in \mixspace^n$ in \cref{alg: np-imcmc with mixture inputs}.
It is easy to see that only the first component of $\mixb$ has effects on the update.
So, the rest of the components are redundant and can be removed.
Writing the first component of $\mixb$ as $\mixa$, the resulting algorithm becomes \cref{alg: state dependent mixture of np-imcmc}.

\begin{algorithm}
\caption{NP-iMCMC with mixture inputs}
\label{alg: np-imcmc with mixture inputs}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of involutions $\set{\new{\ninvo{n}} : \entspace^n \times \auxspace^n \times \mixspace^n \to \entspace^n \times \auxspace^n \times \mixspace^n}_n$ and
    a family of auxiliary kernels $\set{\new{\nauxkernel{n}} : \entspace^n \kernelto \auxspace^n \times \mixspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $(\auxa_0, \mixb_0) \sim \new{\nauxkernel{\len{\enta_0}}}(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa, \mixb) = \new{\ninvo{\len{\enta_0}}}(\enta_0,\auxa_0,\mixb_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    $\mixelem \sim \measure{\mixspace}$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0, \mixb_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem], \mixb_0 \concat [\mixelem])$
    % run involution
    \STATE $(\enta,\auxa, \mixb) = \new{\ninvo{\len{\enta_0}}}(\enta_0,\auxa_0,\mixb_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {\tree{(\range{\enta}{1}{k})}\cdot\new{\nauxpdf{k}}(\range{\enta}{1}{k}, \range{\auxa}{1}{k}, \range{\mixb}{1}{k})}
      {\tree{(\range{\enta_0}{1}{k_0})}\cdot\new{\nauxpdf{k_0}}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0}, \range{\mixb_0}{1}{k_0}) }
    \cdot \abs{\det(\grad{\new{\ninvo{\len{\enta}}}(\enta_0, \auxa_0, \mixb_0)})}\bigg\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}
\fi

\subsection{Auxiliary direction}
\label{app: auxiliary direction (np-imcmc)}

Let $\set{f^{(n)}:\entspace^n \times\auxspace^n \to \entspace^n \times\auxspace^n }_{n\in\Nat}$ be a family of non-involutive bijections where $\set{f^{(n)}}_n$ and $\set{\inv{f^{(n)}}}_n$ satisfy the \invoass{} (\cref{vass: partial block diagonal inv}) and
$\set{\nauxkernel{n}:\entspace^n \kernelto\auxspace^n}_{n\in\Nat}$ be a family of auxiliary kernels
where each is probabilistic and has pdf $\nauxpdf{n}$.
\iffalse
Then, we can define an extended auxiliary kernel $\exauxkernel:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} \auxspace^n$ as
$\exauxkernel(\enta, \auxseta) := \expandint{\auxseta}{\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}{\measure{\auxspace^{n}}}{\auxa}$ for $\range{\enta}{1}{k} \in \support{\tree}$ and
$\exauxkernel(\enta, \auxseta) := \measure{\auxspace^n}(\auxseta)$ otherwise.
\fi

Let $\dirspace := \set{+, -}$ be the direction space equipped with
the $\sigma$-algebra $\algebra{\dirspace} := \powerset(\set{+,-})$; and
the discrete uniform distribution $\measure{\dirspace} := \Uni(\set{+, -})$.

An NP-iMCMC update with \defn{auxiliary direction} proposes the state by generating
a direction variable $\dira\in \dirspace$ from the distribution $\measure{\dirspace}$ on $\dirspace$, and
applying $\set{f^{(n)}}_n$ if $\dira = +$ or $\set{\inv{f^{(n)}}}_n$ if $\dira = -$.
Putting everything together, \cref{alg: np-imcmc with auxiliary direction} gives the pseudocode for an NP-iMCMC update with auxiliary direction.

\begin{algorithm}
\caption{NP-iMCMC with auxiliary direction}
\label{alg: np-imcmc with auxiliary direction}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of non-involutive bijections $\set{f^{(n)} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    a family of auxiliary kernels $\set{\nauxkernel{n} : \entspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $\dira \sim \Uni(\set{+,-})$
  \STATE $\ninvo{n} = \begin{cases}
    f^{(n)} & \text{if } \dira = + \\
    \inv{f^{(n)}} & \text{if } \dira = -
  \end{cases} $ for all $n\in\Nat$
  % \IF{$\dira = +$}
  %   \STATE $\ninvo{n} = f^{(n)}$ for all $n\in\Nat$
  % \ELSE
  %   \STATE $\ninvo{n} = \inv{f^{(n)}}$ for all $n\in\Nat$
  % \ENDIF
  \STATE $\auxa_0 \sim \nauxkernel{\len{\enta_0}}(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \measure{\auxspace}$;
    % \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \nauxkernel{\len{\enta_0}+1}(\entelem, \placeholder)$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {
        \tree{(\range{\enta}{1}{k})}\cdot
        \nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k}) \cdot
        \nstockpdf{n}(\enta, \auxa)
      }
      {
        \tree{(\range{\enta_0}{1}{k_0})}\cdot
        \nauxpdf{k_0}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0}) \cdot
        \nstockpdf{n}(\enta_0, \auxa_0)
      }
    \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
    and $n = \len{\enta}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\iffalse
\subsubsection*{Correctness}

We show the correctness of the NP-iMCMC update with auxiliary direction (\cref{alg: np-imcmc with auxiliary direction}) in two steps:
(1) define an instance of NP-iMCMC update (\cref{alg: np-imcmc with directional inputs}),
which is shown to be correct (\cref{thm: np-imcmc correct}) as long as the assumptions in \cref{sec: assumptions} are satisfied;
(2) argue that the NP-iMCMC update with auxiliary direction is a simplified version of \cref{alg: np-imcmc with directional inputs}.

The instance of NP-iMCMC update argument the auxiliary space $\auxspace$ with the direction space $\dirspace$,
making $(\enta, \auxa, \dirb) \in \entspace^n \times \auxspace^n \times \dirspace^n$ a state which the first component of $\dirb$ indicates which function to be used.

Formally, this update takes as involution $\new{\ninvo{n}}$ on $\entspace^n \times \auxspace^n \times \dirspace^n$
such that
$\new{\ninvo{n}}(\enta, \auxa, \dirb) = (\enta', \auxa', \dirb')$ where
\[
  (\enta', \auxa') =
  \begin{cases}
    f^{(n)}(\enta, \auxa) & \text{if } \seqindex{\dirb}{1} = + \\
    \inv{f^{(n)}}(\enta, \auxa) & \text{if } \seqindex{\dirb}{1} = -
  \end{cases}
  \text{ and }
  \seqindex{\dirb'}{i} = \flip(\seqindex{\dirb}{i}) \text{ for all }i = 1,\dots, n
\]
for each dimension $n\in\Nat$;
and auxiliary kernel $\new{\nauxkernel{n}}:\entspace^n \kernelto \auxspace^n \times \dirspace^n$ such that
\[
  \new{\nauxkernel{n}}(\enta, \auxseta) :=
  \expandint{\dirspace^n}{
    \nauxkernel{n}(\enta, \set{\auxa \in \auxspace^n \mid (\auxa, \dirb) \in \auxseta})
  }{\measure{\dirspace^n}}{\dirb},
\]
which is probabilistic and
has pdf $\new{\nauxpdf{n}}$ on $\entspace^n \times \auxspace^n \times \dirspace^n$ such that
$\new{\nauxpdf{n}}(\enta, \auxa, \dirb) := {\nauxpdf{n}(\enta, \auxa)}$.

It is easy to check that $\new{\ninvo{n}}$ is involutive and satisfies the \invoass{}.
\iffalse
Moreover, for each $\enta \in \entspace^n$,
We follow the procedure and define the extended auxiliary kernel
$\new{\exauxkernel}:\bigcup_{n\in\Nat} \entspace^n \kernelto \bigcup_{n\in\Nat} (\auxspace^n\times\dirspace^n)$ as
\[
  \new{\exauxkernel}(\enta, \auxseta) :=
  \begin{cases}
    \displaystyle
    \expandint{\auxseta}{
    {\nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k})}
    }{(\measure{\auxspace^n}\times\measure{\dirspace^n})}{(\auxa,\dirb)}
    & \text{if } \range{\enta}{1}{k} \in \support{\tree} \text{ and } n = \len{\enta} \\
    (\measure{\auxspace^n}\times\measure{\dirspace^n})(\auxseta)
    & \text{otherwise.}
  \end{cases}
\]
\fi
With these inputs, we can write the NP-iMCMC update (\cref{alg: np-imcmc with directional inputs}) which, by \cref{thm: np-imcmc correct}, correctly samples from the target density function $\tree$.

To see why the NP-iMCMC update with auxiliary direction (\cref{alg: np-imcmc with auxiliary direction}) is a simplified version of \cref{alg: np-imcmc with directional inputs}, consider the direction variable $\dirb \in \dirspace^n$ in \cref{alg: np-imcmc with directional inputs}.
It is easy to see that only the first component of $\dirb$ has effects on the update.
So, the rest of the components are redundant and can be removed.
Writing the first component of $\dirb$ as $\dira$, the resulting algorithm becomes \cref{alg: np-imcmc with auxiliary direction}.

\begin{algorithm}
\caption{NP-iMCMC with directional inputs}
\label{alg: np-imcmc with directional inputs}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of involutions $\set{\new{\ninvo{n}} : \entspace^n \times \auxspace^n \times \dirspace^n \to \entspace^n \times \auxspace^n \times \dirspace^n}_n$ and
    a family of auxiliary kernels $\set{\new{\nauxkernel{n}} : \entspace^n \kernelto \auxspace^n \times \dirspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $(\auxa_0, \dirb_0) \sim \new{\nauxkernel{\len{\enta_0}}}(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa, \dirb) = \new{\ninvo{\len{\enta_0}}}(\enta_0,\auxa_0,\dirb_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    $\direlem \sim \measure{\dirspace}$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0, \dirb_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem], \dirb_0 \concat [\direlem])$
    % run involution
    \STATE $(\enta,\auxa, \dirb) = \new{\ninvo{\len{\enta_0}}}(\enta_0,\auxa_0,\dirb_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {\tree{(\range{\enta}{1}{k})}\cdot\new{\nauxpdf{k}}(\range{\enta}{1}{k}, \range{\auxa}{1}{k},\range{\dirb}{1}{k}) }
      {\tree{(\range{\enta_0}{1}{k_0})}\cdot\new{\nauxpdf{k_0}}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0},\range{\dirb_0}{1}{k_0}) }
    \cdot \abs{\det(\grad{\new{\ninvo{\len{\enta}}}(\enta_0, \auxa_0, \dirb_0)})}\bigg\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$
  \ENDIF
\end{algorithmic}
\end{algorithm}
\fi

\iffalse
\subsection{Composition of NP-iMCMC updates}

Similar to \cref{eg: composition of imcmc udpates}, we see how reversible chains (generated by the NP-iMCMC method) can be made into nonreversible ones.
\fi
\subsection{Persistent Direction}
\label{app: perisitent direction (np-imcmc)}

Let $\set{f^{(n)}:\entspace^n \times\auxspace^n \to \entspace^n \times\auxspace^n }_{n\in\Nat}$ be a family of non-involutive bijections where $\set{f^{(n)}}_n$ and $\set{\inv{f^{(n)}}}_n$ satisfy the \invoass{} (\cref{vass: partial block diagonal inv}) and
$\set{\nauxkernel{n}:\entspace^n \kernelto\auxspace^n}_{n\in\Nat}$ be a family of auxiliary kernels
where each is probabilistic and has pdf $\nauxpdf{n}$.

An NP-iMCMC sampler with \defn{persistent direction} proposes the next sample by applying the same map used in the previous step if the current sample was an accepted proposal,
otherwise a different map is used.

\cref{alg: np-imcmc with persistent direction} formulates this idea using a direction variable $\dira \in \dirspace$ which indicates which map to be used for each update.
(See details of the direction measure space $(\dirspace, \algebra{\dirspace}, \measure{\dirspace})$ in \cref{app: auxiliary direction (np-imcmc)}.)
In this case, $\dira = +$ indicates $\set{f^{(n)}}_n$ and $\dira = -$ indicates $\set{\inv{f^{(n)}}}_n$.
Hence, we see the input and output in \cref{alg: np-imcmc with persistent direction} include a direction variable in $\dirspace$ which stays the same if $\range{\enta}{1}{k} \in \support{\tree}$ is accepted; otherwise flipped.

\begin{algorithm}
\caption{NP-iMCMC with persistent direction}
\label{alg: np-imcmc with persistent direction}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    current direction $\dira_0:\dirspace$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of non-involutive bijections $\set{f^{(n)} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    a family of auxiliary kernels $\set{\nauxkernel{n} : \entspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$, next direction $\dira:\dirspace$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $\ninvo{n} = \begin{cases}
    f^{(n)} & \text{if } \dira = + \\
    \inv{f^{(n)}} & \text{if } \dira = -
  \end{cases} $ for all $n\in\Nat$
  \STATE $\auxa_0 \sim \nauxkernel{\len{\enta_0}}(\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \measure{\auxspace}$;
    % \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \nauxkernel{\len{\enta_0}+1}(\entelem, \placeholder)$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {
        \tree{(\range{\enta}{1}{k})}\cdot
        \nauxpdf{k}(\range{\enta}{1}{k}, \range{\auxa}{1}{k}) \cdot
        \nstockpdf{n}(\enta, \auxa)
      }
      {
        \tree{(\range{\enta_0}{1}{k_0})}\cdot
        \nauxpdf{k_0}(\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0}) \cdot
        \nstockpdf{n}(\enta_0, \auxa_0)
      }
    \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
    and $n = \len{\enta}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$, $\dira_0$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$, $\flip(\dira_0)$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\iffalse
\subsubsection*{Correctness}

We argue the correctness of NP-iMCMC update with persistent direction (\cref{alg: np-imcmc with persistent direction}) by
augmenting the entropy space $\entspace$ with the direction space $\dirspace$,
making the state $(\enta, \dirb, \auxa)$ an element of $\entspace^n \times \dirspace^n \times \auxspace^n$ in which the first component of $\dirb$ indicates which function ($f^{(n)}$ or $\inv{f^{(n)}}$) to be used.

In this case, we redefine the target density function to be
$\new{\tree}:(\traceb, \dirb) \mapsto \tree(\traceb)$ on the parameter space $\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)$, equipped with the
$\sigma$-algebra $\algebra{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)} := \set{\bigcup_{n\in\Nat} \entseta_n \mid \entseta_n \in \algebra{\entspace^n \times \dirspace^n}}$ and
measure $\measure{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)}(\bigcup_{n\in\Nat} \entseta_n) = \sum_{n\in\Nat} \measure{\entspace^n \times \dirspace^n}(\entseta_n)$
where $\entspace^n \times \dirspace^n$ is the Cartesian product of $\entspace^n$ and $\dirspace^n$ equipped with the product $\sigma$-algebra $\algebra{\entspace^n \times \dirspace^n}$ and
product measure $\measure{\entspace^n \times \dirspace^n}$.
Note that $\new{\tree}$ inherits the prefix property, integrability and almost surely terminating property (w.r.t.~$\measure{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)} $) from $\tree$.

We consider the composition of two NP-iMCMC samplers $\imcmca$ and $\imcmcb$ (do $\imcmca$ and then $\imcmcb$);
both update the sample $(\enta, \dirb)$ with density function $\new{\tree}$ on the parameter space $\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)$.

Given a sample $(\enta_0, \dirb_0)$, the first sampler $\imcmca$
applies $f^{(n)}$ or $\inv{f^{(n)}}$ to $(\enta_0, \auxa_0)$ where $\auxa_0$ is a randomly drawn value from $\nauxkernel{n}(\enta_0, \placeholder)$
according to the first component of the direction variable $\dirb_0$,
and flips each component of the directional variable $\dirb_0$, to generate a proposal $(\enta, \dirb)$.
The returned sample $(\enta_1, \dirb_1)$ of $\imcmca$ is either the proposal $(\enta, \dirb)$ or the initial sample $(\enta_0, \dirb_0)$.
This returned sample $(\enta_1, \dirb_1)$ is then passed on to the next sampler $\imcmcb$ which
flips each component of the direction variable $\dirb_1$ and
returns $(\enta_2, \dirb_2) = (\enta_1, \flip(\dirb_1))$.

Consider the change of the direction variable (from $\dirb_0$ to $\dirb_2$) and the accept/reject step in $\imcmca$.
If the proposal in $\imcmca$ is accepted (i.e.~$\enta_2=\enta$),
the direction variable $\dirb_2$ is identical to $\dirb_0$ (the result of flipping each component of $\dirb_0$ twice).
Otherwise (the proposal $\enta$ in $\imcmca$ is rejected and $\enta_2$ remains $\enta_0$), the direction variable $\dirb_2$ is the exact opposite of $\dirb_0$.
Since the first component of the direction variable indicates which function to be used,
when the proposal is accepted,
the direction remains unchanged and the involution ``persists''.

Formally, the first NP-iMCMC update $\imcmca$ takes as involution ${\ninvo{n}}_{\imcmca}$ on $\entspace^n \times \dirspace^n \times \auxspace^n$
such that
${\ninvo{n}}_{\imcmca}(\enta, \dirb, \auxa) = (\enta', \dirb', \auxa')$ where
\[
  (\enta', \auxa') =
  \begin{cases}
    f^{(n)}(\enta, \auxa) & \text{if } \seqindex{\dirb}{1} = + \\
    \inv{f^{(n)}}(\enta, \auxa) & \text{if } \seqindex{\dirb}{1} = -
  \end{cases}
  \text{ and }
  \seqindex{\dirb'}{i} = \flip(\seqindex{\dirb}{i}) \text{ for all }i = 1,\dots, n
\]
for each dimension $n\in\Nat$;
and auxiliary kernel ${\nauxkernel{n}}_{\imcmca}:\entspace^n \times \dirspace^n \kernelto \auxspace^n$ such that
$\nauxkernel{n}_{\imcmca}(\enta, \dirb) := \nauxkernel{n}(\enta)$
which is probabilistic and
has pdf ${\nauxpdf{n}}_{\imcmca}$ on $\entspace^n \times \dirspace^n \times \auxspace^n$ such that
${\nauxpdf{n}}_{\imcmca}(\enta, \dirb, \auxa) := {\nauxpdf{n}(\enta, \auxa)}$.

It is easy to check that ${\ninvo{n}}_{\imcmca}$ is involutive and satisfies the \invoass{}.
Line 4 to 17 in \cref{alg: np-imcmc with directional inputs and flipping} gives the pseudocode for the NP-iMCMC update $\imcmca$.

\iffalse
This means given a current sample, say $(\enta, \dirb)$ where $\seqindex{\dirb}{1} = +$, the iMCMC update $\imcmca$ proposes the next sample by running $f$ on the state $(\enta, \auxa)$ with a randomly drawn auxiliary value $\auxa$ from $\nauxkernel{n}(\enta)$ to obtain $(\enta', \auxa')$ and accepts $(\enta',\flip(\dirb))$ as the next sample with probability
\[
  \min \left\{1,
    \tfrac
      {\new{\tree}(\enta,\dirb) \cdot \exauxpdf_\imcmca({\enta},{\dirb},{\auxa}) }
      {\new{\tree}(\enta_0,\dirb_0) \cdot \exauxpdf_\imcmca({\enta_0},{\dirb_0},{\auxa_0})}
    \abs{\det{\big(\grad{\ninvo{\len{\enta}}_\imcmca}(\enta_0,\dirb_0,\auxa_0)\big)}}
    \right\}
  =
  \min \left\{1,
    \tfrac
      {\tree(\enta) \cdot \exauxpdf({\enta},{\auxa}) }
      {\tree(\enta_0) \cdot \exauxpdf({\enta_0},{\auxa_0})}
    \abs{\det{\big(\grad{f}(\enta_0,\auxa_0)\big)}}
    \right\}.
\]
\fi

Notice that if we simply use $\imcmca$ to generate the Markov chain, it will remain reversible.
To make it nonreversible, it is composed with another iMCMC update $\imcmcb$
with involution $\ninvo{n}_{\imcmcb}(\enta, \dirb, \auxa) := (\enta, \flip(\dirb), \auxa)$
and auxiliary kernel $\nauxkernel{n}_{\imcmcb}(\enta, \dirb, \auxseta) := \measure{\auxspace^n}(\auxseta)$ with is probabilistic and has pdf $\pdf{\measure{\auxspace^n}}$.
\iffalse
For instance, given the current sample, say $(\enta', \dirb')$ with $\seqindex{\dirb'}{1} = -$, the NP-iMCMC sampler $\imcmcb$ (samples an auxiliary variable $\auxa'$ from the stock measure $\measure{\auxspace^{\len{\enta'}}}$ and) simply flips the direction and proposes $(\enta', \flip(\dirb'))$ where $\seqindex{\flip{(\dirb')}}{1} = +$, which is accepted with probability
\[
  \min \left\{1,
    \tfrac
      {\new{\tree}(\enta',\flip(\dirb')) \cdot \exauxpdf_\imcmcb(({\enta'},\flip{(\dirb')}),{\auxa'}) }
      {\new{\tree}(\enta',\dirb') \cdot \exauxpdf_\imcmcb(({\enta'},{\dirb'}),{\auxa'})}
    \abs{\det{\big(\grad{\ninvo{\len{\enta}}_\imcmcb}(\enta_0,\dirb_0,\auxa_0)\big)}}
    \right\}
  =
  1.
\]
\fi

It is obvious that ${\ninvo{n}}_{\imcmcb}$ is involutive and satisfies the \invoass{}.
Line 18 to 30 in \cref{alg: np-imcmc with directional inputs and flipping} gives the pseudocode for the NP-iMCMC update $\imcmcb$.

\begin{algorithm}
\caption{NP-iMCMC with directional inputs and flipping}
\label{alg: np-imcmc with directional inputs and flipping}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0 : \traces$,
    current direction $\dirb_0: \bigcup_{n\in\Nat}\dirspace^n$,
    joint density function $\new{\tree}:\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n) \to \pReal$}
  \STATE \Input{
    a family of involutions for the NP-iMCMC sampler $\imcmca$
    $\set{
      \ninvo{n}_{\imcmca}: (\entspace^n \times \dirspace^n) \times \auxspace^n \to (\entspace^n \times \dirspace^n) \times \auxspace^n
    }_n$,
    a family of auxiliary kernels for the NP-iMCMC sampler $\imcmca$
    $\set{\nauxkernel{n}_{\imcmca}: \entspace^n \times \dirspace^n \kernelto \auxspace^n}_n$,
    a family of involutions for the NP-iMCMC sampler $\imcmcb$
    $\set{
      \ninvo{n}_{\imcmcb}: (\entspace^n \times \dirspace^n) \times \auxspace^n \to (\entspace^n \times \dirspace^n) \times \auxspace^n
    }_n$,
    a family of auxiliary kernels for the NP-iMCMC sampler $\imcmcb$
    $\set{\nauxkernel{n}_{\imcmcb}: \entspace^n \times \dirspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{
    Next sample $\traceb:\traces$,
    next direction $\dirb: \bigcup_{n\in\Nat}\dirspace^n$}
  % NP-iMCMC a
  \STATE $\enta_0 = \traceb_0$
  \STATE $\auxa_0 \sim {\nauxkernel{\len{\enta_0}}}_{\imcmca}(\enta_0, \dirb_0, \placeholder)$
  \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_0}}}_{\imcmca}(\enta_0,\dirb_0,\auxa_0)$
  \WHILE{$(\range{\enta}{1}{k}, \range{\dirb}{1}{k}) \not\in\support{\new{\tree}}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\direlem \sim \measure{\dirspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_0,\dirb_0,\auxa_0) = (\enta_0 \concat [\entelem], \dirb_0 \concat [\direlem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_0}}}_{\imcmca}(\enta_0,\dirb_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min \left\{1,
    \displaystyle\frac
      {\new{\tree}{(\range{\enta}{1}{k}, \range{\dirb}{1}{k})}\cdot\nauxpdf{k}_{\imcmca}(\range{\enta}{1}{k}, \range{\dirb}{1}{k}, \range{\auxa}{1}{k}) }
      {\new{\tree}{(\range{\enta_0}{1}{k_0}, \range{\dirb_0}{1}{k_0})}\cdot\nauxpdf{k_0}_{\imcmca}(\range{\enta_0}{1}{k_0}, \range{\dirb}{1}{k_0}, \range{\auxa_0}{1}{k_0}) }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta}}_{\imcmca}(\enta_0, \dirb_0, \auxa_0)})}\right\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE $\enta_1 = \range{\enta}{1}{k} \in \support{\tree}$ and $\dirb_1 = \range{\dirb}{1}{k}$
  \ELSE
    \STATE $\enta_1 = \range{\enta_0}{1}{k} \in \support{\tree}$ and $\dirb_1 = \range{\dirb_0}{1}{k}$
  \ENDIF
  % NP-iMCMC b
  \STATE $\auxa_1 \sim {\nauxkernel{\len{\enta_1}}}_{\imcmcb}(\enta_1, \dirb_1, \placeholder)$
  \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_1}}}_{\imcmcb}(\enta_1,\dirb_1,\auxa_1)$
  \WHILE{$(\range{\enta}{1}{k}, \range{\dirb}{1}{k}) \not\in\support{\new{\tree}}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\direlem \sim \measure{\dirspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_1,\dirb_1,\auxa_1) = (\enta_1 \concat [\entelem], \dirb_1 \concat [\direlem], \auxa_1 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_1}}}_{\imcmcb}((\enta_1,\dirb_1),\auxa_1)$
  \ENDWHILE
  \STATE $P :=
    \min \left\{1,
    \displaystyle\frac
      {\new{\tree}{(\range{\enta}{1}{k}, \range{\dirb}{1}{k})}\cdot\nauxpdf{k}_{\imcmcb}(\range{\enta}{1}{k}, \range{\dirb}{1}{k}, \range{\auxa}{1}{k}) }
      {\new{\tree}{(\range{\enta_1}{1}{k_1}, \range{\dirb_1}{1}{k_1})}\cdot\nauxpdf{k_1}_{\imcmcb}(\range{\enta_1}{1}{k_1}, \range{\dirb}{1}{k_1}, \range{\auxa_1}{1}{k_1}) }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta}}_{\imcmcb}(\enta_1, \dirb_1, \auxa_1)})}\right\}$
    where $\range{\enta}{1}{k}, \range{\enta_1}{1}{k_1} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\enta_2 = \range{\enta}{1}{k} \in \support{\tree}$ and $\dirb = \range{\dirb}{1}{k}$
  \ELSE
    \STATE \Return $\enta_2 = \range{\enta_1}{1}{k} \in \support{\tree}$ and $\dirb = \range{\dirb_1}{1}{k}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

By \cref{thm: invariant}, the transition kernels of the NP-iMCMC updates $\imcmca$ and $\imcmcb$ are reversible and hence preserves the target density $\new{\tree}$.
As shown in \cref{prop: invariant is closed under composition}, their composition $\imcmcb \circ \imcmca$ (\cref{alg: np-imcmc with directional inputs and flipping}) also preserves $\new{\tree}$.
Finally, we argue that \cref{alg: np-imcmc with persistent direction} is a simplified version of \cref{alg: np-imcmc with directional inputs and flipping} as follows:
\begin{itemize}
  \item $\auxa_1$ in $\imcmcb$ can be omitted as it is not used.

  \item We note $(\enta, \dirb, \auxa) = \ninvo{\len{\enta_1}}_{\imcmcb}(\enta_1, \dirb_1, \auxa_1) = (\enta_1, \flip(\dirb_1), \auxa_1)$ and $\enta = \enta_1 \in \support{\tree}$.
  So the condition of the while loop in Line 20 never satisfy and the while loop (Line 20 to Line 24) can be omitted.

  \item The acceptance ratio of $\imcmcb$ equals to $1$ and hence $\range{\enta}{1}{k}$ and $\range{\dirb}{1}{k}$ can be returned directly.

  \item Only the first component of $\dirb$ has effects on the both updates $\imcmca$ and $\imcmcb$.
  So, the rest of the components are redundant and can be removed.

\end{itemize}
Writing the first component of $\dirb_0$ as $\dira_0$, the resulting algorithm becomes \cref{alg: np-imcmc with persistent direction}.
Hence, \cref{alg: np-imcmc with persistent direction} is correct.
\fi

\subsection{Persistent Auxiliary Kernel}
\label{app: persistent auxiliary kernel (np-imcmc)}

Let
$\set{\ninvo{n}:\entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n $
be a family of involutions that satisfies \invoass{} and
$\set{\nauxkernel{n}_{+}: \entspace^n \kernelto \auxspace^n}_n $ and
$\set{\nauxkernel{n}_{-}: \entspace^n \kernelto \auxspace^n}_n $
be two families of auxiliary kernels
where each is probabilistic and has pdf $\nauxpdf{n}_1$ and $\nauxpdf{n}_2$.

An NP-iMCMC update with \defn{persistent auxiliary kernel} proposes the next sample
by applying $\ninvo{n}$ to the state $(\enta_0, \auxa_0)$
where
$\auxa_0$ is sampled from the auxiliary kernel used in the previous step if the current sample was an accepted proposal,
otherwise a different auxiliary kernel is used.

\cref{alg: np-imcmc with persistent auxiliary kernel} presents this idea using a direction variable $\dira \in \dirspace$ which indicates which auxiliary kernel to use to update the current sample.
(See details of the direction measure space $(\dirspace, \algebra{\dirspace}, \measure{\dirspace})$ in \cref{app: auxiliary direction (np-imcmc)}.)
In this case, $\dira = +$ indicates $\set{\nauxkernel{n}_{+}}_n$ and $\dira = -$ indicates $\set{\nauxkernel{n}_{-}}_n$.
Hence, we see the input and output in \cref{alg: np-imcmc with persistent direction} include a direction variable in $\dirspace$ which stays the same if $\range{\enta}{1}{k} \in \support{\tree}$ is accepted; otherwise flipped.

\begin{algorithm}
\caption{NP-iMCMC with persistent auxiliary kernel}
\label{alg: np-imcmc with persistent auxiliary kernel}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0:\traces$,
    current direction $\dira_0:\dirspace$,
    tree representable function $\tree :\traces \to \pReal$,
    a family of involutions $\set{\ninvo{n} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ and
    two families of auxiliary kernels $\set{\nauxkernel{n}_{+} : \entspace^n \kernelto \auxspace^n}_n$
    and $\set{\nauxkernel{n}_{-} : \entspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{Next sample $\traceb:\traces$, next direction $\dira:\dirspace$}
  \STATE $\enta_0 = \traceb_0$
  \STATE $\auxa_0 \sim \nauxkernel{\len{\enta_0}}_{\dira_0} (\enta_0, \placeholder)$
  \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \WHILE{$\range{\enta}{1}{k} \not\in\support{\tree}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$; $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_0, \auxa_0) = (\enta_0 \concat [\entelem], \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\auxa) = \ninvo{\len{\enta_0}}(\enta_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min\bigg\{1; \;
    \displaystyle\frac
      {
        \tree{(\range{\enta}{1}{k})}\cdot
        \nauxpdf{k}_{\dira_0}(\range{\enta}{1}{k}, \range{\auxa}{1}{k}) \cdot
        \nstockpdf{n}(\enta, \auxa)
      }
      {
        \tree{(\range{\enta_0}{1}{k_0})}\cdot
        \nauxpdf{k_0}_{\flip(\dira_0)} (\range{\enta_0}{1}{k_0}, \range{\auxa_0}{1}{k_0}) \cdot
        \nstockpdf{n}(\enta_0, \auxa_0)
      }
    \cdot \abs{\det(\grad{\ninvo{n}(\enta_0, \auxa_0)})}\bigg\}
    $
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
    and $n = \len{\enta}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\range{\enta}{1}{k} \in \support{\tree}$, $\dira_0$
  \ELSE
    \STATE \Return $\range{\enta_0}{1}{k_0} \in \support{\tree}$, $\flip(\dira_0)$
  \ENDIF
\end{algorithmic}
\end{algorithm}

\iffalse
\subsubsection*{Correctness}

We argue the correctness of NP-iMCMC update with persistent auxiliary kernel (\cref{alg: np-imcmc with persistent auxiliary kernel}) by
augmenting the entropy space $\entspace$ with the direction space $\dirspace$,
making the state $(\enta, \dirb, \auxa)$ an element of $\entspace^n \times \dirspace^n \times \auxspace^n$ in which the first component of $\dirb$ indicates which function ($f^{(n)}$ or $\inv{f^{(n)}}$) to be used.

In this case, we redefine the target density function to be
$\new{\tree}:(\traceb, \dirb) \mapsto \tree(\traceb)$ on the parameter space $\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)$, equipped with the
$\sigma$-algebra $\algebra{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)} := \set{\bigcup_{n\in\Nat} \entseta_n \mid \entseta_n \in \algebra{\entspace^n \times \dirspace^n}}$ and
measure $\measure{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)}(\bigcup_{n\in\Nat} \entseta_n) = \sum_{n\in\Nat} \measure{\entspace^n \times \dirspace^n}(\entseta_n)$
where $\entspace^n \times \dirspace^n$ is the Cartesian product of $\entspace^n$ and $\dirspace^n$ equipped with the product $\sigma$-algebra $\algebra{\entspace^n \times \dirspace^n}$ and
product measure $\measure{\entspace^n \times \dirspace^n}$.
Note that $\new{\tree}$ inherits the prefix property, integrability and almost surely terminating property (w.r.t.~$\measure{\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)} $) from $\tree$.

We consider the composition of two NP-iMCMC samplers $\imcmca$ and $\imcmcb$ (do $\imcmca$ and then $\imcmcb$);
both update the sample $(\enta, \dirb)$ with density function $\new{\tree}$ on the parameter space $\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n)$.

Given a sample $(\enta_0, \dirb_0)$, the first sampler $\imcmca$
applies $\ninvo{n}$ to $(\enta_0, \auxa_0)$ where
$\auxa_0$ is a randomly drawn value from $\nauxkernel{n}_{+}(\enta_0, \placeholder)$ or $\nauxkernel{n}_{-}(\enta_0, \placeholder)$
according to the first component of the direction variable $\dirb_0$,
and flips each component of the directional variable $\dirb_0$, to generate a proposal $(\enta, \dirb)$.
The returned sample $(\enta_1, \dirb_1)$ of $\imcmca$ is either the proposal $(\enta, \dirb)$ or the initial sample $(\enta_0, \dirb_0)$.
This returned sample $(\enta_1, \dirb_1)$ is then passed on to the next sampler $\imcmcb$ which
flips each component of the direction variable $\dirb_1$ and
returns $(\enta_2, \dirb_2) = (\enta_1, \flip(\dirb_1))$.

Consider the change of the direction variable (from $\dirb_0$ to $\dirb_2$) and the accept/reject step in $\imcmca$.
If the proposal in $\imcmca$ is accepted (i.e.~$\enta_2=\enta$),
the direction variable $\dirb_2$ is identical to $\dirb_0$ (the result of flipping each component of $\dirb_0$ twice).
Otherwise (the proposal $\enta$ in $\imcmca$ is rejected and $\enta_2$ remains $\enta_0$), the direction variable $\dirb_2$ is the exact opposite of $\dirb_0$.
Since the first component of the direction variable indicates which function to be used,
when the proposal is accepted,
the direction remains unchanged and the auxiliary kernel ``persists''.

Formally, the first NP-iMCMC update $\imcmca$ takes as involution ${\ninvo{n}}_{\imcmca}$ on $\entspace^n \times \dirspace^n \times \auxspace^n$
such that
${\ninvo{n}}_{\imcmca}(\enta, \dirb, \auxa) = (\enta', \dirb', \auxa')$ where
$(\enta', \auxa') = \ninvo{n}(\enta, \auxa)$
and
$\seqindex{\dirb'}{i} = \flip(\seqindex{\dirb}{i})$ for all $i = 1,\dots, n$
for each dimension $n\in\Nat$;
and auxiliary kernel ${\nauxkernel{n}}_{\imcmca}:\entspace^n \times \dirspace^n \kernelto \auxspace^n$ such that
\[
  \nauxkernel{n}_{\imcmca}(\enta, \dirb) := \begin{cases}
    \nauxkernel{n}_{+}(\enta) & \text{if } \seqindex{\dirb}{1} = + \\
    \nauxkernel{n}_{-}(\enta) & \text{if } \seqindex{\dirb}{1} = -
  \end{cases}
\]
which is probabilistic and
has pdf ${\nauxpdf{n}}_{\imcmca}$ on $\entspace^n \times \dirspace^n \times \auxspace^n$ such that
\[
  {\nauxpdf{n}}_{\imcmca}(\enta, \dirb, \auxa) := \begin{cases}
    {\nauxpdf{n}_1(\enta, \auxa)}& \text{if } \seqindex{\dirb}{1} = + \\
    {\nauxpdf{n}_2(\enta, \auxa)}& \text{if } \seqindex{\dirb}{1} = -.
  \end{cases}
\]

It is easy to check that ${\ninvo{n}}_{\imcmca}$ is involutive and satisfies the \invoass{}.
Line 4 to 17 in \cref{alg: np-imcmc with two auxiliary kernels and flipping} gives the pseudocode for the NP-iMCMC update $\imcmca$.

Notice that if we simply use $\imcmca$ to generate the Markov chain, it will remain reversible.
To make it nonreversible, it is composed with another iMCMC update $\imcmcb$
with involution $\ninvo{n}_{\imcmcb}(\enta, \dirb, \auxa) := (\enta, \flip(\dirb), \auxa)$
and auxiliary kernel $\nauxkernel{n}_{\imcmcb}(\enta, \dirb, \auxseta) := \measure{\auxspace^n}(\auxseta)$ with is probabilistic and has pdf $\pdf{\measure{\auxspace^n}}$.
\iffalse
For instance, given the current sample, say $(\enta', \dirb')$ with $\seqindex{\dirb'}{1} = -$, the NP-iMCMC sampler $\imcmcb$ (samples an auxiliary variable $\auxa'$ from the stock measure $\measure{\auxspace^{\len{\enta'}}}$ and) simply flips the direction and proposes $(\enta', \flip(\dirb'))$ where $\seqindex{\flip{(\dirb')}}{1} = +$, which is accepted with probability
\[
  \min \left\{1,
    \tfrac
      {\new{\tree}(\enta',\flip(\dirb')) \cdot \exauxpdf_\imcmcb(({\enta'},\flip{(\dirb')}),{\auxa'}) }
      {\new{\tree}(\enta',\dirb') \cdot \exauxpdf_\imcmcb(({\enta'},{\dirb'}),{\auxa'})}
    \abs{\det{\big(\grad{\ninvo{\len{\enta}}_\imcmcb}(\enta_0,\dirb_0,\auxa_0)\big)}}
    \right\}
  =
  1.
\]
\fi
It is obvious that ${\ninvo{n}}_{\imcmcb}$ is involutive and satisfies the \invoass{}.
Line 18 to 30 in \cref{alg: np-imcmc with directional inputs and flipping} gives the pseudocode for the NP-iMCMC update $\imcmcb$.

\begin{algorithm}
\caption{NP-iMCMC with two auxiliary kernels and flipping}
\label{alg: np-imcmc with two auxiliary kernels and flipping}
\begin{algorithmic}[1]
  \STATE \Input{
    Current sample $\traceb_0 : \traces$,
    current direction $\dirb_0: \bigcup_{n\in\Nat}\dirspace^n$,
    joint density function $\new{\tree}:\bigcup_{n\in\Nat}(\entspace^n \times \dirspace^n) \to \pReal$}
  \STATE \Input{
    a family of involutions for the NP-iMCMC sampler $\imcmca$
    $\set{
      \ninvo{n}_{\imcmca}: (\entspace^n \times \dirspace^n) \times \auxspace^n \to (\entspace^n \times \dirspace^n) \times \auxspace^n
    }_n$,
    a family of auxiliary kernels for the NP-iMCMC sampler $\imcmca$
    $\set{\nauxkernel{n}_{\imcmca}: \entspace^n \times \dirspace^n \kernelto \auxspace^n}_n$,
    a family of involutions for the NP-iMCMC sampler $\imcmcb$
    $\set{
      \ninvo{n}_{\imcmcb}: (\entspace^n \times \dirspace^n) \times \auxspace^n \to (\entspace^n \times \dirspace^n) \times \auxspace^n
    }_n$,
    a family of auxiliary kernels for the NP-iMCMC sampler $\imcmcb$
    $\set{\nauxkernel{n}_{\imcmcb}: \entspace^n \times \dirspace^n \kernelto \auxspace^n}_n$
  }
  \STATE \Output{
    Next sample $\traceb:\traces$,
    next direction $\dirb: \bigcup_{n\in\Nat}\dirspace^n$}
  % NP-iMCMC a
  \STATE $\enta_0 = \traceb_0$
  \STATE $\auxa_0 \sim {\nauxkernel{\len{\enta_0}}}_{\imcmca}(\enta_0, \dirb_0, \placeholder)$
  \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_0}}}_{\imcmca}(\enta_0,\dirb_0,\auxa_0)$
  \WHILE{$(\range{\enta}{1}{k}, \range{\dirb}{1}{k}) \not\in\support{\new{\tree}}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\direlem \sim \measure{\dirspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $(\enta_0,\dirb_0,\auxa_0) = ((\enta_0 \concat [\entelem], \dirb_0 \concat [\direlem]), \auxa_0 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_0}}}_{\imcmca}(\enta_0,\dirb_0,\auxa_0)$
  \ENDWHILE
  \STATE $P :=
    \min \left\{1,
    \displaystyle\frac
      {\new{\tree}{(\range{\enta}{1}{k}, \range{\dirb}{1}{k})}\cdot\nauxpdf{k}_{\imcmca}(\range{\enta}{1}{k}, \range{\dirb}{1}{k}, \range{\auxa}{1}{k}) }
      {\new{\tree}{(\range{\enta_0}{1}{k_0}, \range{\dirb_0}{1}{k_0})}\cdot\nauxpdf{k_0}_{\imcmca}(\range{\enta_0}{1}{k_0}, \range{\dirb}{1}{k_0}, \range{\auxa_0}{1}{k_0}) }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta}}_{\imcmca}(\enta_0, \dirb_0, \auxa_0)})}\right\}$
    where $\range{\enta}{1}{k}, \range{\enta_0}{1}{k_0} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE $\enta_1 = \range{\enta}{1}{k} \in \support{\tree}$ and $\dirb_1 = \range{\dirb}{1}{k}$
  \ELSE
    \STATE $\enta_1 = \range{\enta_0}{1}{k} \in \support{\tree}$ and $\dirb_1 = \range{\dirb_0}{1}{k}$
  \ENDIF
  % NP-iMCMC b
  \STATE $\auxa_1 \sim {\nauxkernel{\len{\enta_1}}}_{\imcmcb}((\enta_1, \dirb_1), \placeholder)$
  \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_1}}}_{\imcmcb}((\enta_1,\dirb_1),\auxa_1)$
  \WHILE{$(\range{\enta}{1}{k}, \range{\dirb}{1}{k}) \not\in\support{\new{\tree}}$ for all $k = 1,\dots, \len{\enta}$}
    % sample
    \STATE $\entelem \sim \measure{\entspace}$;
    $\direlem \sim \measure{\dirspace}$;
    $\auxelem \sim \measure{\auxspace}$;
    % extend initial state
    \STATE $((\enta_1,\dirb_1),\auxa_1) = ((\enta_1 \concat [\entelem], \dirb_1 \concat [\direlem]), \auxa_1 \concat [\auxelem])$
    % run involution
    \STATE $(\enta,\dirb,\auxa) = {\ninvo{\len{\enta_1}}}_{\imcmcb}((\enta_1,\dirb_1),\auxa_1)$
  \ENDWHILE
  \STATE $P :=
    \min \left\{1,
    \displaystyle\frac
      {\new{\tree}{(\range{\enta}{1}{k}, \range{\dirb}{1}{k})}\cdot\nauxpdf{k}_{\imcmcb}(\range{\enta}{1}{k}, \range{\dirb}{1}{k}, \range{\auxa}{1}{k}) }
      {\new{\tree}{(\range{\enta_1}{1}{k_1}, \range{\dirb_1}{1}{k_1})}\cdot\nauxpdf{k_1}_{\imcmcb}(\range{\enta_1}{1}{k_1}, \range{\dirb}{1}{k_1}, \range{\auxa_1}{1}{k_1}) }
    \cdot \abs{\det(\grad{\ninvo{\len{\enta}}_{\imcmcb}(\enta_1, \dirb_1, \auxa_1)})}\right\}$
    where $\range{\enta}{1}{k}, \range{\enta_1}{1}{k_1} \in \support{\tree}$
  \IF{$\Uni(0,1) < P$}
    \STATE \Return $\enta = \range{\enta}{1}{k} \in \support{\tree}$ and $\dirb = \range{\dirb}{1}{k}$
  \ELSE
    \STATE \Return $\enta = \range{\enta_1}{1}{k} \in \support{\tree}$ and $\dirb = \range{\dirb_1}{1}{k}$
  \ENDIF
\end{algorithmic}
\end{algorithm}

By \cref{thm: invariant}, the transition kernels of the NP-iMCMC updates $\imcmca$ and $\imcmcb$ are reversible and hence preserves the target density $\new{\tree}$.
As shown in \cref{prop: invariant is closed under composition}, their composition $\imcmcb \circ \imcmca$ (\cref{alg: np-imcmc with two auxiliary kernels and flipping}) also preserves $\new{\tree}$.
Finally, we argue that \cref{alg: np-imcmc with persistent auxiliary kernel} is a simplified version of \cref{alg: np-imcmc with two auxiliary kernels and flipping} as follows:
\begin{itemize}
  \item $\auxa_1$ in $\imcmcb$ can be omitted as it is not used.

  \item We note $(\enta, \dirb, \auxa) = \ninvo{\len{\enta_1}}_{\imcmcb}(\enta_1, \dirb_1, \auxa_1) = (\enta_1, \flip(\dirb_1), \auxa_1)$ and $\enta = \enta_1 \in \support{\tree}$.
  So the condition of the while loop in Line 20 never satisfy and the while loop (Line 20 to Line 24) can be omitted.

  \item The acceptance ratio of $\imcmcb$ equals to $1$ and hence $\range{\enta}{1}{k}$ and $\range{\dirb}{1}{k}$ can be returned directly.

  \item Only the first component of $\dirb$ has effects on the both updates $\imcmca$ and $\imcmcb$.
  So, the rest of the components are redundant and can be removed.

\end{itemize}
Writing the first component of $\dirb_0$ as $\dira_0$, the resulting algorithm becomes \cref{alg: np-imcmc with persistent auxiliary kernel}.
Hence, \cref{alg: np-imcmc with persistent auxiliary kernel} is correct.

\iffalse

\subsection{Composite Involution (CI)}
\label{app: composite involution}

Some involutions are by construction compositions of involutions.
Suppose there are families $\set{\elemfn{n}_{\ell} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n \mid n \in \Nat, \ell = 1,\dots, L}$ where, for all $n \in \Nat$, the involution $\ninvo{n}$ is composed of $\set{\elemfn{n}_{\ell}}_{\ell = 1,\dots,L}$.

\subsubsection{Algorithm}

Similar to Vanilla NP-iMCMC, we assume \allvass{} are satisfied. Furthermore, we assume all $\elemfn{n}_i$ are block diagonal. Formally
\begin{description}
  \item[\ciass \label{ciass: elemfn are block diagonal}]
  For each $i$, the family $\set{\elemfn{n}_i:\entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n}_n$ of involutions is \defn{block diagonal} with
  the family $\set{\neutfn{n}_i:\entspace \times \auxspace \to \entspace \times \auxspace }_{n\in\Nat}$ as its extension, i.e.~
  for all $\enta \in \support{\trunc{n}}$, $\auxa \in \auxspace^n$, $\entelem \in \entspace$, $\auxelem \in \auxspace$,
  \[
    \elemfn{n+1}_i(\enta\concat[\entelem],\auxa\concat[\auxelem]) =
    (\enta'\concat[\entelem'],\auxa'\concat[\auxelem'])
  \]
  where
  \(
    \elemfn{n}_i(\enta,\auxa) = (\enta',\auxa')
    \quad \hbox{and} \quad
    \neutfn{n+1}_i(\entelem,\auxelem) = (\entelem',\auxelem')
\)
  \item[\ciass \label{ciass: very strong irreducible}]
  All $\elemfn{n}_i$ are very strong irreducible.
\end{description}
\newcommand{\allciass}{\cref{ciass: elemfn are block diagonal,ciass: very strong irreducible}}

Now running the involution $\ninvo{n}$ means iterating through $\elemfn{n}_{\ell}$ for $\ell = 1,\dots, L$.
Say we are at the $\ell$-th iteration and the current entropy trace $\enta$ is not in the support of the truncation $\trunc{\len{\enta}}$.
After the initial state being extended (\cref{line: CI NP-iMCMC extend initial state}), the involution is run up to $\elemfn{\len{\enta}+1}_{\ell}$ (\cref{line: CI NP-iMCMC loop run involution}).
Hence, the proposal step of \defn{Composition of Involutions (CI) NP-iMCMC} is as in \cref{alg: CI NP-iMCMC}.

\cm{Rewrite algorithm}
\iffalse
\begin{algorithm}[t]
  \Input{
    Current state $(\enta_0,\auxa_0): \states$,
    truncations $\trunc{n} :\entspace^n \to \pReal$,
    families of involutions $\set{\elemfn{n}_{\ell} : \entspace^n \times \auxspace^n \to \entspace^n \times \auxspace^n \mid \ell = 1,\dots, L}_n$
    with extensions $\set{\neutfn{n}_{\ell} :\entspace\times\auxspace\to\entspace\times\auxspace \mid \ell = 1,\dots, L}_{n}$,
    family of auxiliary kernels $\set{\nauxkernel{n} : \entspace \kernelto\auxspace}_n$ }
  \Output{Next state $(\enta,\auxa): \states$ and updated current state $(\enta_0,\auxa_0): \states$}
  \BlankLine
  \tcc{Proposal}
  $(\enta,\auxa) = (\enta_0,\auxa_0)$\;
  \For{$\ell = 1,\dots, L$}{
    \tcc{run the $\ell$-th involution}
    $(\enta,\auxa) = \elemfn{\len{\enta}}_{\ell}(\enta,\auxa)$\;
    \While{$\enta \not\in \support{\trunc{\len{\enta}}}$}{ \label{line: CI NP-iMCMC loop start}
      \tcp{extend initial state}
      % sample
      $\entelem \sim \measure{\entspace}$;
      $\auxelem \sim \auxkernel{\len{\enta_0}+1}(\entelem)$;
      % extend initial state
      $\enta_0 = \enta_0 \concat [\entelem]$;
      $\auxa_0 = \auxa_0 \concat [\auxelem]$\;
      \label{line: CI NP-iMCMC extend initial state}
      \tcp{run involution up to $\elemfn{\len{\enta_0}}_\ell$}
      % run involution
      $(\entelem',\auxelem') = (\neutfn{\len{\enta_0}}_\ell \circ \dots \circ \neutfn{\len{\enta_0}}_1) {(\entelem,\auxelem)}$;
      % extend current state
      $\enta = \enta \concat [\entelem']$;
      $\auxa = \auxa \concat [\auxelem']$
      \label{line: CI NP-iMCMC loop run involution}
    } \label{line: CI NP-iMCMC loop end}
  }
  \Return $((\enta,\auxa),(\enta_0,\auxa_0))$\;
  \caption{Proposal step of CI NP-iMCMC Step}
  \label{alg: CI NP-iMCMC}
\end{algorithm}
\fi
\subsubsection*{Correctness}

% correctness
To justify its correctness, we re-define the valid states in terms of $\elemfn{n}_\ell$ instead of $\ninvo{n}$, i.e.~
\begin{align*}
  \validstates := \{
    (\enta,\auxa)\in \states & \mid
    \enta \in \support{\trunc{\len{\enta}}} \text{ and } \\
    & \forall \ell . (\enta',\auxa') = \elemfn{\len{\enta}}_{\leq \ell} (\enta,\auxa) \Rightarrow \enta' \in\support{\trunc{\len{\enta}}} \text{ and } \\
    & \forall k <\len{\enta} .
      (\range{\enta}{1}{k},\range{\auxa}{1}{k})\not\in \validstates
  \}.
\end{align*}
Then, given \cref{vass: integrable tree,vass: almost surely terminating tree,cass: everywhere positive aux density,ciass: elemfn are block diagonal,ciass: very strong irreducible}, we deduce from \cref{lemma: marginalised distribution is the target distribution,thm: np-imcmc correct} that CI NP-iMCMC algorithm (\cref{alg: CI NP-iMCMC}) is correct.

\subsubsection{Example (NP-HMC)}
\label{sec: Example (NP-HMC)}

The recently introduced \defn{Nonparametric Hamiltonian Monte Carlo (NP-HMC)} algorithm \cite{DBLP:conf/icml/MakZO21}, which infers a probabilistic model defined by a universal PPL program, is an instantiation of NP-iMCMC, by application of the composition of involutions.

Recall HMC is an inference algorithm for a (fixed-dimensional) density function $d$ on $\Real^n$ which, given the current sample $\vec{q_0}$ (and meta parameters: leapfrog step size $\epsilon$ and number of steps $L$), proposes the next sample by ``traversing'' the state $(\vec{q_0},\vec{p_0})$ on the surface $U = -\log d$ with a randomly chosen ``momentum'' $\vec{p_0}$.

To construct a nonparametric extension of HMC, set $\entspace = \auxspace = \Real$, and define the family of involutions to be the Hamiltonian flow, i.e.~$\ninvo{n} := \momentumflip \circ (\elemfn{n})^{L}$, writing $(\elemfn{n})^{L} := \underbrace{\elemfn{n} \circ \dots \circ \elemfn{n}}_{L\text{ times}}$ where $\elemfn{n}$ is defined as a leapfrog step \cite{Neal2011} (also called the Velocity Verlet Algorithm \cite{PhysRev.159.98}):
\begin{align*}
  \vec{p} & = \vec{p} - \epsilon \cdot \grad{U}(\vec{q}) \\
  \vec{q} & = \vec{q} + \epsilon \cdot \vec{p} \\
  \vec{p} & = \vec{p} - \epsilon \cdot \grad{U}(\vec{q})
\end{align*}
\iffalse
\[
  \vec{p} = \vec{p} - \epsilon \cdot \grad{U}(\vec{q}) \qquad
  \vec{q} = \vec{q} + \epsilon \cdot \vec{p} \qquad
  \vec{p} = \vec{p} - \epsilon \cdot \grad{U}(\vec{q})
\]
\fi
and $\momentumflip(\vec{q},\vec{p}) := (\vec{q},-\vec{p}) $ flips the momentum.

It is straightforward to see that the Hamiltonian flow $\ninvo{n}$ is involutive.
The auxiliary space $\auxspace$ is simply the real line $\Real$ with auxiliary kernel $\nauxkernel{n}(\entelem,\auxseta) := \Gau(\auxseta)$ for all $n\in\Nat$, which is everywhere positive (\cref{cass: everywhere positive aux density}).

Moreover, the involutions are series of block diagonal functions (\cref{ciass: elemfn are block diagonal}), which implies $\ninvo{n}$ is partial block diagonal (\cref{vass: partial block diagonal inv}), w.r.t.~the family $\set{\neutfn{n}}_{n\in\Nat}$ where $\neutfn{n}(q,p) := (q+\epsilon \cdot p,p)$ represents the movement on a constant surface.
Hence the composition of involutions NP-iMCMC algorithm (\cref{alg: CI NP-iMCMC}) is applicable, and beneficial as the computation of leapfrog steps is the main expensive operation in HMC.
The resulting algorithm (\cref{alg: NP-HMC}) is thus identical to that given in \cite{DBLP:conf/icml/MakZO21}.
\fi
\fi
